Multiplicative Updates for NMF with $\beta$-Divergences under Disjoint Equality Constraints

Nonnegative matrix factorization (NMF) is the problem of approximating an input nonnegative matrix, $V$, as the product of two smaller nonnegative matrices, $W$ and $H$. In this paper, we introduce a general framework to design multiplicative updates (MU) for NMF based on $\beta$-divergences ($\beta$-NMF) with disjoint equality constraints, and with penalty terms in the objective function. By disjoint, we mean that each variable appears in at most one equality constraint. Our MU satisfy the set of constraints after each update of the variables during the optimization process, while guaranteeing that the objective function decreases monotonically. We showcase this framework on three NMF models, and show that it competes favorably the state of the art: (1)~$\beta$-NMF with sum-to-one constraints on the columns of $H$, (2) minimum-volume $\beta$-NMF with sum-to-one constraints on the columns of $W$, and (3) sparse $\beta$-NMF with $\ell_2$-norm constraints on the columns of $W$.

==> Chapters/2_betaNMF2310.tex <==
% \ngc{Je pense que cette section nécessite un ``serious facelift'' (j'utilise l'expression utilisée un jour par un reviewer).}

% \ngc{Je propose la chose suivante: 
% Avant de mettre `This section is organized as follows', il faut bien réexpliquer le contexte. On veut résoudre $\beta$-NMF avec pénalités et contraintes linéaires disjointes: donner le modèle général~\eqref{eq:betaNMFmodel} et introduire les notations. On voit ainsi directement ce qu'on veut faire/résoudre. 
% Ensuite, comme on fait de l'alterné, montrer que les sous-problèmes à résoudre ont la forme de~\eqref{eq:subprobleminW} et donc~\eqref{eq:minF}. 
% Finalement, donner la structure de la section.  
% }

% \ngc{Je le laisse retravailler cela et je relis après. J'ai mis d'autres commentaires également dans la section.}  

In this paper, we introduce a general framework to tackle $\beta$-NMF with disjoint linear equality constraints, and with penalty terms in the objective function. Let us first introduce specific notations: given a matrix $A \in \mathbb{R}^{F \times N}$ and a list of indices $\mathcal{K} \subseteq \{ (f,k) \ | \ 1 \leq f \leq F, 1 \leq n \leq N\}$, we denote $A(\mathcal{K})$ the vector of dimension $|\mathcal{K}|$ whose entries are the entries of $A$ corresponding to the indices within $\mathcal{K}$. 
Let us introduce $\mathcal{K}_{i}$ ($1 \leq i \leq I$) and $\mathcal{B}_{j}$ ($1 \leq j \leq J$) to be disjoint sets of indices for the entries of $W$ and $H$, respectively, that is, 
\begin{itemize}

    \item $\mathcal{K}_{i} \subseteq \{ (f,k) \ | \ 1 \leq f \leq F, 1 \leq k \leq K\}$ for  $i = 1,2,\dots,I$, 
    
    \item $\mathcal{B}_{j} \subseteq \{ (k,n) \ | \ 1 \leq k \leq K, 1 \leq n \leq N\}$ for $j = 1,2,\dots,J$,
    
    
    \item $\mathcal{K}_{u} \cap \mathcal{K}_{v} = \emptyset$ for all $1 \leq u,v \leq I$ and $u \neq v$,
    
    \item $\mathcal{B}_{q} \cap \mathcal{B}_{p} = \emptyset$ for all $1 \leq q,p \leq J$ and $q \neq p$. 
\end{itemize} 
We now define penalized $\beta$-NMF with disjoint linear equality constraints as follows 
\begin{equation}\label{eq:betaNMFmodel}
\begin{aligned}
& \underset{W\in \mathbb{R}^{F \times K}_+,H\in \mathbb{R}^{K \times N}_+}{\min}
& & D_{\beta}\left(V|WH\right) + \lambda_1 \Phi_1(W) + \lambda_2 \Phi_2(H) \\
& \text{such that}
%& & H \geq 0, W \geq 0, \\
%& \text{}
& & \alphab_i^{T} W \left( \mathcal{K}_{i} \right) = b_i \text{ for } 1\leq i \leq I, \\
& \text{}
& &  \gammab_j^{T} H \left( \mathcal{B}_{j} \right) = c_j \text{ for } 1\leq j \leq J,
\end{aligned}
\end{equation}
where %$D_{\beta}\left(V|WH\right)=\sum_{f,n} d_{\beta}(V_{fn}|[ \,WH] \,_{fn})$, 
\begin{itemize}
    \item the penalty functions $\Phi_1(W)$ and $\Phi_2(H)$ are separable functions\footnote{\ngi{This assumption is not strictly necessary, but is made because it greatly simplifies the presentation. It can be relaxed to the requirement that $\Phi_1(W)$ and $\Phi_2(H)$ possess an entry-wise quadratic separable majorizer of the form given in~\eqref{eq:Lipschtiz_case}. 
    This will be the case for our example in Section~\ref{sec_minvolKLNMF} where $\Phi_1(W) = \logdet(W^T W + \delta I)$ satisfies only the latter assumption.}} w.r.t.\ the rows of $W$ and columns of $H$,  respectively, that is, we have  
    $\Phi_2(H) = \sum_{n=1}^N \Phi_2(\hb_n)$ where $\hb_n \in \mathbb{R}_+^{F}$ denotes the $n$-th column of $H$, and similarly for $\Phi_1$. We will also need that $\Phi_1$ and $\Phi_2$ are concave, or admit an $L$-smooth gradient;  see Assumption~\ref{ass:phi} below. 
    
    \item $\lambda_1$ and $\lambda_2$ are the penalty weights (nonnegative scalars). 
    
    \item $\alphab_i \in \mathbb{R}^{|\mathcal{K}_i|}_{++}$ ($1\leq i \leq I$) and $\gammab_j \in \mathbb{R}^{|\mathcal{B}_j|}_{++}$ ($1\leq j \leq J$) are vectors with positive entries. 
    Note that if $\alphab_i$ or $\gammab_j$ contains zero entries,  the corresponding indices can be removed from $\mathcal{K}_{i}$ and $\mathcal{B}_{j}$.  
    
    \item $b_i$ ($1\leq i \leq I$) and $c_j$  ($1\leq j \leq J$) are positive scalars. 
\end{itemize}
% We denote by $\Psi$ the objective function 
% of~\eqref{eq:betaNMFmodel}, that is, 
% \[
% \Psi (W,H) = 
% D_{\beta}\left(V|WH\right) + \lambda_1 \Phi_1(W) + \lambda_2 \Phi_2(H). 
% \] 
%\ngc{(1) on a vraiment besoin qu'elles soient séparables? On montre justement plus bas comment s'en sortir si ce n'est pas le cas, non? Je pense qu'il faut juste qu'elles soient séparables par lignes de $W$ / colonnes de $H$, non? (2)  il faudrait de toute façon définir séparable.} \ngc{C'est la même pénalité sur $W$ et $H$? Ce n'est pas ce qu'on fait dans les exemples... Utiliser $\lambda_2 \Phi_2(H)$? Si c'était la même pénalité, il faudrait d'ailleurs plutôt utiliser  $\Phi_1(H^T)$ pour avoir la symmétrie.}  

As for most NMF algorithms, we propose to resort to a  block coordinate descent (BCD) framework 
to solve problem~\eqref{eq:betaNMFmodel}: at each iteration we tackle two sub-problems separately; one in $W$ and the other in $H$. 
% \algsetup{indent=2em}
% \begin{algorithm}[ht!]
% \caption{BCD framework to tackle NMF optimization problems \label{algo:metaalgo} }
% \begin{algorithmic}[1]
% \REQUIRE Input matrix $V \in \mathbb{R}^{F \times N}_+$, the factorization rank $K$ and
%  number of iterations maxiter. 
% \ENSURE $(W,H)$ is an approximate solution of~\eqref{eq:betaNMFmodel}. 
%     \medskip  
% \STATE Initialize $(W^{0}, H^{0}) \in \mathbb{R}^{F \times K}_+ \times \mathbb{R}^{K \times N}_+$. 
% \FOR {$k=1,2,\dots,$ maxiter}
%     \STATE \emph{\% Update $W$} 
%     \STATE $W^{k} \longleftarrow \text{update} (V,W^{k-1},H^{k-1}) \text{ typically such that }\Psi(W^{k},H^{k-1}) \leq \Psi(W^{k-1},H^{k-1})$ 
%     \STATE \emph{\% Update $H$} 
%     \STATE $H^{k} \longleftarrow \text{update} (V,W^{k},H^{k-1}) \text{ typically such that }\Psi(W^{k},H^{k}) \leq \Psi(W^{k},H^{k-1})$  
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}  
The subproblems in $W$ and $H$ are essentially the same, by symmetry of the model. Hence, we may focus on solving the  subproblem in $H$ only, namely 
\begin{equation}
\label{eq:betaNMFmodelH}
 \underset{H\in \mathbb{R}^{K \times N}_+}{\min}
 D_{\beta}\left(V|WH\right) + \lambda_2 \Phi_2(H) 
\quad \text{ such that } \quad 
 \gammab_j^{T} H \left( \mathcal{B}_{j} \right)=c_j \text{ for } 1\leq j \leq J. 
\end{equation} 
In order to tackle~\eqref{eq:betaNMFmodelH}, we will design MU based on the majorization-minimization (MM) framework~\cite{sun2017majorization}, which is the standard in the NMF literature; see~\cite{Fevotte_betadiv} and the references therein. 
It consists in two steps: find a function that is an upper approximation of the objective and is tight at the current iterate, which is referred to as a majorizer, 
then minimize the majorizer to obtain the next iterate. This guarantees the objective function to decrease at each step of this iterative process. 


To do so, we first provide a majorizer for the objective of~\eqref{eq:betaNMFmodelH} in Section~\ref{sec:majorizer}. This majorizer has the property to be separable in each entry of $H$. In order to handle the equality constraints, 
we introduce Lagrange dual variables in Section~\ref{sec:lagrange}, and explain how they can be computed efficiently. 
This allows us to derive general MU in Section~\ref{betanmf_disjointconstraint} in the case of non-penalized $\beta$-NMF under disjoint linear equality constraints.
 This is showcased on simplex-structured $\beta$-NMF in Section~\ref{sec_ssbetaNMF}. In Section~\ref{sec_minvolKLNMF}, we will illustrate on minimum-volume NMF  how to derive MU in the presence of penalty terms. 



%and then derive the proposed MU for~\eqref{eq:betaNMFmodelH} in Section~\ref{}.   


\subsection{Separable majorizer for the objective function} 
\label{sec:majorizer} 

The objective function of~\eqref{eq:betaNMFmodelH} can be decoupled into $n$ independent terms, one for each column $\hb_n$ of $H$: 
\begin{equation}
\label{eq:psi(H)}
\psi(H) := D_{\beta}\left(V|WH\right) + \lambda \Phi(H) = \sum_{n=1}^N \psi(\hb_n), 
\end{equation}
\ji{where $\psi(\hb_n) = D_{\beta}\left(\vb_n|W\hb_n\right) + \lambda \Phi(\hb_n)$.}
Note that, to simplify the notation, we write $\Phi_2(H) = \Phi(H)$, and $\lambda = \lambda_2$.  
Let us focus on a specific column of $H$, denoted $\hb \in \mathbb{R}^K_+$, and 
let us majorize the function $\psi(\hb)$. % = D_{\beta}\left(v|Wh\right) + \lambda \Phi(h)$.
Given any $\widetilde{\hb}\geq 0$ of the same dimension as $\hb$, we need to find a majorizer $G\big(\hb|\tilde{\hb}\big)$ such that 
\begin{enumerate}
    \item $G\big(\hb|\widetilde{\hb}\big)  \geq \psi(\hb)$ for all $\hb$, and 

    \item $G\big(\widetilde{\hb}|\widetilde{\hb}\big)  = \psi\big(\widetilde{\hb}\big)$.
\end{enumerate}
%Now, let us provide a majorizer $G\big(\hb|\widetilde{\hb}\big)$ for $\psi(\hb)$ 
This can be done by majorizing $D_{\beta}(\vb|W\hb)$ and $\Phi(\hb)$ separately: 
\begin{itemize}
%\item The first term $D_{\beta}\big(v|Wh\right)$ is upper bounded using decomposition of $d_{\beta}$ presented in  Appendix~\ref{convconcacm}. It follows the methodology introduced in \cite{Fevotte_betadiv} to upper bound the convex and the concave terms. It is given by  
\item The first term $D_{\beta}(\vb|W\hb)=\sum_{f=1}^F d_{\beta}(v_f|(W\hb)_f)$ is upper bounded following the methodology introduced in \cite{Fevotte_betadiv}, \ji{which consists in applying a convex-concave procedure \cite{Yuille03} to $d_{\beta}$}, as presented in Appendix~\ref{convconcacm}. The resulting upper bound is given by
%
\begin{equation}
\label{eqn:auxbeta}
d_{\beta}(v_f|(W\hb)_f) \leq
\sum_{k=1}^K \frac{w_{fk}\widetilde{h}_k}{\widetilde{v}_f}\widecheck{d} \left( v_f |  \widetilde{v}_f \frac{h_k}{\widetilde{h}_k} \right)
+ \widehat{d}'\big(v_f|\widetilde{v}_f\big) \sum_{k=1}^K w_{fk} \big(h_k - \widetilde{h}_k\big)
+ \widehat{d}\big(v_f | \widetilde{v}_f\big), 
\end{equation}
where $\widetilde{v}_f = \big(W \widetilde{\hb}\big)_f$, and $\widehat{d}$ and $\widecheck{d}$ are the concave and convex parts of $d$, respectively. %\ngc{C'est correct?} 

\item For the second term $\Phi(\hb)$, we will rely on the following assumption for $\Phi$. 
\begin{assumption} \label{ass:phi}
The function 
$\Phi : \mathbb{R}^K_+ \mapsto \mathbb{R}$ %_\ngi{+}$
\jibis{is lower-bounded, and} it is either concave or has an $L$-Lipschitz continuous gradient. 
\end{assumption}
Let us consider the two cases separately:
\begin{enumerate}
    \item If $\Phi$ is concave, an upper approximation can be obtained using the first-order Taylor approximation of $\Phi$ at $\widetilde{\hb}$: 
%
\begin{equation}
\label{eq:concave_case}
\Phi(\hb)\leq\Phi\big(\widetilde{\hb}\big)+\left\langle\nabla\Phi\big(\widetilde{\hb}\big),\hb-\widetilde{\hb}\right\rangle . 
\end{equation}
%
Moreover,
\begin{equation}
\label{eq:geq0}
\nabla\Phi\big(\widetilde{\hb}\big) \geq 0,
\end{equation}
otherwise we would have $\lim_{y\rightarrow\infty}\Phi\big(\widetilde{\hb}+y\eb_j\big)=-\infty$ because of the concavity of $\Phi$, where $\eb_j$ is the $j$th unit vector. This would contradict the \jibis{fact that $\Phi$ is bounded from below.} %nonnegativity of $\Phi$. %\ngc{Où a-t-on supposé que $\Phi$ est nonnégatif? Mhmh... cela est-il le cas de fonctions concaves intéressantes? On a quoi en tête comme type de fonction à part du linéaire ($\ell_1$ penalty) en fait? J'avoue ne pas y avoir réfléchis avant.}   
%\ngc{Why is this important? Il faudrait expliquer.} 
\ngi{Examples of such penalty functions include \jibis{sparsity-promoting regularizers} $\Phi(\hb) = \| \hb \|_p^p =  \sum_k \hb_k^p$ for $0 < p \leq 1$ since $\hb \geq 0$.} %that promote the sparsity of $\hb$.}   

\item If $\Phi$ has an $L$-Lipschitz continuous gradient, we have: 
%
\begin{equation}
\label{eq:Lipschtiz_case}  
\Phi(\hb)\leq\Phi\big(\widetilde{\hb}\big)+\left\langle\nabla\Phi\big(\widetilde{\hb}\big),\hb-\widetilde{\hb}\right\rangle+\frac{L}2\big\|\hb-\widetilde{\hb}\big\|^2,
\end{equation}
%
for some constant $L > 0$, according to the descent lemma~\cite{Bertsekas99}. %\ngc{don't we need convexity here?}
\jibis{Examples of such penalty functions include any smooth convex functions;} \ngi{for example any quadratic penalty, such as   $||A \hb - b||_2^2$ for some matrix $A$ and vector $b$ in which case $L = \sigma_1(A)^2$.} 

%the \emph{minimum-volume} regularizer $\text{vol}(W)=\logdet(W^{T}W+\delta I)$ with $\delta>0$ (see \cite{9084229} and Section~\ref{sec_minvolKLNMF}).}
%\jibis{Section~\ref{sec_minvolKLNMF}, ça serait bien d'indiquer ce que vaut $L$. Logiquement, ce $L$ intervient dans l'algorithme, ce qu'on ne voit pas explicitement dans la Section~\ref{sec_minvolKLNMF}}
 

%\ngc{Je ne comprends pas le but de cette phrase ni ce que cela facilite... Pour $L=0$, la pénalité est linéaire et donc concave effectivement mais c'est un cas assez particulier...} 

\end{enumerate}

Interestingly \eqref{eq:concave_case} is a special case of  \eqref{eq:Lipschtiz_case} by taking $L=0$. This allows us to tackle these two classes of penalty functions in an unified way in what follows. Note that the result given by equation~\eqref{eq:geq0} is used further for the proof of Proposition~\ref{prop:mingmu} and is only valid for the special case $L=0$.

\end{itemize}


%\ngc{Par contre, on a pas $\nabla\Phi\big(\widetilde{\yb}\big) \geq 0$ pour le cas Lipschitz, non?-> en effet mais le résultat n'est utilisé plus tard que pour un cas particulier où L=0} 

\ji{For each column $\hb$ of $H$, a majorizer $G\big(\hb|\widetilde{\hb}\big)$ of $\psi(\hb)$ is obtained by combining \eqref{eqn:auxbeta} and \eqref{eq:Lipschtiz_case}. Finally, according to~\eqref{eq:psi(H)}, we obtain a majorizer $G\big(H|\widetilde{H}\big)$ for $\psi(H)$ as a sum of column-wise majorizers. The result is obviously separable into a sum of $K\times N$ component-wise majorizers, up to an additive constant:
%
\begin{equation}
%\label{eq:G}
G\big(H|\widetilde{H}\big) 
= \sum_{n=1}^N\sum_{k=1}^K g\big(h_{kn}|\widetilde{\hb}_n\big) + C\big(\widetilde{H}\big),
\end{equation}
where
\begin{align}
\label{eq:Gkn}
g\big(h_{kn}|\widetilde{\hb}_n\big) &= \sum_{f=1}^F \frac{w_{fk}\widetilde{h}_{kn}}{\widetilde{v}_{fn}}\widecheck{d} \left( v_{fn} |  \widetilde{v}_{fn} \frac{h_{kn}}{\widetilde{h}_{kn}} \right)
+ a h_{kn}^2 + p_{kn} h_{kn},
\\
C\big(\widetilde{H}\big) &= \sum_{n=1}^N\sum_{f=1}^F\left(\widehat{d}\big(v_{fn} | \widetilde{v}_{fn}\big)
- \sum_{k=1}^K\widehat{d}'\big(v_{fn}|\widetilde{v}_{fn}\big) w_{fk} \widetilde{h}_{kn}\right),
\notag
\end{align}
with $a=\lambda\frac{L}{2}$ and
\begin{equation*}
p_{kn}=\sum_{f=1}^F w_{fk}\widehat{d}'\big(v_{fn}|\widetilde{v}_{fn}\big) +\lambda\left(\frac{\partial \Phi}{\partial h_{kn}}\big(\widetilde{\hb}_n\big)- L\widetilde{h}_{kn}\right).
\end{equation*}
}
%Finally, it is important to note that the majorizer $G(h|\widetilde{h})$ of $\psi(h)$, obtained  by combining \eqref{eqn:auxbeta} and \eqref{eq:Lipschtiz_case}, is separable, that is, it can be written in the form 
%\[
%G(h|\widetilde{h}) 
%= \sum_{k=1}^K G_k(h_k|\widetilde{h}_k),
%\] 
%see~\eqref{eq:gj} in the next section for the expression of $G_k$.
This will allow us to minimize the majorizer under the equality constraints efficiently, as presented in the next section.  



\subsection{Dealing with equality constraints via Lagrange dual variables}  \label{sec:lagrange} 

In the previous section, we derived a majorizer for $\psi(H)$, $G\big(H|\widetilde{H}\big)$, which is separable in each entry of $H$. Without the equality constraints, we could then compute closed-form solutions to univariate problems to minimize $G\big(H|\tilde{H}\big)$ to obtain the standard MU for NMF as in~\cite{Fevotte_betadiv}. 

However, in problem~\eqref{eq:betaNMFmodelH}, the entries of $H$ in the subsets $\mathcal{B}_j$ are not independent as they are linked with the equality constraints $\gammab_j^{T} H ( \mathcal{B}_{j})=c_j$ for $j = 1,2,\dots,J$. 
In fact, to minimize the majorizer under the equality constraints, we need to solve 
%
\begin{equation}
\label{eq:betaNMFmodelHmajor}
\underset{H\in \mathbb{R}^{K \times N}_+}{\min}
 G\big(H|\widetilde{H}\big) 
\quad  \text{ such that } \quad 
\gammab_j^{T} H (\mathcal{B}_{j})=c_j \text{ for } 1\leq j \leq J. 
\end{equation} 
%
The variables in different sets $\mathcal{B}_j$ can be optimized independently, as they do not interact in the majorizer nor in the constraints. Note that, for the entries of $H$ that do not appear in any constraints, the standard MU~\cite{Fevotte_betadiv} can be used. 
For simplicity, let us fix $j$ and 
denote $\mathcal{B}=\mathcal{B}_j$, $L = |\mathcal{B}|$, 
$\yb = H(\mathcal{B}) \in \mathbb{R}^{L}_{+}$, $\gammab = \gammab_j \in \mathbb{R}^{L}_{++}$, 
and $c = c_j > 0$.  
The problems we need to solve have the form 
\begin{equation}
\label{eq:minG}
\min_{\yb \in \Yc} G\big(\yb | \widetilde{H} \big), 
\end{equation} 
where $\Yc=\left\{\yb \in \mathbb{R}^{L}_+ \ | \ \gammab^T\yb=c \right\}$
\ji{and
\begin{equation}
\label{eq:Gy}
G\big(\yb | \widetilde{H}\big)=\sum_{(k,n)\in \mathcal{B}}g\big(h_{kn}|\widetilde{\hb}_n\big),
\end{equation} 
where the component-wise majorizers $g\big(h_{kn}|\widetilde{\hb}_n\big)$ are defined by~\eqref{eq:Gkn}. Using a more convenient notation, let us rewrite~\eqref{eq:Gy} as $G\big(\yb | \widetilde{H}\big)=\sum_{\ell=1}^L g\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$, where $n(\ell)$ is the first element of any pair $\ell\in\mathcal{B}$, while $k(\ell)$ will denote the second element.}
%
%Recall that $G(\yb | \widetilde{\yb} )$ is separable, that is, 
%$$
%G(\yb|\widetilde{\yb}) 
%= \sum_{\ell = 1}^L g(y_\ell|\widetilde{\yb}) + C,
%$$
%where $C$ is a constant, and each component $g$ is given by: 
%\begin{align}
%g(y_\ell|\widetilde{\yb})&=\sum_{f=1}^F \frac{w_{fk(\ell)}\widetilde{\yb}_\ell}
%{\widetilde{v}_f}\widecheck{d} \big( v_f | \widetilde{v}_f \frac{y_\ell}{\widetilde{y}_\ell} \big) + a y_\ell^2 + p_\ell y_\ell,
%\label{eq:gj}
%\end{align}
%%
%\ngc{J'ai changé $b$ par $p$ car je l'utilisais pour les contraintes linéaires en $W$; cf. (2)}
%with $a=\lambda\frac{L}{2}$, 
%%
%\begin{equation}
%\label{eq:pell}
%p_\ell=\sum_{f=1}^F w_{fk(\ell)}\widehat{d}'(v_f|\widetilde{v}_f) +\lambda\big(\frac{\partial \Phi}{\partial y_\ell}(\widetilde{\yb})- L\widetilde{\hb}_{n(\ell)\big), 
%\end{equation}
%and the constants $w_{fk(\ell)}$ correspond to entries of $W$ and are assumed to be positive. \ngc{Il faudrait mieux les définir, je suppose que $z$ peut être construit à partir de $W$, mais ce serait intéressant d'écrire la formule explicitement.}    
%
%In order to solve \eqref{eq:minF} using an iterative majorization-minimization scheme, let us consider the constrained problem
%\begin{equation}
%\label{eq:minG}
%\min_{\yb\in \Yc} G(\yb|\widetilde{\yb}).
%\end{equation}
The corresponding Lagrangian function reads
\ji{
\begin{equation}
\label{eq:Gmuy}
    G^\mu\big(\yb|\widetilde{H}\big)  
    = G\big(\yb|\widetilde{H}\big)-\mu(\gammab^T\yb-c) 
    = \mu c + C\big(\widetilde{H}\big) + \sum_{\ell=1}^L g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big), 
\end{equation}
%\ngc{Faire attention avec les sommes indicées: cela peut prêter à confusion. Je préfère 
%$\mu c + C + \sum_{\ell=1}^L g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$.} 
where
%---------------------------
\begin{align}
g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)&=g\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)-\mu \gamma_\ell\,y_\ell\notag\\
&= \sum_{f=1}^F \frac{w_{fk(\ell)}\widetilde{y}_\ell}{\widetilde{v}_{fn(\ell)}}\widecheck{d} \left( v_{fn(\ell)} |  \widetilde{v}_{fn(\ell)} \frac{y_\ell}{\widetilde{y}_\ell} \right)
+ a y_\ell^2 + (p_\ell-\mu \gamma_\ell) y_\ell,
\label{eq:gmu}
\\
p_\ell&=\sum_{f=1}^F w_{fk(\ell)}\widehat{d}'\big(v_{fn(\ell)}|\widetilde{v}_{fn(\ell)}\big) +\lambda\left(\frac{\partial \Phi}{\partial y_\ell}\big(\widetilde{\hb}_{n(\ell)}\big)- L\widetilde{y}_\ell\right), 
\label{eq:pell}
\end{align}
}
and $\mu\in\mathbb{R}$.
Note that $G^\mu$ is separable, as is $G$, because the term $\gammab^T \yb$ is linear. 
%for any fixed value for $\mu$, $G^{\mu}$ \eqref{eq:Gmuy} is a separable approximation of the Lagrangian function $\Psi(\yb)-\mu(\gammab^T\yb-c)$.

Assume for now that the Lagrangian multiplier $\mu$ is known, and let us minimize $G^\mu\big(\yb|\widetilde{H}\big)$ on $(0,\infty)^L$. 
Such a problem is separable under the form of $L$ subproblems, consisting in minimizing univariate functions  $g^\mu\big(\cdot|\widetilde{\hb}_{n(\ell)}\big)$ separately over $(0,\infty)$. We now show in Proposition~\ref{prop:mingmu} that, under mild conditions, each subproblem admits a unique solution over $(0,\infty)$. %Let us emphasise the fact that in Proposition~\ref{prop:mingmu}, we assume that the optimal value for $\mu$ is known. 
%to be minimized on $y\in(0,\infty)$, where $\mu\in\mathbb{R}$.
%
%---------------------------
\begin{proposition}
\label{prop:mingmu}
%\ngc{Je pense que pour cette proposition, il faut considérer un seul $\ell$: j'ai modifié, please check :-)}
Let $\ell \in \{1,2,\dots,L\}$. 
Assume that $\beta<2$ and $\widetilde{y}_\ell,v_{fn(\ell)},w_{fk(\ell)}>0$ for all $f$.
%\ngc{Vérifier les indices... Faut-il vraiment que $V>0$? Cela parait restrictif...}
Moreover, if $\beta\leq1$ and $a=0$, assume that $\mu<\frac{p_\ell}{\gamma_\ell}$. 
Then there exists a unique minimizer $y_\ell^\star(\mu)$ of $g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ in $(0,\infty)$.  
\end{proposition}
%---------------------------

%
\begin{proof}
According to Proposition~\ref{prop:approxdbeta} (see Appendix~\ref{convconcacm}), each $g^\mu$ is $C^\infty$ and strictly convex on $(0,\infty)$, so its infimum is uniquely attained in the closure of $(0,\infty)$. We have to prove that it is neither reached at $0$ nor at $\infty$.

On the one hand, \ji{from \eqref{eq:gmu}, we have 
%
\begin{equation}
\label{eqgmu'}
(g^\mu)'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=\sum_{f=1}^F w_{fk(\ell)}\widecheck{d}' \left( v_{fn(\ell)} | \widetilde{v}_{fn(\ell)}\frac{y_\ell}{\widetilde{y}_\ell} \right) +2a y_\ell + p_\ell -\gamma_\ell\mu
\end{equation}
}%
and, for any $\beta<2$ and any $x>0$,
%
\begin{equation}
\label{eq:d'0}
\lim_{y\rightarrow0^+}\widecheck{d}'(x|y)=-\infty,\\
\end{equation}
%
so $\lim_{y_\ell\rightarrow0^+}(g^\mu)'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=-\infty$, which ensures that the infimum is not reached at $0$.
%\ji{This would not apply to the case $\beta\geq2$. Things are probably OK then if $\lambda=0$, but I have decided to discard the case $\beta\geq2$ for the sake of coherence, and because it is not of great interest from the application viewpoint. This could maybe deserve a comment somewhere (but we should first check the calculations when $\beta\geq2$).}

On the other hand,
%
\begin{equation}
\lim_{y\rightarrow\infty}\widecheck{d}'(x|y)=\begin{cases}0&\text{if } \beta\leq1,\\\infty&\text{otherwise.}\end{cases}
\label{eq:d'inty}
\end{equation}
%
According to \eqref{eqgmu'} and \eqref{eq:d'inty}, the distinction must be made between two cases:
%
\begin{itemize}
\item If $a>0$ or $\beta\in(1,2)$: $\lim_{y_\ell\rightarrow\infty}(g^\mu)'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=\infty$, so the infimum is reached at a finite value of $y_\ell$.
\item If $a=0$ and $\beta\leq1$: $\lim_{y_\ell\rightarrow\infty}(g^\mu)'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=p_\ell -\gamma_\ell\mu$, so the same conclusion holds if and only if $\mu<\frac{p_\ell}{\gamma_\ell}$. 
\end{itemize}
\end{proof}
We just proved that, under mild conditions, each $g^\mu$ has a unique minimizer over $(0,\infty)$.
%\ngc{Discuter la condition $\mu<\frac{p_\ell}{\gamma_\ell}$?} 
However we assumed that the value of $\mu$ is fixed.  
Now given $\yb^\star(\mu)=\big[y_1^\star(\mu),\ldots,y_L^\star(\mu)\big]^T$, let us show 
that the solution to $\gammab^T \yb^\star(\mu) =c$ is unique. The corresponding value of $\mu$, which we denote  $\mu^\star$, provides  the minimizer $\yb^\star(\mu^\star)$ of $G^\mu(\yb|\widetilde{H})$ that satisfies the linear constraint $\gammab^T\yb^\star(\mu^\star)=c$. \ji{Moreover, $\mu^\star$ naturally fulfills $\mu^\star<\frac{p_\ell}{\gamma_\ell}$ for all $\ell$ when $\beta\leq1$ and $a=0$, as required in Proposition~\ref{prop:mingmu}.}
%Finally, we prove that $\mu^\star$ is unique on some specific interval under mild conditions. 
%\sout{further}
%Let us remark that, at this stage, $\yb^\star$ is a vector function of $\mu$.
%
%---------------------------
\begin{proposition}
\label{prop:mu_unicity}
Assume that $\beta<2$ and $\widetilde{y}_\ell, v_{fn(\ell)},w_{fk(\ell)}>0$ for all $\ell,f$, %\ngc{Vérifier les indices}
%and let $y_\ell^\star(\mu)$ be the unique minimizer of  $g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ in $(0,\infty)$ as defined in Proposition~\ref{prop:mingmu}, for $\ell=1,2,\dots,L$. %\ngc{Ne doit-on pas indiquer les conditions sur $\mu$ comme dans la Proposition 1: $\mu < \min_{\ell} \frac{c_\ell}{\gammab_l}$ when $\beta \le 1$ et $a=0$?} 
%=(y_1^\star,\ldots,y_P^\star)^T$.  
Then the scalar equation $\gammab^T \yb^\star(\mu) =c$ in the variable $\mu$ admits a unique solution $\mu^\star$ in $(-\infty,t)$, where
$$
t=\begin{cases}\ji{\min_\ell \frac{p_\ell}{\gamma_\ell}}\geq0&\text{if $\beta\leq1$ and $a=0$},\\\infty&\text{otherwise,}\end{cases}
$$
such that $\yb^\star(\mu^\star)$ is the unique solution to problem~\eqref{eq:minG}.
\end{proposition}
%---------------------------
\begin{proof}
Under the conditions of Proposition~\ref{prop:mingmu}, $g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ has a unique minmizer $y^\star_\ell(\mu)$ for each $j$.  
%\ngc{A rephraser. Veux-tu dire que: 
%According to Proposition~\ref{prop:mingmu}, $g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ has a unique minmizer for each $j$, which we denote $y^\star_\ell$.} 
By the first-order optimality condition, $y^\star_\ell(\mu)$ is a solution of $(g^\mu)'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=0$ or equivalently, by \eqref{eqgmu'}, a solution of $\gamma_\ell^{-1}g'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=\mu$ over $(0,\infty)$ where 
%
\begin{equation}
\label{eq:g'}
\gamma_\ell^{-1}g'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=\gamma_\ell^{-1}\sum_{f=1}^F w_{fk(\ell)}\widecheck{d}' \left( v_{fn(\ell)} | \widetilde{v}_{fn(\ell)} \frac{y_\ell}{\widetilde{y}_\ell} \right) +2 \frac{a_\ell}{\gamma_\ell}y_\ell + \frac{p_\ell}{\gamma_\ell}
\end{equation}
%
is strictly increasing on $(0,\infty)$ (since $g$ is strictly convex) and one-to-one from $(0,\infty)$ to an open interval
$T_\ell=(t^-_\ell,t^+_\ell)$ where
%
\begin{align}
t^-_\ell&=\lim_{y_\ell\rightarrow0}g'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=-\infty,\\
t^+_\ell&=\lim_{y_\ell\rightarrow\infty}g'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)
=\begin{cases}\frac{p_\ell}{\gamma_\ell}&\text{if $\beta\leq1$ and $a=0$,}\\\infty&\text{otherwise.}\end{cases}
\end{align}
%
Moreover, $p_\ell\geq0$ if $a=0$ (then $L=0$) and $\beta\leq1$ according to~\eqref{eq:geq0} and \eqref{eq:pell}.
As a consequence, $\gamma_\ell^{-1}g'(y_\ell^\star|\widetilde{y}_\ell)=\mu$ is equivalent to
\begin{equation}
\label{eq:yhat}
y_\ell^\star = \big(g'\big)^{-1}(\gamma_\ell\mu),
\end{equation}
where $\mu\in T_\ell$ and $\big(g'\big)^{-1}$ denotes the inverse function of $g'$.

Coming back to the multivariate problem~\eqref{eq:minG}, we must find a value $\mu^\star$ of the Lagrangian multiplier such that the constraint $\gammab^T\yb^\star(\mu)=c$ is satisfied. Given~\eqref{eq:yhat}, $\mu^\star$ is a solution of
%
\begin{equation}
\label{eq:muhat}
\sum_{\ell=1}^L \gamma_\ell\big(g'\big)^{-1}(\gamma_\ell\mu)=c.
\end{equation}
%
Each $g'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ being strictly increasing on $(0,\infty)$, $(g')^{-1}(\gamma_\ell\mu)$ is also strictly increasing (from $T_\ell$ to $(0,\infty)$), this is a direct consequence of $(f^{-1})'=\frac1{f' \circ f^{-1}}$ where $f$ is any strictly increasing function on some interval. Finally $\sum_{\ell=1}^L \gamma_\ell(g')^{-1}(\gamma_\ell\mu)$ is strictly increasing from $\cap_{j=1}^J T_\ell=(-\infty,t)$ to $(0,\infty)$, with $t\geq0$. Therefore, the solution $\mu^\star$ is unique. 
\end{proof}

 Proposition~\ref{prop:mu_unicity} shows that the optimal Lagrangian multiplier is the unique solution of \eqref{eq:muhat}. It is clear that finding the solution of \eqref{eq:muhat} is equivalent to finding the root of a function $r(\mu)$. We propose here-under to use a Newton-Raphson method to compute $\mu^\star$, and show that this method generates a sequence of iterates $\mu_n$ that converges towards $\mu^\star$ at a quadratic speed.

%---------------------------
\begin{proposition}
\label{NR}
Assume that $\beta<2$ and $\widetilde{y}_\ell,v_{fn(\ell)},w_{fk(\ell)}>0$ for all $\ell,f$. %\ngc{Vérifier les indices}
Let
$$
r(\mu)=\sum_{\ell=1}^L \gamma_\ell(g')^{-1}\big(\gamma_\ell\mu\big)-c
$$
for $\mu\in(-\infty,t)$, and denote $\mu^*$ the unique solution of $r(\mu)=0$. From any initial point $\mu_0\in(\mu^*,t)$, Newton-Raphson's iterates
$$
\mu_{n+1}=\mu_n-\frac{r(\mu_n)}{r'(\mu_n)}
$$
decrease towards $\mu^*$ at a quadratic speed.
\end{proposition}
\begin{proof}
We already know that $r$ is strictly increasing from $(-\infty,t)$ to $(0,\infty)$. Let us show that $r$ is also strictly convex.
According to the third item of Proposition~\ref{prop:approxdbeta} in Appendix~\ref{convconcacm}, $\widecheck{d}''(x|y)$ is completely monotonic, so it is strictly decreasing in $y$. Equivalently, $\widecheck{d}'(x|y)$ is strictly concave in $y$, and each $g'$ is also strictly concave according to~\eqref{eq:g'}. Since the inverse of a strictly increasing, strictly concave function $f$ is strictly increasing and strictly convex, which is a direct consequence of $(f^{-1})''=-\frac{f''\circ f^{-1}}{(f' \circ f^{-1})^3}$, 
then each $(g')^{-1}$ is strictly convex, and finally, $r$ is strictly convex.

For any $\mu_0\in(\mu^*,t)$, we have $r(\mu_0)>0$, so $\mu_1=\mu_0-\frac{r(\mu_0)}{r'(\mu_0)}<\mu_0$. We have also $\mu_1>\mu^*$ as a consequence of the strict convexity of $r$. By immediate recurrence, we obtain that $\mu_n$ is a decreasing series that converges towards $\mu^*$. According to \cite{Ortega70}, it converges at a quadratic speed since $|r'|$ and $|r''|$ are bounded away from 0 in $[\mu^*,\mu_0]$.
\end{proof}

At this point, we have derived an optimization framework to tackle problem~\eqref{eq:minG}. 
The optimal Lagrangian multiplier value is determined before each majorization-minimization update using a Newton-Raphson algorithm. However, such a formal solution is implementable if and only if each $y_\ell^\star(\mu)$ can be actually computed as the minimizer of $g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ in $(0,\infty)$. In some cases, computing $y_\ell^\star(\mu)$ is equivalent to extracting the roots of a polynomial of a degree smaller or equal to four, which is possible in closed form. In other cases, we have to solve a polynomial equation of degree larger than four, or even an equation that is not polynomial. Table~\ref{tab:poldeg} indicates the cases where a closed-form solution is available. 
\begin{table}[h]
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\hfill$\beta\in$     &$(-\infty,1)\setminus\{0\}$&$\{0\}$&$\{1\}$&\multicolumn{4}{|c|}{$(1,2)$}      \\
Penalization&    &   &   &$\frac54$&$\frac43$&$\frac32$&other           \\\hline
No penalization& 1 & 1  & 1  & 1        &  1       &  1       &  1           \\\hline
Concave&1&1&1&3&4&2&$\rip$\\\hline
Lipschitz continuous gradient&$\rip$&3&2&$\rip$&$\rip$&3&$\rip$\\\hline
\end{tabular}
\caption{%\ji{Est-ce que nous devrions ajouter une ligne "no penalization", qui correspondrait aus cas traite en Sous-section~\ref{betanmf_disjointconstraint} ? Dans ce cas, sauf erreur, le degre est 1 dans chaque cas. } \ngc{Oui, tout à fait d'accord, et cela permet de motiver pq on considère ce cas dans la section 2.3!} 
The cases where \eqref{eq:yhat} can be computed in closed form are indicated by the degree of the corresponding polynomial equation, otherwise the symbol $\rip$ is used.}
%\ji{(I have maintained $\beta\geq2$ here, we will need to decide what to do with this case.)}
\label{tab:poldeg}
\end{table}





% This section is organized as follows:
% \begin{itemize}
%     \item Subsection~\ref{convconcacm} presents the convexity, concavity and complete monotonicity properties of a convex-concave decomposition of the discrete $\beta$-divergence that is crucial for the efficiency of the general framework and the derived algorithms,
%     \item Subsection~\ref{prob_algo_generalframe} firstly introduces the general form of a multivariate minimization problem involving a finite sum of discrete $\beta$-divergence terms under a linear constraint with a possible penalty term in the objective function. This penalty term can be either concave or Lipschitz smooth. % with constant $L$.
%     Secondly we present the general framework to tackle such optimization problems relying on the construction at the current iterate of an auxiliary function for the Lagrangian that is minimized in closed-form. Thirdly, we present the rate of convergence for the Newton-Raphson method used to compute the optimal Lagrangian multipliers at each iteration of the optimization framework.
%     \item Subsection~\ref{betanmf_disjointconstraint} presents the algorithm obtained from the general framework in the case of nonpenalized $\beta$-NMF under disjoint linear equality constraints.
% \end{itemize}

% \subsection{Convexity, concavity and complete monotonicity for a convex-concave decomposition of the discrete $\beta$-divergence}\label{convconcacm}
% The discrete $\beta$-divergence can always be expressed as the sum of convex, concave, and constant terms. In Table~\ref{tab:decompbetadiv} we introduce a convex-concave decomposition of the $\beta$-divergence which slightly differ from the one given in \cite[Table\,1]{Fevotte_betadiv} (by the fact that ours contains no constant term $\widebar{d}$) as follows:
% % \[
% % \widecheck{d}(x|y)=  \begin{cases}
% % \frac{1}{1-\beta} x \,y^{\beta -1}
% %       &\text{for}\quad \beta<1, \beta\neq0,  \\
% % \frac{x}{y}
% %       &\text{for}\quad \beta=0,   \\
% % %y-x-x\log \frac{y}{x}           
% % -x\log y           
% %       &\text{for}\quad \beta=1,  \\
% % \frac1{\beta}y^{\beta}-\frac1{\beta-1} xy^{\beta-1} &\text{for} \quad \beta \in \left(1,2\right), \\
% % \frac{1}{\beta} y^{\beta}
% %       &\text{for}\quad \beta\geq2,
% %   \end{cases}
% % \]
% % and
% % \[
% % \widehat{d}(x|y)= \begin{cases}
% %  \frac{1}{\beta}y^{\beta}-\frac{1}{\beta\,(1-\beta)} x^{\beta}
% %       &\text{for}\quad \beta<1, \beta\neq0,  \\
% % \log\frac{y}{x} - 1
% %       &\text{for}\quad \beta=0,   \\
% % %y-x-x\log \frac{y}{x}           
% % y + x\, \log x - x          
% %       &\text{for}\quad \beta=1,  \\
% % \frac{1}{\beta\,(\beta-1)} x^{\beta} &\text{for} \quad \beta \in \left(1,2\right), \\
% % -\frac{1}{\beta-1} x \,y^{\beta -1}+\frac{1}{\beta\,(\beta-1)} x^{\beta}
% %       &\text{for}\quad \beta\geq2,
% %   \end{cases}
% % \]
% % \ji{a remplacer peut-etre par une table a 5 lignes, 2 colonnes}



% \begin{table}[h]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \hfill$\beta$     &$(-\infty,1)\setminus\{0\}$&$0$&$1$&$(1,2)$ &   $[2,+\infty)$    \\
% Decomposition $d_{\beta}(x|y)$&  &   &  &    &   \\\hline
% $\widecheck{d}(x|y)$& $\frac{1}{1-\beta} x \,y^{\beta -1}$    & $\frac{x}{y}$  & $-x\log y$  &  $\frac1{\beta}y^{\beta}-\frac1{\beta-1} xy^{\beta-1}$  & $\frac{1}{\beta} y^{\beta}$  \\\hline
% $\widehat{d}(x|y)$&$ \frac{1}{\beta}y^{\beta}-\frac{1}{\beta\,(1-\beta)} x^{\beta}$&$\log\frac{y}{x} - 1$&$y + x\, \log x - x  $&$\frac{1}{\beta\,(\beta-1)} x^{\beta}$&$-\frac{1}{\beta-1} x \,y^{\beta -1}+\frac{1}{\beta\,(\beta-1)} x^{\beta}$\\\hline
% \end{tabular}
% }
% \caption{
% Proposed concave-convex decomposition of the discrete $\beta$-divergence.}
% %\ji{(I have maintained $\beta\geq2$ here, we will need to decide what to do with this case.)}
% \label{tab:decompbetadiv}
% \end{table}



% where $y\in(0,\infty)$, $\beta$ is real valued and $x\in(0,\infty)$, so that $d_{\beta}(x|y)=\widehat{d}(x|y)+\widecheck{d}(x|y)$. Further, $\beta$ and $x$ are considered as parameters, $d_{\beta}$, $\widehat{d}$ and $\widecheck{d}$ being handled as univariate functions of $y$.\\

% Let us now recall the definition of a complete monotonic function $f$:
% \begin{definition}
% A function $r$ is said to be completely monotonic (c.m.) on an interval $I$ if $r$ has derivatives of all orders on $I$ and $(-1)^n f^{(n)}(x)\geq0$ for $x\in I$ and $n\geq0$.
% \end{definition}
% We can now introduce the properties of concavity, convexity and monotonicity for  our convex-concave formulation of the discrete $\beta$-divergence:

% \begin{proposition} Given $\widecheck{d}(\cdot|\cdot)$ and $\widehat{d}(\cdot|\cdot)$ as defined above, we have that
% \label{prop:approxdbeta}
% \hfill
% \begin{enumerate}
% \item $\widecheck{d}(x|y)$ is $C^\infty$ and strictly convex on $(0,\infty)$ for $x>0$ and $\beta\in\mathbb{R}$;
% \item $\widehat{d}(x|y)$ is concave for $x>0$ and $\beta\in\mathbb{R}$;
% \item for all $\beta<2$, $\widecheck{d}''_{\beta}(x|y)$ and $\widehat{d}'_{\beta}(x|y)$ are c.m. 
% \end{enumerate}
% %Functions $g_1,\ldots,g_5$ are stricly convex on $(0,\infty)$. Moreover, $g_1$, $g_2$, $1-g'_3$, and $g''_4$ are completely monotonic on $(0,\infty)$.
% \end{proposition}
% \begin{proof}
% The proof is straightforward, given that $\widecheck{d}(x|y)$ and $\widehat{d}(x|y)$ linearly combine $C^\infty$ functions on $(0,\infty)$, and that in the same interval, 
% \begin{itemize}
% \item $\log y$ is strictly concave;
% \item $y^\nu$ is strictly convex for all  $\nu\in(-\infty,0)\cup(1,\infty)$, and strictly concave for all $\nu\in(0,1)$;
% \item $y^\nu$ is c.m. for all $\nu<0$.
% \end{itemize}
% \end{proof}
% According to the first two items of Proposition~\ref{prop:approxdbeta}, $\widecheck{d}$ and $\widehat{d}$ indeed yield a convex-concave decomposition of the $\beta$-divergence, which is a variant of \cite[Table\,1]{Fevotte_betadiv}. Let us remark that the successive minimization of an upper approximation of this convex-concave decomposition following the methodology presented in \cite{Fevotte_betadiv} yields to the usual multiplicative update scheme. 
% In the following subsection, we take advantage of these properties to build up a framework that enables to efficiently tackle penalized minimization problems relying on discrete $\beta$-divergence under linear constraints.








\subsection{MU for $\beta$-NMF with disjoint linear equality constraints, without penalty terms}\label{betanmf_disjointconstraint}


In this section, we derive an algorithm based on the general framework presented in the previous section to tackle the $\beta$-NMF problem under disjoint linear equality constraints in the non-penalized case, that is,  problem~\eqref{eq:betaNMFmodel} with $\lambda_1=\lambda_2=0$.
We consider this simplified case here as it allows to provide explicit MU for any value of $\beta < 2$; see the first row 'No penalization' of Table~\ref{tab:poldeg}. These updates  satisfy the constraints after each update of $W$ or $H$, and monotonically decrease the objective function $D_{\beta}\left(V|WH\right)$. 
% \subsubsection{Algorithm for disjoint-constrained $\beta$-NMF}\label{sec_algodisjointConstrainedbetaNMF} 

Let us then consider the subproblem of \eqref{eq:betaNMFmodel} over $H$ when $W$ is fixed and with $\lambda_2=0$, that is,  
%
\begin{equation}\label{eq:subprobleminW}
 \underset{H\in \mathbb{R}^{K \times N}_+}{\min}
 D_{\beta}\left(V|WH\right) 
\quad \text{such that} \quad \gammab_j^{T} H (\mathcal{B}_{j})=c_j \text{ for } 1\leq j \leq J.
\end{equation}
%\ngc{Ce n'est pas très naturel de faire tout en $W$ ici, alors qu'on a fait $H$ avant... ce n'est pas grave, mais juste un peu 'confusing'. Surtout que dans la section suivante, on est de retour sur $H$ avec le showcase 1... Cela vaudrait la peine de changer, mais ce n'est pas une priorité.}  
%In the following we derive MU for $H$ that decrease the objective in \eqref{eq:subprobleminW}. 
Let us follow the framework presented above. First, an auxiliary function, which we denote $G(H| \widetilde{H})$, is constructed at the current iterate $\widetilde{H}$ so that it majorizes the objective for all $H$ and is defined as follows:
%
\begin{equation}
\label{eq:G}
\begin{aligned}
G\left(H|\widetilde{H}\right)&=\sum_{f,n}\left[\sum_{k} \frac{W_{fk}\widetilde{H}_{kn}}{\widetilde{V}_{fn}}\widecheck{d}\left(V_{fn}|\widetilde{V}_{fn}\frac{H_{kn}}{\widetilde{H}_{kn}}\right)\right] \\
&+\left[\widehat{d}'\big(V_{fn}|\widetilde{V}_{fn}\big)\sum_{k}W_{fk}\big(H_{kn}-\widetilde{H}_{kn}\big)+\widehat{d}\big(V_{fn}|\widetilde{V}_{fn}\big) \right], 
\end{aligned}
\end{equation} 
%\ngc{Give a bit more details: convex-concave-constant decomposition, etc.}
where $\widecheck{d}(.|.)$ and $\widehat{d}(.|.)$ are the ones defined in Appendix~\ref{convconcacm}.
Second, we need to minimize $G\left(H|\widetilde{H}\right)$ 
%$D_{\beta}\left(V|WH\right)$ over $\mathbb{R}_{+}^{K \times N}$ with the auxiliary function of $G$, 
while imposing the set of linear constraints $\gammab_j^{T} H (\mathcal{B}_{j})=c_j$. The Lagrangian function of $G$ is given by 
\begin{equation}\label{eq:Gmu}
\begin{aligned}
G^{\mu}(H|\widetilde{H})= G(H |\widetilde{H} )-\sum_{j}^{J} \left[\mu_{j} \left( \gammab_j^{T} H (\mathcal{B}_{j})-c_j\right) \right], 
\end{aligned}
\end{equation} 
 where $\mu_{j}$ are the Lagrange multipliers associated to each linear constraint $\gammab_j^{T} H (\mathcal{B}_{j})=c_j$. We observe that $G^{\mu}$ in~\eqref{eq:Gmu} is a separable majorizer in the variables $H$ of the Lagrangian function $D_{\beta}\left(V|WH\right) - \sum_{j}^{J} \left[ \mu_{j} \left( \gammab_j^{T} H (\mathcal{B}_{j})-c_j\right) \right]$. Due to the disjoitness of each subset of variables $\mathcal{B}_{j}$ \eqref{eq:Gmu}, we only consider the optimization over one specific subset $\mathcal{B}_{j}$. 
The minimizer \eqref{eq:yhat} of $G^{\mu}(H\left( \mathcal{B}_{j} \right)|\widetilde{H}\left( \mathcal{B}_{j} \right))$ has the following component-wise expression:
\begin{equation}\label{eq:updateW}
\begin{aligned}
H^\star\left(\mathcal{B}_{j}\right)=\widetilde{H}\left(\mathcal{B}_{j}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{j}\right) \right]}{\left[ D\left(\mathcal{B}_{j}\right) - \mu_{j}  \gammab_j \right]} \right)^{.\left( \gamma \left( \beta \right)\right)} , 
\end{aligned}
\end{equation}  
where $C=W^{T} \left( \left( WH \right)^{.\left( \beta-2 \right) } \odot V \right)$, $D=W^{T}\left( WH\right)^{.\left( \beta-1 \right) }$, $\gamma(\beta)=\frac{1}{2-\beta}$ for $\beta < 1$, $\gamma(\beta)=1$ for $\beta \in \left[1,2\right]$ and $\gamma(\beta)=\frac{1}{\beta-1}$ for $\beta >2$ \cite[Table 2]{Fevotte_betadiv}, $A \odot B$ 
(resp.\@ $\frac{\left[ A \right]}{\left[ B \right]}$) is the Hadamard product (resp.\@ division) between $A$ and $B$,  
$A^{.(\alpha)}$ is the element-wise $\alpha$ exponent of $A$. 
%\ngc{Tu ne définirais pas dès le début $f_i = a_i^T W\left(\mathcal{K}_{i}\right) + b_i$, cela simplifierai tout ceci et serait plus concret.} 
Finally, we need now to find the optimal value for $\mu_j$, denoted $\mu_j^\star$,  wihch is the solution of $\gamma_j^{T} H^\star \left( \mathcal{B}_{j} \right)=c_j$. It requires to finding the root of the function 
\begin{equation} \label{eq:fmulincstr}
r_j(\mu_j)=\sum_{\ell=1}^{L} \gamma_{j,\ell} \left[ \widetilde{H}\left(\mathcal{B}_{j}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{j}\right) \right]}{\left[ D\left(\mathcal{B}_{j}\right) - \mu_{j}  \gamma_j \right]} \right)^{.\left( \gamma \left( \beta \right)\right)} \right]_{\ell}  -c_j , 
\end{equation}
where $\left[A\right]_{\ell}$ denotes the $\ell$-th entry of expression $A$. Proposition~\ref{prop:mu_unicity} shows that $\mu_j^\star$ is unique on some interval $\left(-\infty, t \right)$. 
Indeed, $r_j(\mu_j)$ is a finite sum of elementary rationale functions of $\mu_j$ and each of them is an increasing, convex function in $\mu_{j}$ over $\left(-\infty, t_{\ell},\right)$ with  $t_{\ell}=\frac{D_{\ell}\left(\mathcal{B}_{j}\right)}{\gamma_{j,\ell}}$ for all $\beta$. It is even completely monotone for all $\beta$ in $\left(-\infty, t_{\ell}\right)$ because $\gamma\left( \beta \right)>0$~\cite{miller2001}. As a consequence $r_j(\mu_j)$ is also a completely monotone, convex increasing function of $\mu_{j}$ in $\left(-\infty, t \right)$, where $t=\text{min}\left( t_{\ell} \right)$. Finally, we can easily show that the function $r_j(\mu_j)$ changes of sign on the interval $\left(-\infty, t \right)$ by computing two limits at the closure of the interval. As $\mu^\star \in (-\infty,t)$, the update \eqref{eq:updateW} is nonnegative.
%\ji{Je pense qu'on peut encore raccourcir ce paragraphe en faisant reference aux propositions de la sous-section 2.2.} 
To evaluate $\mu^\star$, we use a Newton-Raphson method, with any initial point $\mu_0\in(\mu^*,t)$, with a quadratic rate of convergence as demonstrated in Proposition~\ref{NR}. 
Algorithm~\ref{consDisBetaNMF} summarizes our method to tackle~\eqref{eq:betaNMFmodel} for all the $\beta$-divergences which we refer to as disjoint-constrained $\beta$-NMF algorithm. The update for matrix $W$ can be derived in the same way, by symmetry of the problem. 


%where $\mathcal{K}$ designates the full set of variables in $W$.
%\ngc{On pourrait parler du computational cost ici, et ne plus en parler après, ou dire que c'est similaire à ce cas c-à-d que le coût est dominé par les matrix-matrix products, et par par le caclul de $\mu^*$.} 

It can be verified that the computational complexity of Algorithm~\ref{consDisBetaNMF} is asymptotically equivalent to the standard MU for $\beta$-NMF, that is, it requires $\mathcal{O}\left(FNK \right)$ operations per iteration. Indeed, the complexity is mainly driven by matrix products and, based on numerical experiments, we confirm that the Newton-Raphson shows quadratic rates of convergence as shown by Proposition~\ref{NR}. Provided that a good initial approximation is known and by imposing to compute $J+I$ roots, the average theoretical complexity is the cost of calculating $r_i(x)/r_i'(x)$ and $r_j(x)/r_j'(x)$ and the number of iterations to converge. In practice, we report that the number of iterations required for the convergence of the Newton-Raphson method is in the order of magnitude of 10 to 100 and since $\max(J,I) \ll \max(F,K,N)$ in practice, the resulting complexity is dominated by the matrix products that require $\mathcal{O}\left(FNK \right)$ operations. 
The same conclusions apply to the algorithms presented in 
Sections~\ref{sec_ssbetaNMF}, \ref{sec_minvolKLNMF} and~\ref{sec_nonlinear}. 

\algsetup{indent=2em}
\begin{algorithm}[ht!]
\caption{$\beta$-NMF with disjoint linear constraints \label{consDisBetaNMF}}
\begin{algorithmic}[1] 
\REQUIRE A matrix $V \in \mathbb{R}^{F \times N}$, 
an initialization $H \in \mathbb{R}^{K \times N}_+$ and $W  \in \mathbb{R}^{F \times K}$, 
a factorization rank $K$, 
a maximum number of iterations, maxiter, 
a value for $\beta$, and 
the linear constraints defined by 
$\mathcal{K}_{i}$, $\alphab_j$ and $b_i$ for $i=1,2,\dots,I$, and 
$\mathcal{B}_{j}$, $\gammab_j$ and $c_j$ for $j=1,2,\dots,J$.  
\ENSURE A rank-$K$ NMF $(W,H)$ of $V$ satisfying constraints in \eqref{eq:betaNMFmodel}. 
    \medskip  
\FOR{$it$ = 1 : maxiter}
    \STATE \emph{\% Update of matrix $H$} 
    \STATE $C \leftarrow W^{T}\left( \left( WH \right)^{.\left( \beta-2 \right) } \odot V \right)$
    \STATE $D \leftarrow W^{T}\left( WH\right)^{.\left( \beta-1 \right) }$
    \FOR{$j = 1 : J$}
            \STATE $\mu_{j} \leftarrow \text{root}\left( r_j(\mu_j) \right)$ \quad \emph{\% see Equation~\eqref{eq:fmulincstr} }
            \STATE $H\left(\mathcal{B}_{j}\right) \leftarrow H\left(\mathcal{B}_{j}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{j}\right) \right]}{\left[ D\left(\mathcal{B}_{j}\right) -  \mu_{j}  \gamma_j \right]} \right)^{.\left( \gamma \left( \beta \right)\right)}$
    \ENDFOR
    \STATE $\mathcal{B}_{c} = \{ (k,n) \ | 1 \leq k  \leq K, 1 \leq n \leq N \} \backslash  \left(\cup_{j}^{J} \mathcal{B}_{j} \right).$ \quad \emph{\% $\mathcal{B}_{c}$ is the complement of $\cup_{j}^{J} \mathcal{B}_{j}$  }
    
    \STATE $H\left(\mathcal{B}_{c}\right) \leftarrow H\left(\mathcal{B}_{c}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{c}\right) \right]}{\left[ D\left(\mathcal{B}_{c}\right) \right]} \right)^{.\left( \gamma \left( \beta \right)\right)}$
	\STATE \emph{\% Update of matrix $W$}
    \STATE $W$ is updated in the same way as $H$, by symmetry of the problem. 
\ENDFOR
\end{algorithmic}  
\end{algorithm} 



==> alphabet.tex <==
% Document LaTeX        GLB (25/05/94)
% Modification :        Gio (15/09/95)
%                       JI  (format Latex 2e, taille adaptative 22/03/99)
%                           (fonte blackboard 27/08/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{(necessite les packages xspace, amsmath, bbm)}
\typeout{}

\RequirePackage{amsmath}
\RequirePackage{xspace}
%\RequirePackage{bbm}
\RequirePackage{amssymb}
%\RequirePackage{bbold}
%\RequirePackage{mathbbol}
%\RequirePackage{doublestroke}

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
%\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)
\def\sbl#1{\ensuremath{\mathbb{#1}}}              % Style blackboard (necessite amssymb)

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}

% Complément intéressant...

\def\ellb{\sbmm{\ell}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}


% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}    \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}



==> arXiv v2/Chapters/1_Introduction.tex <==


Given a non-negative matrix $V \in \mathbb{R}_{+}^{F \times N}$ and a factorization rank $K \ll \min(F,N)$, nonnegative matrix factorization (NMF) aims to compute two non-negative matrices, $W$ with $K$ columns and $H$ with $K$ rows, such that $V\approx WH$~\cite{lee1999learning}. 
Over the last two decades, NMF has shown to be a powerful tool for the analysis of high-dimensional data. The main reason is that NMF automatically extracts sparse and meaningful features from a set of nonnegative data vectors. NMF has been successfully used in many applications such as image processing, text mining, hyperspectral imaging, blind source separation, single-channel audio source separation, clustering and music analysis; see~\cite{gillis2014, cichocki2009nonnegative, chi2012tensors, neymeyr2018set, fu2019nonnegative, gillis2020bk} and the references therein. 

%NMF approximate each column of $V$ by a linear combination of the columns of $W$ weighted by the components of the corresponding column of $H$. 
To compute $W$ and $H$, the most standard approach is to solve the following optimization problem 
\begin{equation}\label{eq:2}
 \underset{W\in \mathbb{R}^{F \times K},H\in \mathbb{R}^{K \times N}}{\min}
 D\left(V|WH\right)  \quad  \text{ such that } \quad H \geq 0 \text{ and } W \geq 0, 
\end{equation}
where $D\left(V|WH\right)=\sum_{f,n} d(V_{fn}|[ \,WH] \,_{fn})$ with 
$d(x|y)$ a measure of distance between two scalars, 
and 
$A \geq 0$ means that the matrix $A$ is component-wise nonnegative. 
In this paper, we focus on $\beta$-NMF for which the measure of fit is the discrete $\beta$-divergence denoted $d_{\beta}(x|y)$ and defined as 
\[
d_{\beta}\left(x|y\right) = 
%\left\{  \begin{array}{lr}
  \begin{cases}
    \frac{1}{\beta \left(\beta-1\right)}   \left(x^{\beta}+\left(\beta-1\right)y^{\beta}-\beta xy^{\beta-1}\right) & \text{for} \quad \beta \in \mathbb{R} \setminus \left\{0,1\right\}, \\
    x\log\frac{x}{y}-x+y           
      &   \text{for}\quad \beta=1,  \\
    \frac{x}{y}-\log\frac{x}{y}-1  
      &  \text{for}\quad \beta=0. 
  \end{cases}
%  \end{array} \right.
\] 
For $\beta=2$, $d_2(x|y)=\frac12(x-y)^2$, so $D\left(V|WH\right)$ is the halved standard squared Euclidean distance between $V$ and $WH$, that is, 
the halved squared Frobenius norm $\frac{1}{2}\|V-WH\|_F^2$ . 
For $\beta=1$ and $\beta=0$, 
the $\beta$-divergence corresponds to the Kullback-Leibler (KL) divergence and the Itakura-Saito (IS) divergence, respectively. 
The error measure should be chosen accordingly with the distribution of the noise assumed on the data. 
The Frobenius norm assumes i.i.d.\@ Gaussian noise, KL divergence assumes a Poisson distribution, 
and the IS divergence assumes multiplicative gamma noise; see for example~\cite{fevotte2009nonnegative, dikmen2015learning, hong2020generalized} and the references therein. 
In the NMF literature, $\beta$-divergences are the most widely used objective functions. 

% \ngc{Ceci n'a rien à faire ici: à supprimer et expliquer plus tard.}
% \sout{Note that the divergence can always be expressed as the sum of a convex, concave, and constant part, such that:} 
%   \begin{equation*}
%   d_{\beta}(x|y)= \widecheck{d}_{\beta}(x|y)+\widehat{d}_{\beta}(x|y)+\widebar{d}_{\beta}(x|y),
%   \end{equation*}
% \sout{where $\widecheck{d}$ is convex function of $y$, $\widehat{d}$ is a concave function of $y$ and $\widebar{d}$ is a constant of $y$, see \cite{Fevotte_betadiv} for \ji{a possible} definition of these terms for different values of $\beta$.}

Most NMF algorithms developed to tackle~\eqref{eq:2} are based on iterative schemes that alternatively updates the factors $W$ and $H$. 
At each iteration, the minimization over one factor, $W$ or $H$, is performed with various optimization methods. 
For $\beta$-divergences, the most popular approach is to use multiplicative updates (MU) which were introduced for NMF in the seminal papers of Lee and Seung~\cite{lee1999learning, algoNMFlee}. 
In all applications we are aware of, $\beta$ is always chosen smaller than two. The reason is that, for $\beta > 2$,  $\beta$-divergences become more and more sensitive to outliers. Already for $\beta = 2$, it is well-known that the squared Frobenius norm is sensitive to outliers. However, the case $\beta = 2$ is particular because the subproblem in $W$ and $H$ are nonnegative least squares problems, that is, convex quadratic problems with Lipschitz continuous gradient. 
Therefore, highly efficient schemes exist when $\beta = 2$ that outperform the MU; for example exact block coordinate descent methods~\cite{Cichocki07HALS, gillis2012accelerated, kim2014algorithms, acc_NMF}, or fast gradient methods~\cite{guan2012nenmf, le2020inertial}. % to an optimization problem in $W$  for which highly efficient schemes can be derived, such as fast projected gradient descent methods~\cite{} 
In this paper, we focus on the case $\beta < 2$. 



In many applications, on top of the nonnegative constraints on the variables, additional constraints are needed to provide a meaningful solution. 
An instrumental example is the constraint that the entries in each column of $H$ sum to one; this is the so-called sum-to-one constraint that is crucial in blind hyperspectral unmixing; see Section~\ref{sec_ssbetaNMF}. 
Another example is a sum-to-one constraint on the columns of $W$ along with a volume regularizer on $W$. This model leads to identifiability of the factors $W$ and $H$ under mild conditions; see Section~\ref{sec_minvolKLNMF}. 
Most algorithms that deal with such equality constraints do it a posteriori with a projection onto the feasible set, or with a renormalization of the columns of $W$ and the rows of $H$ (that is, replace $W(:,k)$ and $H(k,:)$ by $\alpha_k W(:,k)$ and $H(k,:)/\alpha_k$ for some $\alpha_k > 0$),
so that their product $WH$ remains unchanged, and hence $D(V|WH)$ remains unchanged. 
Such approaches are not ideal: 
\begin{itemize}
    \item Projection requires to perform a line-search to ensure the monotonicity of the algorithm, that is, to ensure that the objective does not increase after each iteration, 
    which may be computationally heavy. 
    
    \item  Renormalization of the columns of $W$ and the rows of $H$ is only useful when each constraint applies to a column of $W$ {or} a row of $H$. 
    It is not applicable for example for the sum-to-one constraint on the columns of $H$ mentioned above. Moreover, in the presence of regularization terms in the objective function, it may destroy the monotonicity of the algorithm. 
    
\end{itemize} 
Another approach is to use parametrization. However, as far as we know, it does not guarantee the monotonicity of the algorithm; see Section~\ref{sec_ssbetaNMF} for more details.  




\paragraph{Outline and contribution} 


In this paper, we introduce a general framework to design MU for 
$\beta$-NMF with disjoint linear equality constraints, and with penalty terms in the objective function. By disjoint, we mean that each variable appears in at most one equality constraint. 
This framework, presented in Section~\ref{sec_generalframework}, does not resort to projection, renormalization, or parametrization.  
Our MU satisfy the set of constraints after each update of the variables during the optimization process, while guaranteeing that the objective function decreases monotonically. 
This framework works as follows:  
\begin{itemize}
    \item First, as for the standard MU for $\beta$-NMF, we majorize the objective function using a separable majorizer, that is, the majorizer is the sum of functions involving a single variable. 
    
    \item Second, we construct the augmented Lagrangian for the majorizer. Because the majorizer is separable, the problem can be decomposed into independent subproblems involving only variables that occur in the same equality constraint since they are  disjoint.   
    For a fixed value of the Lagrange multipliers, we prove that the solution of these subproblems are unique, under mild conditions (Proposition~\ref{prop:mingmu}). Moreover, it can be written in closed form via MU for specific values of $\beta$ and depending on the regularizer used (this is summarized in Table~\ref{tab:poldeg}). 
    
    \item Finally, we prove that, under mild conditions, there is a unique solution for the Lagrange multipliers so that the equality constraints are satisfied (Proposition~\ref{prop:mu_unicity}). This allows us to apply the Newton-Raphson method to compute the Lagrange multipliers while guaranteeing quadratic convergence (Proposition~\ref{NR}). 
    
    
\end{itemize}

We then showcase this framework on two NMF models, and show that it competes favorably with the state of the art: 
\begin{enumerate}
    \item A $\beta$-NMF model with sum-to-one constraints on the columns of $H$, which we refer to as simplex-structured $\beta$-NMF (Section~\ref{sec_ssbetaNMF}), and 
    
    \item A minimum-volume $\beta$-NMF model with sum-to-one constraints on the columns of $W$ (Section~\ref{sec_minvolKLNMF}).  
\end{enumerate} 
Finally, Section~\ref{sec_nonlinear} shows that the framework can be extended to the case of quadratic disjoints constraints, which we showcase on 
sparse $\beta$-NMF with $\ell_2$-norm constraints on the columns of $W$. 


%The paper is organized as follows. 
%In Section~\ref{sec_generalframework}, 
%we present the general framework to 
%minimize a multivariate minimization problem of the form 
%$\beta$-divergences under linear constraints. 
%we then decline the framework to tackle $\beta$-NMF with disjoint linear equality constraints, and explain how to derive MU that satisfy these constraints during the optimization procedure. 


%In , we showcase this approach on $\beta$-NMF with the sum-to-one constraints on the columns of $H$, which we refer to as simplex-structured $\beta$-NMF. 
%We show that in general, it performs significantly better than a recently proposed heuristic algorithm based on parametrization for the same model for blind hyperspectral unmixing. Moreover, it is guaranteed to decrease the objective function at each iteration.  
%In , we extend the approach to $\beta$-NMF with sum-to-one constraints on the columns of $W$ and with a minimum-volume regularizer on the columns of $W$. This model is particularly powerful since it leads to identifiable solutions under mild conditions. 
%In this more general case, we are only able to derive updates in the case $\beta = 1$. We show that our approach outperforms a recent projection-based algorithm. 
%Finally, in , we extend our method to. 

%\paragraph{Notation} 





==> arXiv v2/Chapters/2_betaNMF.tex <==
% \ngc{Je pense que cette section nécessite un ``serious facelift'' (j'utilise l'expression utilisée un jour par un reviewer).}

% \ngc{Je propose la chose suivante: 
% Avant de mettre `This section is organized as follows', il faut bien réexpliquer le contexte. On veut résoudre $\beta$-NMF avec pénalités et contraintes linéaires disjointes: donner le modèle général~\eqref{eq:betaNMFmodel} et introduire les notations. On voit ainsi directement ce qu'on veut faire/résoudre. 
% Ensuite, comme on fait de l'alterné, montrer que les sous-problèmes à résoudre ont la forme de~\eqref{eq:subprobleminW} et donc~\eqref{eq:minF}. 
% Finalement, donner la structure de la section.  
% }

% \ngc{Je le laisse retravailler cela et je relis après. J'ai mis d'autres commentaires également dans la section.}  

In this paper, we introduce a general framework to tackle $\beta$-NMF with disjoint linear equality constraints, and with penalty terms in the objective function. Let us first introduce specific notations: given a matrix $A \in \mathbb{R}^{F \times N}$ and a list of indices $\mathcal{K} \subseteq \{ (f,n) \ | \ 1 \leq f \leq F, 1 \leq n \leq N\}$, we denote by $A(\mathcal{K})$ the vector of dimension $|\mathcal{K}|$ whose entries are the entries of $A$ corresponding to the indices within $\mathcal{K}$. 
Let us introduce $\mathcal{K}_{i}$ ($1 \leq i \leq I$) and $\mathcal{B}_{j}$ ($1 \leq j \leq J$) to be disjoint sets of indices for the entries of $W$ and $H$, respectively, that is, 
\begin{itemize}

    \item $\mathcal{K}_{i} \subseteq \{ (f,k) \ | \ 1 \leq f \leq F, 1 \leq k \leq K\}$ for  $i = 1,2,\dots,I$, 
    
    \item $\mathcal{B}_{j} \subseteq \{ (k,n) \ | \ 1 \leq k \leq K, 1 \leq n \leq N\}$ for $j = 1,2,\dots,J$,
    
    
    \item $\mathcal{K}_{u} \cap \mathcal{K}_{v} = \emptyset$ for all $1 \leq u,v \leq I$ and $u \neq v$,
    
    \item $\mathcal{B}_{p} \cap \mathcal{B}_{q} = \emptyset$ for all $1 \leq p,q \leq J$ and $p \neq q$. 
\end{itemize} 
We now define penalized $\beta$-NMF with disjoint linear equality constraints as follows 
\begin{equation}\label{eq:betaNMFmodel}
\begin{aligned}
& \underset{W\in \mathbb{R}^{F \times K}_+,H\in \mathbb{R}^{K \times N}_+}{\min}
& & D_{\beta}\left(V|WH\right) + \lambda_1 \Phi_1(W) + \lambda_2 \Phi_2(H) \\
& \text{such that}
%& & H \geq 0, W \geq 0, \\
%& \text{}
& & \alphab_i^{T} W \left( \mathcal{K}_{i} \right) = b_i \text{ for } 1\leq i \leq I, \\
& \text{}
& &  \gammab_j^{T} H \left( \mathcal{B}_{j} \right) = c_j \text{ for } 1\leq j \leq J,
\end{aligned}
\end{equation}
where %$D_{\beta}\left(V|WH\right)=\sum_{f,n} d_{\beta}(V_{fn}|[ \,WH] \,_{fn})$, 
\begin{itemize}
    \item the penalty functions $\Phi_1(W)$ and $\Phi_2(H)$ 
    are lower bounded  and admit a particular upper approximation;  see Assumption~\ref{ass:phi} below. 
    %are separable functions\footnote{\ngi{This assumption is not strictly necessary, but is made because it greatly simplifies the presentation. It can be relaxed to the requirement that $\Phi_1(W)$ and $\Phi_2(H)$ possess an entry-wise quadratic separable majorizer of the form given in~\eqref{eq:Lipschtiz_case}. 
    %This will be the case for our example in Section~\ref{sec_minvolKLNMF} where $\Phi_1(W) = \logdet(W^T W + \delta I)$ satisfies only the latter assumption.}} w.r.t.\ the rows of $W$ and columns of $H$,  respectively, that is, we have  
   % $\Phi_2(H) = \sum_{n=1}^N \Phi_2(\hb_n)$ where $\hb_n \in \mathbb{R}_+^{F}$ denotes the $n$-th column of $H$, and similarly for $\Phi_1$. We will also need that $\Phi_1$ and $\Phi_2$ are concave, or admit an $L$-smooth gradient;  see Assumption~\ref{ass:phi} below. 
    
    \item $\lambda_1$ and $\lambda_2$ are the penalty weights (nonnegative scalars). 
    
    \item $\alphab_i \in \mathbb{R}^{|\mathcal{K}_i|}_{++}$ ($1\leq i \leq I$) and $\gammab_j \in \mathbb{R}^{|\mathcal{B}_j|}_{++}$ ($1\leq j \leq J$) are vectors with positive entries. 
    Note that if $\alphab_i$ or $\gammab_j$ contains zero entries,  the corresponding indices can be removed from $\mathcal{K}_{i}$ and $\mathcal{B}_{j}$.  
    
    \item $b_i$ ($1\leq i \leq I$) and $c_j$  ($1\leq j \leq J$) are positive scalars. 
\end{itemize}
% We denote by $\Psi$ the objective function 
% of~\eqref{eq:betaNMFmodel}, that is, 
% \[
% \Psi (W,H) = 
% D_{\beta}\left(V|WH\right) + \lambda_1 \Phi_1(W) + \lambda_2 \Phi_2(H). 
% \] 
%\ngc{(1) on a vraiment besoin qu'elles soient séparables? On montre justement plus bas comment s'en sortir si ce n'est pas le cas, non? Je pense qu'il faut juste qu'elles soient séparables par lignes de $W$ / colonnes de $H$, non? (2)  il faudrait de toute façon définir séparable.} \ngc{C'est la même pénalité sur $W$ et $H$? Ce n'est pas ce qu'on fait dans les exemples... Utiliser $\lambda_2 \Phi_2(H)$? Si c'était la même pénalité, il faudrait d'ailleurs plutôt utiliser  $\Phi_1(H^T)$ pour avoir la symmétrie.}  

As for most NMF algorithms, we propose to resort to a  block coordinate descent (BCD) framework 
to solve problem~\eqref{eq:betaNMFmodel}: at each iteration we tackle two sub-problems separately; one in $W$ and the other in $H$. 
% \algsetup{indent=2em}
% \begin{algorithm}[ht!]
% \caption{BCD framework to tackle NMF optimization problems \label{algo:metaalgo} }
% \begin{algorithmic}[1]
% \REQUIRE Input matrix $V \in \mathbb{R}^{F \times N}_+$, the factorization rank $K$ and
%  number of iterations maxiter. 
% \ENSURE $(W,H)$ is an approximate solution of~\eqref{eq:betaNMFmodel}. 
%     \medskip  
% \STATE Initialize $(W^{0}, H^{0}) \in \mathbb{R}^{F \times K}_+ \times \mathbb{R}^{K \times N}_+$. 
% \FOR {$k=1,2,\dots,$ maxiter}
%     \STATE \emph{\% Update $W$} 
%     \STATE $W^{k} \longleftarrow \text{update} (V,W^{k-1},H^{k-1}) \text{ typically such that }\Psi(W^{k},H^{k-1}) \leq \Psi(W^{k-1},H^{k-1})$ 
%     \STATE \emph{\% Update $H$} 
%     \STATE $H^{k} \longleftarrow \text{update} (V,W^{k},H^{k-1}) \text{ typically such that }\Psi(W^{k},H^{k}) \leq \Psi(W^{k},H^{k-1})$  
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}  
The subproblems in $W$ and $H$ are essentially the same, by symmetry of the model, since transposing the relation $X \approx WH$ gives $X^T \approx H^T W^T$. Hence, we may focus on solving the  subproblem in $H$ only, namely 
\begin{equation}
\label{eq:betaNMFmodelH}
 \underset{H\in \mathbb{R}^{K \times N}_+}{\min}
 D_{\beta}\left(V|WH\right) + \lambda_2 \Phi_2(H) 
\quad \text{ such that } \quad 
 \gammab_j^{T} H \left( \mathcal{B}_{j} \right)=c_j \text{ for } 1\leq j \leq J. 
\end{equation} 



%\paragraph{High-level approach to solve~\eqref{eq:betaNMFmodelH}}  

In order to solve~\eqref{eq:betaNMFmodelH}, we will design MU based on the majorization-minimization (MM) framework~\cite{sun2017majorization}, which is the standard in the NMF literature; see~\cite{Fevotte_betadiv} and the references therein. 
Let us briefly recall the high-level ideas to obtain MU via MM. 
Let us consider the general  problem 
\[
\min_{h \in \mathcal{H}} f(h). 
\] 
Given an initial iterate $\widetilde{h}\in \mathcal{H}$, MM generates a new iterate $\hat{h}\in \mathcal{H}$ that is guaranteed to decrease the objective function, that is,
$f\big( \hat{h} \big) \leq f\big( \widetilde{h}  \big)$. To do so, it uses the following two steps: 
\begin{itemize} 
\item Majorization: find a function that is an upper approximation of the objective and is tight at the current iterate, which is referred to as a majorizer. More precisely find a function $g\big(h|\widetilde{h}\big)$ such that 
\[
(i) ~ g\big(\widetilde{h}|\widetilde{h}\big) = f\big(\widetilde{h}\big) 
\quad \text{ and } \quad 
(ii)  ~  g\big({h}|\widetilde{h}\big) \geq f({h}) \text{ for all } h \in  \mathcal{H}. 
\]

\item Minimization: minimize the majorizer, that is, 
solve $\min_{h \in \mathcal{H}} g\big({h}|\widetilde{h}\big)$ approximately or exactly, to obtain the next iterate $\hat{h} \in \mathcal{H}$ which is such that $(iii) ~ g\big(\hat{h}|\widetilde{h}\big)  \leq g(\widetilde{h}|\widetilde{h})$. 
This guarantees the objective function to decrease at each step of this iterative process since 
\[
f\big(\hat{h}\big) 
\; 
\underset{(ii)}{\leq} 
\; 
g\big(\hat{h}|\widetilde{h}\big) 
\; 
\underset{(iii)}{\leq}  
\; 
g\big(\widetilde{h}|\widetilde{h}\big) 
\; 
\underset{(i)}{=} 
\; 
f\big(\widetilde{h}\big). 
\] 
\end{itemize}  
The MU for NMF are obtained using MM where the majorizer $g$ is chosen separable, that is, $g\big(h|\widetilde{h}\big) = \sum_{i=1} g_i\big(h_i|\widetilde{h}_i\big)$ for some well chosen univariate functions $g_i$'s; see~\eqref{eqn:auxbeta} in the next section. 
This choice typically makes the minimization of $g$ admits a closed-form solution which is multiplicative, that is, it has the form 
$\hat{h} = \widetilde{h} \odot c\big(\widetilde{h}\big)$ where $\odot$ is the component-wise product, and $c\big(\widetilde{h}\big)$ is a nonnegative vector that  depends on $\widetilde{h}$. We will encounter several examples later in this paper. 


%Let us illustrate this for the simplest case: standard NMF with $\beta = 2$. Each column of $H$ can be optimized independently since $||V-WH||_F^2 = \sum_{n = 1}^N \|  - W \|_2^2$. Let us denote Since the problem is independent for each column of $V$, this requires to solve $\min_{\hb \geq 0} \| \vb - W\hb \|_2^2$ where $\vb$ represents a column of $v$, and $\hb$ the corresponding column of $H$.   The majorizer is \[g(\hb | \widetilde{h}) =  \] 
 




In summary, to derive MU for~\eqref{eq:betaNMFmodelH}, we will follow the MM framework. 
\color{black}  
We first provide a majorizer for the objective of~\eqref{eq:betaNMFmodelH} in Section~\ref{sec:majorizer}. This majorizer has the property to be separable in each entry of $H$. In order to handle the equality constraints, 
we introduce Lagrange dual variables in Section~\ref{sec:lagrange}, and explain how they can be computed efficiently. 
This allows us to derive general MU in Section~\ref{betanmf_disjointconstraint} in the case of non-penalized $\beta$-NMF under disjoint linear equality constraints.
 This is showcased on simplex-structured $\beta$-NMF in Section~\ref{sec_ssbetaNMF}. In Section~\ref{sec_minvolKLNMF}, we will illustrate on minimum-volume KL-NMF  how to derive MU in the presence of penalty terms. 


%and then derive the proposed MU for~\eqref{eq:betaNMFmodelH} in Section~\ref{}.   


\ngi{\subsection{Separable majorizer for the objective function}}
\label{sec:majorizer} 

Let us derive a majorizer for 
$\Psi(H) := D_{\beta}\left(V|WH\right) + \lambda \Phi(H)$, 
that is, a function $G\big(H|\widetilde{H}\big)$ satisfying 
(i) $G\big(H|\widetilde{H}\big)  \geq \Psi(H)$ for all $H$, and 
(ii)  $G\big(\widetilde{H}|\widetilde{H} \big)  = \Psi\big(\widetilde{H} \big)$. Note that, to simplify the presentation, we denote $\Phi_2(H) = \Phi(H)$ and $\lambda = \lambda_2$. 
To do so, let us analyze each term of $\Psi(H)$ independently. 

\paragraph{Majorizing $D_{\beta}\left(V|WH\right)$} The first term $D_{\beta}\left(V|WH\right)$ can be decoupled into $N$ independent terms, one for each column $\hb_n$ of $H$, that is, 
$D_{\beta}\left(V|WH\right) = \sum_{n=1}^N D_{\beta}\left(\vb_n|W\hb_n\right)$, 
where $\vb_n$ denotes the $n$th column of matrix $V$. 
Let us focus on a specific column of $H$, denoted $\hb \in \mathbb{R}^K_+$, and the corresponding column of $V$, denoted $\vb \in \mathbb{R}^K_+$.  
We majorize $D_{\beta}(\vb|W\hb)=\sum_{f=1}^F d_{\beta}(v_f|(W\hb)_f)$  following the methodology introduced in \cite{Fevotte_betadiv}, {which consists in applying a convex-concave procedure \cite{Yuille03} to $d_{\beta}$}, as presented in Appendix~\ref{convconcacm}. The resulting upper bound is given by
%
\begin{equation}
\label{eqn:auxbeta}
d_{\beta}(v_f|(W\hb)_f) \leq
\sum_{k=1}^K \frac{w_{fk}\widetilde{h}_k}{\widetilde{v}_f}\widecheck{d} \left( v_f |  \widetilde{v}_f \frac{h_k}{\widetilde{h}_k} \right)
+ \widehat{d}'\big(v_f|\widetilde{v}_f\big) \sum_{k=1}^K w_{fk} \big(h_k - \widetilde{h}_k\big)
+ \widehat{d}\big(v_f | \widetilde{v}_f\big), 
\end{equation}
where $w_{fk}$ denotes the entry of matrix $W$ at position $(f,k)$, 
$\widetilde{v}_f := \big(W \widetilde{\hb}\big)_f$ denotes the $f$th entry of $\widetilde{\vb}$, 
and 
$\widehat{d}$ and $\widecheck{d}$ are the concave and convex parts of $d$, respectively. %\ngc{C'est correct?} 


\paragraph{Majorizing $\Phi(H)$}  For the second term $\Phi(H)$, we rely on the following assumption for $\Phi$. 
\begin{assumption} \label{ass:phi}
The function 
$\Phi : \mathbb{R}^{K \times N}_+ \mapsto \mathbb{R}$ %_\ngi{+}$
{is lower bounded, and} 
for any $\widetilde{H} \in \mathbb{R}^{K \times N}_+$ there exists constants $L_{kn}$ ($1 \leq k \leq K, 1 \leq n \leq N$) such that  the inequality 
\begin{equation} \label{eq:Lipschtiz_case} 
\Phi(H) 
  \;  \leq \;    \Phi\big( \widetilde{H} \big) + \left\langle \nabla\Phi(\widetilde{H}), H - \widetilde{H} \right\rangle + \sum_{k,n} \frac{L_{kn}}{2} (H_{kn} - \widetilde{H}_{kn})^2 
\end{equation} 
  is satisfied for all $H \in \mathbb{R}^{K \times N}_+$.  (Note that the constants $L_{kn}$ may depend on $\widetilde{H}$, this will be the case for example in Section~\ref{sec_minvolKLNMF}\color{black}).   
    % \Phi(H) 
    % \; \leq \;  \Phi\big( \widetilde{H} \big) + \left\langle \nabla\Phi(\widetilde{H}), H - \widetilde{H} \right\rangle + \frac{L}{2} \| H - \widetilde{H} \|_F^2, 
\end{assumption}

Let us mention two important classes of functions satisfying Assumption~\ref{ass:phi}. 
\begin{enumerate}

\item Smooth concave functions that are lower bounded on the nonnegative orthant. For such functions, we can take $L_{kn} = 0$ for all $k,n$ since they are upper approximated by their first-order Taylor approximation.  
Note that, in this case, 
\begin{equation}
\label{eq:geq0}
\nabla\Phi(\widetilde{H}) \geq 0,
\end{equation}
otherwise we would have 
$\lim_{y\rightarrow\infty}\Phi\big(H + y \eb_i \eb_j^T \big)=-\infty$, where $\eb_i$ is the $i$th unit vector, and 
this would contradict the fact that $\Phi$ is bounded from below. 
This observation will be useful in  the proof of Proposition~\ref{prop:mingmu} and is only valid for the special case $L_{kn} = 0$ for all $k,n$.  

Examples of such penalty functions include the  sparsity-promoting regularizers $\Phi(H) = \| H \|_p^p =  \sum_{k,n} H(k,n)^p$ for $0 < p \leq 1$ since $H \geq 0$.

\item Lower-bounded functions with Lipschitz continuous gradient for which~\eqref{eq:Lipschtiz_case} follows from the descent lemma~\cite{Bertsekas99}. 

Examples of such penalty functions include any smooth convex functions; for example any quadratic penalty, such as  
$||A H - B ||_2^2$ for some matrices $A$ and $B$ in which case $L_{kn} = \sigma_1(A)^2$ for all $k,n$.  
We will encounter another example later in the paper, namely $\logdet\big(HH^\top + \delta I\big)$ for $\delta > 0$ which allows to minimize the volume of the rows of $H$; see Section~\ref{sec_minvolKLNMF} for the details  %It was shown to satisfy~\eqref{eq:Lipschtiz_case} in~\cite{9084229}.  
(Note that we will use this regularizer for $W$). 

\end{enumerate}

% \begin{remark}[Tighter upper bound] \label{rem_tightUB}
% Assumption~\ref{ass:phi} can be replaced with an assumption which requires the existence of constants $L_{k,n}$ ($1 \leq i \leq K, 1 \leq n \leq N$) such that  the inequality 
% \[
% \Phi(H) 
%   \;  \leq \;    \Phi\big( \widetilde{H} \big) + \left\langle \nabla\Phi(\widetilde{H}), H - \widetilde{H} \right\rangle + \sum_{k,n} \frac{L_{k,n}}{2} (H - \widetilde{H})_{k,n}^2 
%   \]  
%   is satisfied for all $H \in \mathbb{R}^{K \times N}_+$. 
%   However, for simplicity of the presentation, we only consider a single constant $L$. In practice, it is better to consider different values for the $L_{k,n}$'s to obtain tighter upper bounds, as done for example in Section~\ref{sec_minvolKLNMF}. 
% \end{remark}


\paragraph{Majorizing $\Psi(H)$} 

Combining \eqref{eqn:auxbeta} and \eqref{eq:Lipschtiz_case}, we can construct a majorizer for $\Psi(H)$. Since both \eqref{eqn:auxbeta} and \eqref{eq:Lipschtiz_case} are separable in each entry of $H$, 
%For each column $\hb$ of $H$, a majorizer $G\big(\hb|\widetilde{\hb}\big)$ of $\psi(\hb)$ is obtained by combining . Finally, according to~\eqref{eq:psi(H)}, we obtain a majorizer $G\big(H|\widetilde{H}\big)$ for $\psi(H)$ as a sum of column-wise majorizers. 
their combination is also separable into a sum of $K\times N$ component-wise majorizers, up to an additive constant: 
%
\begin{equation}
%\label{eq:G}
G\big(H|\widetilde{H}\big) 
= \sum_{n=1}^N\sum_{k=1}^K g\big(h_{kn}|\widetilde{H}\big) + C\big(\widetilde{H}\big),
\end{equation}
where
\begin{align}
\label{eq:Gkn}
g\big(h_{kn}|\widetilde{H}\big) &= \sum_{f=1}^F \frac{w_{fk}\widetilde{h}_{kn}}{\widetilde{v}_{fn}}\widecheck{d} \left( v_{fn} |  \widetilde{v}_{fn} \frac{h_{kn}}{\widetilde{h}_{kn}} \right)
+ a_{kn} h_{kn}^2 + p_{kn} h_{kn},
\\
C\big(\widetilde{H}\big) &= \sum_{n=1}^N\sum_{f=1}^F\left(\widehat{d}\big(v_{fn} | \widetilde{v}_{fn}\big)
- \sum_{k=1}^K\widehat{d}'\big(v_{fn}|\widetilde{v}_{fn}\big) w_{fk} \widetilde{h}_{kn}\right) \ngi{+ a_{kn} \widetilde{h}_{kn}^2},
\notag
\end{align}
with $a_{kn}=\lambda\frac{L_{kn}}{2}$, and
\begin{equation*}
p_{kn}=\sum_{f=1}^F w_{fk}\widehat{d}'\big(v_{fn}|\widetilde{v}_{fn}\big) +\lambda\left(\frac{\partial \Phi}{\partial h_{kn}}\big(\widetilde{H}\big)- L_{kn} \widetilde{h}_{kn}\right).
\end{equation*} 
%Finally, it is important to note that the majorizer $G(h|\widetilde{h})$ of $\psi(h)$, obtained  by combining \eqref{eqn:auxbeta} and \eqref{eq:Lipschtiz_case}, is separable, that is, it can be written in the form 
%\[
%G(h|\widetilde{h}) 
%= \sum_{k=1}^K G_k(h_k|\widetilde{h}_k),
%\] 
%see~\eqref{eq:gj} in the next section for the expression of $G_k$.
%This will allow us to minimize the majorizer $G\big(H|\widetilde{H}\big)$ under the equality constraints efficiently, as presented in the next section.  



\subsection{Dealing with equality constraints via Lagrange dual variables}  \label{sec:lagrange} 

In the previous section, we derived a majorizer for $\Psi(H)$, $G\big(H|\widetilde{H}\big)$, which is separable in each entry of $H$. Without the equality constraints, we could then compute closed-form solutions to univariate problems to minimize $G\big(H|\tilde{H}\big)$ to obtain the standard MU for NMF as in~\cite{Fevotte_betadiv}. 

However, in problem~\eqref{eq:betaNMFmodelH}, the entries of $H$ in the subsets $\mathcal{B}_j$ are not independent as they are linked with the equality constraints $\gammab_j^{T} H ( \mathcal{B}_{j})=c_j$ for $j = 1,2,\dots,J$. 
In fact, to minimize the majorizer under the equality constraints, we need to solve 
%
\begin{equation}
\label{eq:betaNMFmodelHmajor}
\underset{H\in \mathbb{R}^{K \times N}_+}{\min}
 G\big(H|\widetilde{H}\big) 
\quad  \text{ such that } \quad 
\gammab_j^{T} H (\mathcal{B}_{j})=c_j \text{ for } 1\leq j \leq J. 
\end{equation} 
%
The variables in different sets $\mathcal{B}_j$ can be optimized independently, as they do not interact in the majorizer nor in the constraints. Note that, for the entries of $H$ that do not appear in any constraints, the standard MU~\cite{Fevotte_betadiv} can be used. 
For simplicity, let us fix $j$ and 
denote $\mathcal{B}=\mathcal{B}_j$, $Q = |\mathcal{B}|$, 
$\yb = H(\mathcal{B}) \in \mathbb{R}^{Q}_{+}$, $\gammab = \gammab_j \in \mathbb{R}^{Q}_{++}$, 
and $c = c_j > 0$.  
The problems we need to solve have the form 
\begin{equation}
\label{eq:minG}
\min_{\yb \in \Yc} G\big(\yb | \widetilde{H} \big), 
\end{equation} 
where $\Yc=\left\{\yb \in \mathbb{R}^{Q}_+ \ | \ \gammab^T\yb=c \right\}$ and
\begin{equation}
\label{eq:Gy}
G\big(\yb | \widetilde{H}\big)=\sum_{(k,n)\in \mathcal{B}}g\big(h_{kn} | \widetilde{H} \big),
\end{equation} 
where the component-wise majorizers $g\big(h_{kn}|\widetilde{H}\big)$ are defined by~\eqref{eq:Gkn}. 
Let us introduce a convenient notation: for ${q} = 1,2,\dots,Q$, we denote by $(k({q}), n({q}))$ the $q$th pair belonging to  $\mathcal{B}$. 
Hence the Lagrangian function of~\eqref{eq:Gy} can be written as 
%$G\big(\yb | \widetilde{H}\big) = \sum_{{q}=1}^Q g\big(y_{q}|\widetilde{H}\big)$. 
%
%Recall that $G(\yb | \widetilde{\yb} )$ is separable, that is, 
%$$
%G(\yb|\widetilde{\yb}) 
%= \sum_{{q} = 1}^Q g(y_{q}|\widetilde{\yb}) + C,
%$$
%where $C$ is a constant, and each component $g$ is given by: 
%\begin{align}
%g(y_{q}|\widetilde{\yb})&=\sum_{f=1}^F \frac{w_{fk({q})}\widetilde{\yb}_{q}}
%{\widetilde{v}_f}\widecheck{d} \big( v_f | \widetilde{v}_f \frac{y_{q}}{\widetilde{y}_{q}} \big) + a y_{q}^2 + p_{q} y_{q},
%\label{eq:gj}
%\end{align}
%%
%\ngc{J'ai changé $b$ par $p$ car je l'utilisais pour les contraintes linéaires en $W$; cf. (2)}
%with $a=\lambda\frac{L}{2}$, 
%%
%\begin{equation}
%\label{eq:pell}
%p_{q}=\sum_{f=1}^F w_{fk({q})}\widehat{d}'(v_f|\widetilde{v}_f) +\lambda\big(\frac{\partial \Phi}{\partial y_{q}}(\widetilde{\yb})- L\widetilde{\hb}_{n({q})\big), 
%\end{equation}
%and the constants $w_{fk({q})}$ correspond to entries of $W$ and are assumed to be positive. \ngc{Il faudrait mieux les définir, je suppose que $z$ peut être construit à partir de $W$, mais ce serait intéressant d'écrire la formule explicitement.}    
%
%In order to solve \eqref{eq:minF} using an iterative majorization-minimization scheme, let us consider the constrained problem
%\begin{equation}
%\label{eq:minG}
%\min_{\yb\in \Yc} G(\yb|\widetilde{\yb}).
%\end{equation}
%The corresponding  reads
{
\begin{equation}
\label{eq:Gmuy}
    G^\mu\big(\yb|\widetilde{H}\big)  
    = G\big(\yb|\widetilde{H}\big)-\mu(\gammab^T\yb-c) 
    = \mu c + C\big(\widetilde{H}\big) + \sum_{{q}=1}^Q  g^\mu\big(y_{q}|\widetilde{H}\big), 
\end{equation}
%\ngc{Faire attention avec les sommes indicées: cela peut prêter à confusion. Je préfère 
%$\mu c + C + \sum_{{q}=1}^Q g^\mu\big(y_{q}|\widetilde{H}\big)$.} 
where
%---------------------------
\begin{align}
g^\mu\big(y_{q}|\widetilde{H}\big) 
& = g\big(y_{q}|\widetilde{H}\big)-\mu \gamma_{q}\,y_{q}\notag \\ 
& = \sum_{f=1}^F \frac{w_{fk({q})}\widetilde{y}_{q}}{\widetilde{v}_{fn({q})}}\widecheck{d} \left( v_{fn({q})} |  \widetilde{v}_{fn({q})} \frac{y_{q}}{\widetilde{y}_{q}} \right)
+ a_q y_{q}^2 + (p_{q}-\mu \gamma_{q}) y_{q},
\label{eq:gmu}
\\
p_{q}&=\sum_{f=1}^F w_{fk({q})}\widehat{d}'\big(v_{fn({q})}|\widetilde{v}_{fn({q})}\big) +\lambda\left(\frac{\partial \Phi}{\partial y_{q}}\big(\widetilde{H}\big)- L_{k(q)n(q)} \widetilde{y}_{q}\right), 
\label{eq:pell}
\end{align}
}
and $\mu\in\mathbb{R}$.
Note that $G^\mu$ is separable, as is $G$, because the term $\gammab^T \yb$ is linear. 
%for any fixed value for $\mu$, $G^{\mu}$ \eqref{eq:Gmuy} is a separable approximation of the Lagrangian function $\Psi(\yb)-\mu(\gammab^T\yb-c)$.

Assume for now that the Lagrangian multiplier $\mu$ is known, and let us minimize $G^\mu\big(\yb|\widetilde{H}\big)$ on $(0,\infty)^Q$. 
Such a problem is separable under the form of $Q$ subproblems, consisting in minimizing univariate functions  $g^\mu\big(\cdot|\widetilde{H}\big)$ separately over $(0,\infty)$. We now show in Proposition~\ref{prop:mingmu} that, under mild conditions, each subproblem admits a unique solution over $(0,\infty)$. %Let us emphasise the fact that in Proposition \ref{prop:mingmu}, we assume that the optimal value for $\mu$ is known. 
%to be minimized on $y\in(0,\infty)$, where $\mu\in\mathbb{R}$.
%
%---------------------------
\begin{proposition}
\label{prop:mingmu}
%\ngc{Je pense que pour cette proposition, il faut considérer un seul ${q}$: j'ai modifié, please check :-)}
Let ${q} \in \{1,2,\dots,Q\}$. 
Assume that $\beta<2$ and $\widetilde{y}_{q},v_{fn({q})},w_{fk({q})}>0$ for all $f$.
%\ngc{Vérifier les indices... Faut-il vraiment que $V>0$? Cela parait restrictif...}
Moreover, when $\beta\leq1$, assume that $\mu < \frac{p_{q}}{\gamma_{q}}$ for all $q$ such that $a_q=0$. 
Then there exists a unique minimizer $y_{q}^\star(\mu)$ of $g^\mu\big(y_{q}|\widetilde{H}\big)$ in $(0,\infty)$.  
\end{proposition}
%---------------------------

%
\begin{proof}
According to Proposition~\ref{prop:approxdbeta} (see Appendix~\ref{convconcacm}), each $g^\mu$ is $C^\infty$ and strictly convex on $(0,\infty)$, so its infimum is uniquely attained in the closure of $(0,\infty)$. We have to prove that it is neither reached at $0$ nor at $\infty$. 
On the one hand, \ji{from \eqref{eq:gmu}, we have 
%
\begin{equation}
\label{eqgmu'}
(g^\mu)'\big(y_{q}|\widetilde{H}\big)=\sum_{f=1}^F w_{fk({q})}\widecheck{d}' \left( v_{fn({q})} | \widetilde{v}_{fn({q})}\frac{y_{q}}{\widetilde{y}_{q}} \right) +2a_q y_{q} + p_{q} -\gamma_{q}\mu
\end{equation}
}%
and, for any $\beta<2$ and any $x>0$,
%
\begin{equation*}
%\label{eq:d'0} not used 
\lim_{y\rightarrow0^+}\widecheck{d}'(x|y)=-\infty,\\
\end{equation*}
%
so $\lim_{y_{q}\rightarrow0^+}(g^\mu)'\big(y_{q}|\widetilde{H}\big)=-\infty$, which ensures that the infimum is not reached at $0$.
%\ji{This would not apply to the case $\beta\geq2$. Things are probably OK then if $\lambda=0$, but I have decided to discard the case $\beta\geq2$ for the sake of coherence, and because it is not of great interest from the application viewpoint. This could maybe deserve a comment somewhere (but we should first check the calculations when $\beta\geq2$).} 
On the other hand,
%
\begin{equation}
\lim_{y\rightarrow\infty}\widecheck{d}'(x|y)=\begin{cases}0&\text{if } \beta\leq1,\\\infty&\text{otherwise.}\end{cases}
\label{eq:d'inty}
\end{equation}
%
According to \eqref{eqgmu'} and \eqref{eq:d'inty}, the distinction must be made between two cases:
%
\begin{itemize}
\item If $a_q>0$ or $\beta\in(1,2)$: $\lim_{y_{q}\rightarrow\infty}(g^\mu)'\big(y_{q}|\widetilde{H}\big)=\infty$, so the infimum is reached for a finite $y_{q}$. 
\item If $a_q=0$ and $\beta\leq1$: $\lim_{y_{q}\rightarrow\infty}(g^\mu)'\big(y_{q}|\widetilde{H}\big)=p_{q} -\gamma_{q}\mu$, so the same conclusion holds if $\mu<\frac{p_{q}}{\gamma_{q}}$. 
\end{itemize}
\end{proof}
We just proved that, under mild conditions, each $g^\mu$ has a unique minimizer over $(0,\infty)$.
%\ngc{Discuter la condition $\mu<\frac{p_{q}}{\gamma_{q}}$?} 
However we assumed that the value of $\mu$ is fixed.  
Now given $\yb^\star(\mu)=\big[y_1^\star(\mu),\ldots,y_Q^\star(\mu)\big]^T$, let us show 
that the solution to $\gammab^T \yb^\star(\mu) =c$ is unique. The corresponding value of $\mu$, which we denote  $\mu^\star$, provides  the minimizer $\yb^\star(\mu^\star)$ of $G^\mu(\yb|\widetilde{H})$ that satisfies the linear constraint $\gammab^T\yb^\star(\mu^\star)=c$. \ji{Moreover, $\mu^\star$ naturally fulfills $\mu^\star<\frac{p_{q}}{\gamma_{q}}$ for all $q$ when $\beta\leq1$ and $a_q=0$, as required in Proposition~\ref{prop:mingmu}.}
%Finally, we prove that $\mu^\star$ is unique on some specific interval under mild conditions. 
%\sout{further}
%Let us remark that, at this stage, $\yb^\star$ is a vector function of $\mu$.
%
%---------------------------
\begin{proposition}
\label{prop:mu_unicity} 
Assume that $\beta<2$ and $\widetilde{y}_{q}, v_{fn({q})},w_{fk({q})}>0$ for all ${q},f$. %\ngc{Vérifier les indices}
%and let $y_{q}^\star(\mu)$ be the unique minimizer of  $g^\mu\big(y_{q}|\widetilde{H}\big)$ in $(0,\infty)$ as defined in Proposition~\ref{prop:mingmu}, for ${q}=1,2,\dots,L$. %\ngc{Ne doit-on pas indiquer les conditions sur $\mu$ comme dans la Proposition 1: $\mu < \min_{{q}} \frac{c_{q}}{\gammab_l}$ when $\beta \le 1$ et $a=0$?} 
%=(y_1^\star,\ldots,y_P^\star)^T$.  
Then the scalar equation $\gammab^T \yb^\star(\mu) =c$ in the variable $\mu$ admits a unique solution $\mu^\star$ in $(-\infty,t)$, where
\begin{align}
\label{eq:t}
t&=\min_{1 \leq q \leq Q} t_q, \text{ where }
%\begin{cases}\ji{\min_{\{q | a_q = 0\}} \frac{p_{q}}{\gamma_{q}}}\geq0&\text{if $\beta\leq1$ and $a_q=0$ for some $q$},\\\infty&\text{otherwise,}\end{cases}
t_q=\begin{cases} \frac{p_{q}}{\gamma_{q}}&\text{if $\beta\leq1$ and $a_q=0$,}\\\infty&\text{otherwise, }\end{cases}
\end{align} 
{so that $\yb^\star(\mu^\star)$ $\in(0,\infty)^Q$} is the unique solution to problem~\eqref{eq:minG}.
\end{proposition}
%---------------------------
\begin{proof}
Under the conditions of Proposition~\ref{prop:mingmu}, $g^\mu\big(y_{q}|\widetilde{H}\big)$ has a unique minimizer $y^\star_{q}(\mu)$ for each $j$.  
%\ngc{A rephraser. Veux-tu dire que: 
%According to PrYurii Nesterovoposition~\ref{prop:mingmu}, $g^\mu\big(y_{q}|\widetilde{H}\big)$ has a unique minmizer for each $j$, which we denote $y^\star_{q}$.} 
By the first-order optimality condition, $y^\star_{q}(\mu)$ is a solution of $(g^\mu)'\big(y_{q}|\widetilde{H}\big)=0$ or equivalently, by \eqref{eqgmu'}, a solution of $\gamma_{q}^{-1}g'\big(y_{q}|\widetilde{H}\big)=\mu$ over $(0,\infty)$ where 
%
\begin{equation}
\label{eq:g'}
\gamma_{q}^{-1}g'\big(y_{q}|\widetilde{H}\big)=\gamma_{q}^{-1}\sum_{f=1}^F w_{fk({q})}\widecheck{d}' \left( v_{fn({q})} | \widetilde{v}_{fn({q})} \frac{y_{q}}{\widetilde{y}_{q}} \right) +2 \frac{a_q}{\gamma_{q}}y_{q} + \frac{p_{q}}{\gamma_{q}}
\end{equation}
%
is strictly increasing on $(0,\infty)$ (since $g$ is strictly convex) and one-to-one from $(0,\infty)$ to an open interval
$T_{q}=(t^-_{q},t^+_{q})$ where
%
\begin{align}
t^-_{q}&=\lim_{y_{q}\rightarrow0}g'\big(y_{q}|\widetilde{H}\big)=-\infty,\\
t^+_{q}&=\lim_{y_{q}\rightarrow\infty}g'\big(y_{q}|\widetilde{H}\big)
 = t_q. 
%\begin{cases} \frac{p_{q}}{\gamma_{q}}&\text{if $\beta\leq1$ and $a_q=0$,}\\\infty&\text{otherwise.}\end{cases}
\end{align}
%
Moreover, $p_{q}\geq0$ if $a_q=0$ (then $L=0$) and $\beta\leq1$ according to~\eqref{eq:geq0} and \eqref{eq:pell}.
As a consequence, $\gamma_{q}^{-1}g'(y_{q}^\star|\widetilde{y}_{q})=\mu$ is equivalent to
\begin{equation}
\label{eq:yhat}
y_{q}^\star(\mu) = \big(g'\big)^{-1}(\gamma_{q}\mu),
\end{equation}
where $\mu\in T_{q}$ and $\big(g'\big)^{-1}$ denotes the inverse function of $g'$.

Coming back to the multivariate problem~\eqref{eq:minG}, we must find a value $\mu^\star$ of the Lagrangian multiplier such that the constraint $\gammab^T\yb^\star(\mu)=c$ is satisfied. Given~\eqref{eq:yhat}, $\mu^\star$ is a solution of
%
\begin{equation}
\label{eq:muhat}
\sum_{{q}=1}^Q \gamma_{q}\big(g'\big)^{-1}(\gamma_{q}\mu)=c.
\end{equation}
%
Each $g'\big(y_{q}|\widetilde{H}\big)$ being strictly increasing on $(0,\infty)$, $(g')^{-1}(\gamma_{q}\mu)$ is also strictly increasing (from $T_{q}$ to $(0,\infty)$), this is a direct consequence of $(f^{-1})'=\frac1{f' \circ f^{-1}}$ where $f$ is any strictly increasing function on some interval. Finally $\sum_{{q}=1}^Q  \gamma_{q}(g')^{-1}(\gamma_{q}\mu)$ is strictly increasing from $\cap_{j=1}^J T_{q}=(-\infty,t)$ to $(0,\infty)$, with $t\geq0$. Therefore, the solution $\mu^\star$ is unique. 
\end{proof}

 Proposition~\ref{prop:mu_unicity} shows that the optimal Lagrangian multiplier is the unique solution of~\eqref{eq:muhat}. Finding the solution of~\eqref{eq:muhat} is equivalent to finding the root of a function $r(\mu)$. We propose here-under to use a Newton-Raphson method to compute $\mu^\star$, and show that this method generates a sequence of iterates $\mu_n$ that converges towards $\mu^\star$ at a quadratic speed.

%---------------------------
\begin{proposition}
\label{NR} 
Assume that $\beta<2$ and $\widetilde{y}_{q},v_{fn({q})},w_{fk({q})}>0$ for all ${q},f$. %\ngc{Vérifier les indices}
Let
$$
r(\mu)=\sum_{{q}=1}^Q  \gamma_{q}(g')^{-1}\big(\gamma_{q}\mu\big)-c
$$
for $\mu\in(-\infty,t)$ where $t$ is defined in~\eqref{eq:t}, and denote $\mu^\star$ the unique solution of $r(\mu)=0$. 
From any initial point $\mu_0\in(\mu^\star,t)$, Newton-Raphson's iterates
$$
\mu_{n+1}=\mu_n-\frac{r(\mu_n)}{r'(\mu_n)}
$$
decrease towards $\mu^\star$ at a quadratic speed.
\end{proposition}
\begin{proof}
We already know that $r$ is strictly increasing from $(-\infty,t)$ to $(0,\infty)$. Let us show that $r$ is also strictly convex.
According to the third item of Proposition~\ref{prop:approxdbeta} in Appendix~\ref{convconcacm}, $\widecheck{d}''(x|y)$ is completely monotonic, so it is strictly decreasing in $y$. Equivalently, $\widecheck{d}'(x|y)$ is strictly concave in $y$, and each $g'$ is also strictly concave according to~\eqref{eq:g'}. Since the inverse of a strictly increasing, strictly concave function $f$ is strictly increasing and strictly convex, which is a direct consequence of $(f^{-1})''=-\frac{f''\circ f^{-1}}{(f' \circ f^{-1})^3}$, 
then each $(g')^{-1}$ is strictly convex, and finally, $r$ is strictly convex.

For any $\mu_0\in(\mu^\star,t)$, we have $r(\mu_0)>0$, so $\mu_1=\mu_0-\frac{r(\mu_0)}{r'(\mu_0)}<\mu_0$. We have also $\mu_1>\mu^\star$ as a consequence of the strict convexity of $r$. By immediate recurrence, we obtain that $\mu_n$ is a decreasing series that converges towards $\mu^\star$. According to \cite{Ortega70}, it converges at a quadratic speed since $|r'|$ and $|r''|$ are bounded away from 0 in $[\mu^\star,\mu_0]$.
\end{proof}



\paragraph{Discussion} 

At this point, we have derived an optimization framework to tackle problem~\eqref{eq:minG}. 
The optimal Lagrangian multiplier value is determined before each majorization-minimization update using a Newton-Raphson algorithm. However, such a formal solution is implementable if and only if each $y_{q}^\star(\mu)$ can be actually computed as the minimizer of $g^\mu\big(y_{q}|\widetilde{H}\big)$ in $(0,\infty)$. In some cases, computing $y_{q}^\star(\mu)$ is equivalent to extracting the roots of a polynomial of a degree smaller or equal to four, which is possible in closed form. In other cases, we have to solve a polynomial equation of degree larger than four, or even an equation that is not polynomial. Table~\ref{tab:poldeg} indicates the cases where a closed-form solution is available, and hence when our framework can be efficiently implemented. 
\begin{table}[h]
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\hfill     
&$\beta \in (-\infty,1)\setminus\{0\}$ 
& $\beta = 0$ 
& $\beta = 1$ & 
\multicolumn{4}{|c|}{$\beta \in (1,2)$}      \\
 &    &   &   &$\frac54$&$\frac43$&$\frac32$&other           \\\hline
%No penalization& 1 & 1  & 1  & 1        &  1       &  1       &  1           \\\hline
\begin{tabular}{c}
\revise{No penalization, or} \\ 
\revise{{$L_{kn} = 0$ for all $k,n$}} 
\end{tabular} 
&1&1&1&3&4&2&$\rip$\\\hline
{$L_{kn} > 0$ for some $k,n$}  &$\rip$&3&2&$\rip$&$\rip$&3&$\rip$\\\hline
\end{tabular}
\caption{%\ji{Est-ce que nous devrions ajouter une ligne "no penalization", qui correspondrait aus cas traite en Sous-section~\ref{betanmf_disjointconstraint} ? Dans ce cas, sauf erreur, le degre est 1 dans chaque cas. } \ngc{Oui, tout à fait d'accord, et cela permet de motiver pq on considère ce cas dans la section 2.3!} 
Cases where \eqref{eq:yhat} can be computed in closed form. They are indicated by the degree of the corresponding polynomial equation, otherwise the symbol $\rip$ is used. The constants $L_{kn}$ are the one needed in Assumption~\ref{ass:phi} for the penalization functions $\Phi_1(H)$ and $\Phi_2(W)$; see~\eqref{eq:Lipschtiz_case}. }
%\ji{(I have maintained $\beta\geq2$ here, we will need to decide what to do with this case.)}
\label{tab:poldeg}
\end{table}
\revise{We observe that, without penalization or with penalization satisfying $L_{kn} = 0$ for all $k,n$ (e.g., smooth concave functions), 
the polynomial equation is of degree one, and hence always admit a closed form for $\beta \leq 1$ 
and $\beta \in \left\{\frac{5}{4}, \frac{4}{3}, \frac{3}{2} \right\}$. 
} 
This particular case is discussed in the next section, which we will exemplify in Section~\ref{sec_ssbetaNMF} with $\beta$-NMF with sum-to-one constraints on the columns of $H$.  
In Section~\ref{sec_minvolKLNMF}, we will present an important example with $L_{kn} > 0$ for all $k,n$ and $\beta = 1$, namely minimum-volume KL-NMF. 




% This section is organized as follows:
% \begin{itemize}
%     \item Subsection \ref{convconcacm} presents the convexity, concavity and complete monotonicity properties of a convex-concave decomposition of the discrete $\beta$-divergence that is crucial for the efficiency of the general framework and the derived algorithms,
%     \item Subsection \ref{prob_algo_generalframe} firstly introduces the general form of a multivariate minimization problem involving a finite sum of discrete $\beta$-divergence terms under a linear constraint with a possible penalty term in the objective function. This penalty term can be either concave or Lipschitz smooth. % with constant $L$.
%     Secondly we present the general framework to tackle such optimization problems relying on the construction at the current iterate of an auxiliary function for the Lagrangian that is minimized in closed-form. Thirdly, we present the rate of convergence for the Newton-Raphson method used to compute the optimal Lagrangian multipliers at each iteration of the optimization framework.
%     \item Subsection \ref{betanmf_disjointconstraint} presents the algorithm obtained from the general framework in the case of nonpenalized $\beta$-NMF under disjoint linear equality constraints.
% \end{itemize}

% \subsection{Convexity, concavity and complete monotonicity for a convex-concave decomposition of the discrete $\beta$-divergence}\label{convconcacm}
% The discrete $\beta$-divergence can always be expressed as the sum of convex, concave, and constant terms. In Table \ref{tab:decompbetadiv} we introduce a convex-concave decomposition of the $\beta$-divergence which slightly differ from the one given in \cite[Table\,1]{Fevotte_betadiv} (by the fact that ours contains no constant term $\widebar{d}$) as follows:
% % \[
% % \widecheck{d}(x|y)=  \begin{cases}
% % \frac{1}{1-\beta} x \,y^{\beta -1}
% %       &\text{for}\quad \beta<1, \beta\neq0,  \\
% % \frac{x}{y}
% %       &\text{for}\quad \beta=0,   \\
% % %y-x-x\log \frac{y}{x}           
% % -x\log y           
% %       &\text{for}\quad \beta=1,  \\
% % \frac1{\beta}y^{\beta}-\frac1{\beta-1} xy^{\beta-1} &\text{for} \quad \beta \in \left(1,2\right), \\
% % \frac{1}{\beta} y^{\beta}
% %       &\text{for}\quad \beta\geq2,
% %   \end{cases}
% % \]
% % and
% % \[
% % \widehat{d}(x|y)= \begin{cases}
% %  \frac{1}{\beta}y^{\beta}-\frac{1}{\beta\,(1-\beta)} x^{\beta}
% %       &\text{for}\quad \beta<1, \beta\neq0,  \\
% % \log\frac{y}{x} - 1
% %       &\text{for}\quad \beta=0,   \\
% % %y-x-x\log \frac{y}{x}           
% % y + x\, \log x - x          
% %       &\text{for}\quad \beta=1,  \\
% % \frac{1}{\beta\,(\beta-1)} x^{\beta} &\text{for} \quad \beta \in \left(1,2\right), \\
% % -\frac{1}{\beta-1} x \,y^{\beta -1}+\frac{1}{\beta\,(\beta-1)} x^{\beta}
% %       &\text{for}\quad \beta\geq2,
% %   \end{cases}
% % \]
% % \ji{a remplacer peut-etre par une table a 5 lignes, 2 colonnes}



% \begin{table}[h]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \hfill$\beta$     &$(-\infty,1)\setminus\{0\}$&$0$&$1$&$(1,2)$ &   $[2,+\infty)$    \\
% Decomposition $d_{\beta}(x|y)$&  &   &  &    &   \\\hline
% $\widecheck{d}(x|y)$& $\frac{1}{1-\beta} x \,y^{\beta -1}$    & $\frac{x}{y}$  & $-x\log y$  &  $\frac1{\beta}y^{\beta}-\frac1{\beta-1} xy^{\beta-1}$  & $\frac{1}{\beta} y^{\beta}$  \\\hline
% $\widehat{d}(x|y)$&$ \frac{1}{\beta}y^{\beta}-\frac{1}{\beta\,(1-\beta)} x^{\beta}$&$\log\frac{y}{x} - 1$&$y + x\, \log x - x  $&$\frac{1}{\beta\,(\beta-1)} x^{\beta}$&$-\frac{1}{\beta-1} x \,y^{\beta -1}+\frac{1}{\beta\,(\beta-1)} x^{\beta}$\\\hline
% \end{tabular}
% }
% \caption{
% Proposed concave-convex decomposition of the discrete $\beta$-divergence.}
% %\ji{(I have maintained $\beta\geq2$ here, we will need to decide what to do with this case.)}
% \label{tab:decompbetadiv}
% \end{table}



% where $y\in(0,\infty)$, $\beta$ is real valued and $x\in(0,\infty)$, so that $d_{\beta}(x|y)=\widehat{d}(x|y)+\widecheck{d}(x|y)$. Further, $\beta$ and $x$ are considered as parameters, $d_{\beta}$, $\widehat{d}$ and $\widecheck{d}$ being handled as univariate functions of $y$.\\

% Let us now recall the definition of a complete monotonic function $f$:
% \begin{definition}
% A function $r$ is said to be completely monotonic (c.m.) on an interval $I$ if $r$ has derivatives of all orders on $I$ and $(-1)^n f^{(n)}(x)\geq0$ for $x\in I$ and $n\geq0$.
% \end{definition}
% We can now introduce the properties of concavity, convexity and monotonicity for  our convex-concave formulation of the discrete $\beta$-divergence:

% \begin{proposition} Given $\widecheck{d}(\cdot|\cdot)$ and $\widehat{d}(\cdot|\cdot)$ as defined above, we have that
% \label{prop:approxdbeta}
% \hfill
% \begin{enumerate}
% \item $\widecheck{d}(x|y)$ is $C^\infty$ and strictly convex on $(0,\infty)$ for $x>0$ and $\beta\in\mathbb{R}$;
% \item $\widehat{d}(x|y)$ is concave for $x>0$ and $\beta\in\mathbb{R}$;
% \item for all $\beta<2$, $\widecheck{d}''_{\beta}(x|y)$ and $\widehat{d}'_{\beta}(x|y)$ are c.m. 
% \end{enumerate}
% %Functions $g_1,\ldots,g_5$ are stricly convex on $(0,\infty)$. Moreover, $g_1$, $g_2$, $1-g'_3$, and $g''_4$ are completely monotonic on $(0,\infty)$.
% \end{proposition}
% \begin{proof}
% The proof is straightforward, given that $\widecheck{d}(x|y)$ and $\widehat{d}(x|y)$ linearly combine $C^\infty$ functions on $(0,\infty)$, and that in the same interval, 
% \begin{itemize}
% \item $\log y$ is strictly concave;
% \item $y^\nu$ is strictly convex for all  $\nu\in(-\infty,0)\cup(1,\infty)$, and strictly concave for all $\nu\in(0,1)$;
% \item $y^\nu$ is c.m. for all $\nu<0$.
% \end{itemize}
% \end{proof}
% According to the first two items of Proposition~\ref{prop:approxdbeta}, $\widecheck{d}$ and $\widehat{d}$ indeed yield a convex-concave decomposition of the $\beta$-divergence, which is a variant of \cite[Table\,1]{Fevotte_betadiv}. Let us remark that the successive minimization of an upper approximation of this convex-concave decomposition following the methodology presented in \cite{Fevotte_betadiv} yields to the usual multiplicative update scheme. 
% In the following subsection, we take advantage of these properties to build up a framework that enables to efficiently tackle penalized minimization problems relying on discrete $\beta$-divergence under linear constraints.








\subsection{MU for $\beta$-NMF with disjoint linear equality constraints without penalization}\label{betanmf_disjointconstraint}


In this section, we derive an algorithm based on the general framework presented in the previous section to tackle the $\beta$-NMF problem under disjoint linear equality constraints without penalization, that is,  problem~\eqref{eq:betaNMFmodel} with $\lambda_1=\lambda_2=0$.
We consider this simplified case here as it allows to provide explicit MU for any value of $\beta < 2$; see the row `No penalization' of Table~\ref{tab:poldeg}. These updates  satisfy the constraints after each update of $W$ or $H$, and monotonically decrease the objective function $D_{\beta}\left(V|WH\right)$. 
% \subsubsection{Algorithm for disjoint-constrained $\beta$-NMF}\label{sec_algodisjointConstrainedbetaNMF} 

Let us then consider the subproblem of \eqref{eq:betaNMFmodel} over $H$ when $W$ is fixed and with $\lambda_2=0$, that is,  
%
\begin{equation}\label{eq:subprobleminW}
 \underset{H\in \mathbb{R}^{K \times N}_+}{\min}
 D_{\beta}\left(V|WH\right) 
\quad \text{such that} \quad \gammab_j^{T} H (\mathcal{B}_{j})=c_j \text{ for } 1\leq j \leq J.
\end{equation}
%\ngc{Ce n'est pas très naturel de faire tout en $W$ ici, alors qu'on a fait $H$ avant... ce n'est pas grave, mais juste un peu 'confusing'. Surtout que dans la section suivante, on est de retour sur $H$ avec le showcase 1... Cela vaudrait la peine de changer, mais ce n'est pas une priorité.}  
%In the following we derive MU for $H$ that decrease the objective in \eqref{eq:subprobleminW}. 
Let us follow the framework presented above. First, an auxiliary function, which we denote $G(H| \widetilde{H})$, is constructed at the current iterate $\widetilde{H}$ so that it majorizes the objective for all $H$ and is defined as follows:
%
\begin{equation}
\label{eq:G}
\begin{aligned}
G\big(H|\widetilde{H}\big) 
& = \sum_{f,n}\left[\sum_{k} \frac{w_{fk}\widetilde{h}_{kn}}{\widetilde{v}_{fn}}\widecheck{d}\left(v_{fn} \Big|\widetilde{v}_{fn}\frac{h_{kn}}{\widetilde{h}_{kn}}\right)\right] +\left[\widehat{d}'\big(v_{fn}|\widetilde{v}_{fn}\big)\sum_{k}w_{fk}\big(h_{kn}-\widetilde{h}_{kn}\big)+\widehat{d}\big(v_{fn}|\widetilde{v}_{fn}\big) \right], 
\end{aligned}
\end{equation} 
%\ngc{Give a bit more details: convex-concave-constant decomposition, etc.}
where $\widecheck{d}(.|.)$ and $\widehat{d}(.|.)$ are  given in Appendix~\ref{convconcacm}.
Second, we need to minimize $G\big(H|\widetilde{H}\big)$ 
%$D_{\beta}\left(V|WH\right)$ over $\mathbb{R}_{+}^{K \times N}$ with the auxiliary function of $G$, 
while imposing the set of linear constraints $\gammab_j^{T} H (\mathcal{B}_{j})=c_j$. The Lagrangian function of $G$ is given by 
\begin{equation}\label{eq:Gmu}
\begin{aligned}
G^{\mu}(H|\widetilde{H})= G(H |\widetilde{H} )-\sum_{j}^{J} \left[\mu_{j} \left( \gammab_j^{T} H (\mathcal{B}_{j})-c_j\right) \right], 
\end{aligned}
\end{equation} 
 where $\mu_{j}$ are the Lagrange multipliers associated to each linear constraint $\gammab_j^{T} H (\mathcal{B}_{j})=c_j$. We observe that $G^{\mu}$ in~\eqref{eq:Gmu} is a separable majorizer in the variables $H$ of the Lagrangian function $D_{\beta}\left(V|WH\right) - \sum_{j}^{J} \left[ \mu_{j} \left( \gammab_j^{T} H (\mathcal{B}_{j})-c_j\right) \right]$. Due to the disjoitness of each subset of variables $\mathcal{B}_{j}$ \eqref{eq:Gmu}, we only consider the optimization over one specific subset $\mathcal{B}_{j}$. 
The minimizer \eqref{eq:yhat} of $G^{\mu}(H\left( \mathcal{B}_{j} \right)|\widetilde{H}\left( \mathcal{B}_{j} \right))$ has the following component-wise expression:
\begin{equation}\label{eq:updateW}
\begin{aligned}
H^\star\left(\mathcal{B}_{j}\right)=\widetilde{H}\left(\mathcal{B}_{j}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{j}\right) \right]}{\left[ D\left(\mathcal{B}_{j}\right) - \mu_{j}  \gammab_j \right]} \right)^{. \eta \left( \beta \right)} , 
\end{aligned}
\end{equation}  
where $C=W^{T} \left( \left( WH \right)^{.\left( \beta-2 \right) } \odot V \right)$, $D=W^{T}\left( WH\right)^{.\left( \beta-1 \right) }$, $\eta(\beta)=\frac{1}{2-\beta}$ for $\beta \leq 1$, 
%$\eta(\beta)=1$ for $\beta \in \left[1,2\right]$ 
and $\eta(\beta)=\frac{1}{\beta-1}$ for $\beta \geq 2$ \cite[Table 2]{Fevotte_betadiv}, $A \odot B$ 
(resp.\@ $\frac{\left[ A \right]}{\left[ B \right]}$) is the Hadamard product (resp.\@ division) between $A$ and $B$,  
$A^{.\alpha}$ is the element-wise $\alpha$ exponent of $A$. 
\revise{
The case $\beta \in (1,2)$ is more difficult: 
we need to find a root of a function of the form 
$\mu + b x^{\beta-1} - c x^{\beta-2} = 0$. 
For example, for $\beta = \frac{3}{2}$, we have  
$\mu  + b x^{1/2} - c x^{-1/2} = 0$. 
Using  $y=\sqrt{x}$, and after simplifications, 
we obtain 
$\mu y + b y^{2}  - c = 0$ leading to the positive root 
$x = \left(\frac{\sqrt{\mu^2+4bc} -\mu}{2b}\right)^2$.  
} 

%\ngc{Tu ne définirais pas dès le début $f_i = a_i^T W\left(\mathcal{K}_{i}\right) + b_i$, cela simplifierai tout ceci et serait plus concret.} 
{According to Proposition~\ref{prop:mu_unicity}, \eqref{eq:updateW} is a well-defined update from $(0,\infty)^Q$ to itself, provided that $\mu_j$ is tuned to $\mu_j^\star$. This brings us a structural guarantee that $D\left(\mathcal{B}_j\right) - \mu_j^\star  \gammab_j$ cannot cancel.}

Finally, we need to \revise{evaluate $\mu_j^\star$, which is uniquely determined on some interval $\left(-\infty, t \right)$ according to Proposition~\ref{prop:mu_unicity}. This amounts to solve $\gammab_j^{T} H^\star \left( \mathcal{B}_{j} \right)=c_j$. When $\beta\not\in(1,2)$, this is equivalent} to find the root of the function 
\begin{equation} \label{eq:fmulincstr} 
r_j(\mu_j)=\sum_{{q}=1}^{Q} \gamma_{j,{q}} \left[ \widetilde{H}\left(\mathcal{B}_{j}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{j}\right) \right]}{\left[ D\left(\mathcal{B}_{j}\right) - \mu_{j}  \gammab_j \right]} \right)^{. \eta \left( \beta \right)} \right]_{{q}}  -c_j , 
\end{equation}
where $\left[A\right]_{{q}}$ denotes the ${q}$-th entry of expression $A$.  
Indeed, $r_j(\mu_j)$ is a finite sum of elementary rational functions of $\mu_j$ and each of them is an increasing, convex function in $\mu_{j}$ over $\left(-\infty, t_{{q}}\right)$ with  $t_{{q}}=\frac{D_{{q}}\left(\mathcal{B}_{j}\right)}{\gamma_{j,{q}}}$ for each $q$. It is even completely monotone for all $\mu$ in $\left(-\infty, t_{{q}}\right)$
%\ngc{C'est pas $\mu$ ici?}
because $\eta\left( \beta \right)>0$~\cite{miller2001}. As a consequence $r_j(\mu_j)$ is also a completely monotone, convex increasing function of $\mu_{j}$ in $\left(-\infty, t \right)$, where $t=\text{min}\left( t_{{q}} \right)$. Finally, we can easily show that the function $r_j(\mu_j)$ changes of sign on the interval $\left(-\infty, t \right)$ by computing two limits at the closure of the interval. As $\mu^\star \in (-\infty,t)$, the update \eqref{eq:updateW} is nonnegative.
%\ji{Je pense qu'on peut encore raccourcir ce paragraphe en faisant reference aux propositions de la sous-section 2.2.} 
To evaluate $\mu^\star$, we use a Newton-Raphson method, with any initial point $\mu_0\in(\mu^\star,t)$, with a quadratic rate of convergence as demonstrated in Proposition~\ref{NR}. 
Algorithm~\ref{consDisBetaNMF} summarizes our method to tackle~\eqref{eq:betaNMFmodel} for all the $\beta$-divergences, \jiter{$\beta\not\in(1,2)$} which we refer to as disjoint-constrained $\beta$-NMF algorithm. The update for matrix $W$ can be derived in the same way, by symmetry of the problem. \revise{For $\beta\in(1,2)$, a case-by-case analysis could be carried out for the values of $\beta$ for which the minimizer of \eqref{eq:Gmu} takes a closed-form expression.}

%where $\mathcal{K}$ designates the full set of variables in $W$.
%\ngc{On pourrait parler du computational cost ici, et ne plus en parler après, ou dire que c'est similaire à ce cas c-à-d que le coût est dominé par les matrix-matrix products, et par par le caclul de $\mu^\star$.} 
 
 
 \begin{remark} 
 As noted above, the denominators of \eqref{eq:updateW} and \eqref{eq:fmulincstr} will be different from zero. This follows notably from our assumption 
 that $(W,H)>0$; see Propositions~\ref{prop:mingmu},~\ref{prop:mu_unicity} and~\ref{NR}. 
 This is a standard assumption in the NMF literature: the entries of $(W,H)$ are initialized with positive entries which ensures all iterates to remain positive. This is important because the MU cannot change an entry equal to zero~\cite{lin2007projected}; % voilà ;-) mais je ne sais pas d'où vient le terme 'zero locking phenomenon' initialement 
 this is the so-called zero-locking phenomenon.   This implies $C$ and $D$ in~\eqref{eq:updateW} and~\eqref{eq:fmulincstr} are positive matrices (as long as $V$ has at least one nonzero entry per row and column). 
 In practice, one should however be careful because some entries of $W$ and $H$ can numerically be set to zero (because of finite precision). Hence, in our implementation, we use the machine precision as a lower bound for the entries of $W$ and $H$, as recommended in~\cite{gillis2012accelerated}. 
 \end{remark}
 \color{black} 
 
 
 
\paragraph{Computational cost}  
The computational cost of Algorithm~\ref{consDisBetaNMF} is asymptotically equivalent to the standard MU for $\beta$-NMF, that is, it requires $\mathcal{O}\left(FNK \right)$ operations per iteration. Indeed, the complexity is mainly driven by matrix products required to compute $C$ and $D$; see~\eqref{eq:updateW}.  
To compute the roots of~\eqref{eq:fmulincstr} corresponding to $H$ using Newton-Raphson, each  iteration requires to compute  $r_j(\mu_j)/r_j'(\mu_j)$ for all $j$ which requires $\mathcal{O}(KN)$ operations (when every entry of $H$ appears in a constraint).  
Finding the roots therefore requires $\mathcal{O}(K N)$ operations times the number of Newton-Raphson iterations. By symmetry, it requires $\mathcal{O}(K F)$ operations to compute the roots corresponding to $W$. 
Because of the quadratic convergence, the number of iterations required for the convergence of the Newton-Raphson method is typically small, namely between 10 to 100 in our experiments using the stopping criterion 
$|r (\mu_j)| \leq 10^{-6}$ for all $j$.  
%Since $\min(F,N) \gg \mathcal{O}(1)$, on peut enlever, pas très précis  
Therefore, in practice, the overall complexity of Algorithm~\ref{consDisBetaNMF} is dominated by the matrix products that require $\mathcal{O}\left(FNK \right)$ operations. 
The same conclusions apply to the algorithms presented in 
Sections~\ref{sec_ssbetaNMF}, \ref{sec_minvolKLNMF} and~\ref{sec_nonlinear}, and this will be confirmed by our numerical experiments. 

\algsetup{indent=2em}
\begin{algorithm}[ht!]
\caption{$\beta$-NMF with disjoint linear constraints \label{consDisBetaNMF}}
\begin{algorithmic}[1] 
\REQUIRE A matrix $V \in \mathbb{R}^{F \times N}$, 
an initialization $H \in \mathbb{R}^{K \times N}_+$ and $W  \in \mathbb{R}^{F \times K}$, 
a factorization rank $K$, 
a maximum number of iterations, maxiter, 
a value for \jiter{$\beta\not\in(1,2)$}, and 
the linear constraints defined by 
$\mathcal{K}_{i}$, $\alphab_j$ and $b_i$ for $i=1,2,\dots,I$, and 
$\mathcal{B}_{j}$, $\gammab_j$ and $c_j$ for $j=1,2,\dots,J$.  
\ENSURE A rank-$K$ NMF $(W,H)$ of $V$ satisfying constraints in \eqref{eq:betaNMFmodel}. 
    \medskip  
\FOR{$it$ = 1 : maxiter}
    \STATE \emph{\% Update of matrix $H$} 
    \STATE $C \leftarrow W^{T}\left( \left( WH \right)^{.\left( \beta-2 \right) } \odot V \right)$
    \STATE $D \leftarrow W^{T}\left( WH\right)^{.\left( \beta-1 \right) }$
    \FOR{$j = 1 : J$}
            \STATE $\mu_{j} \leftarrow \text{root}\left( r_j(\mu_j) \right)$ \quad \emph{\% see Equation~\eqref{eq:fmulincstr} }
            \STATE $H\left(\mathcal{B}_{j}\right) \leftarrow H\left(\mathcal{B}_{j}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{j}\right) \right]}{\left[ D\left(\mathcal{B}_{j}\right) -  \mu_{j}  \gamma_j \right]} \right)^{.\left( \eta \left( \beta \right)\right)}$
    \ENDFOR
    \STATE $\mathcal{B}_{c} = \{ (k,n) \ | 1 \leq k  \leq K, 1 \leq n \leq N \} \; \backslash \; \big(\cup_{j}^{J} \mathcal{B}_{j} \big).$ \quad \emph{\% $\mathcal{B}_{c}$ is the complement of $\cup_{j}^{J} \mathcal{B}_{j}$  }
    
    \STATE $H\left(\mathcal{B}_{c}\right) \leftarrow H\left(\mathcal{B}_{c}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{c}\right) \right]}{\left[ D\left(\mathcal{B}_{c}\right) \right]} \right)^{. \eta \left( \beta \right)}$
	\STATE \emph{\% Update of matrix $W$}
    \STATE $W$ is updated in the same way as $H$, by symmetry of the problem. 
\ENDFOR
\end{algorithmic}  
\end{algorithm} 



==> arXiv v2/Chapters/2_betaNMF2310.tex <==
% \ngc{Je pense que cette section nécessite un ``serious facelift'' (j'utilise l'expression utilisée un jour par un reviewer).}

% \ngc{Je propose la chose suivante: 
% Avant de mettre `This section is organized as follows', il faut bien réexpliquer le contexte. On veut résoudre $\beta$-NMF avec pénalités et contraintes linéaires disjointes: donner le modèle général~\eqref{eq:betaNMFmodel} et introduire les notations. On voit ainsi directement ce qu'on veut faire/résoudre. 
% Ensuite, comme on fait de l'alterné, montrer que les sous-problèmes à résoudre ont la forme de~\eqref{eq:subprobleminW} et donc~\eqref{eq:minF}. 
% Finalement, donner la structure de la section.  
% }

% \ngc{Je le laisse retravailler cela et je relis après. J'ai mis d'autres commentaires également dans la section.}  

In this paper, we introduce a general framework to tackle $\beta$-NMF with disjoint linear equality constraints, and with penalty terms in the objective function. Let us first introduce specific notations: given a matrix $A \in \mathbb{R}^{F \times N}$ and a list of indices $\mathcal{K} \subseteq \{ (f,k) \ | \ 1 \leq f \leq F, 1 \leq n \leq N\}$, we denote $A(\mathcal{K})$ the vector of dimension $|\mathcal{K}|$ whose entries are the entries of $A$ corresponding to the indices within $\mathcal{K}$. 
Let us introduce $\mathcal{K}_{i}$ ($1 \leq i \leq I$) and $\mathcal{B}_{j}$ ($1 \leq j \leq J$) to be disjoint sets of indices for the entries of $W$ and $H$, respectively, that is, 
\begin{itemize}

    \item $\mathcal{K}_{i} \subseteq \{ (f,k) \ | \ 1 \leq f \leq F, 1 \leq k \leq K\}$ for  $i = 1,2,\dots,I$, 
    
    \item $\mathcal{B}_{j} \subseteq \{ (k,n) \ | \ 1 \leq k \leq K, 1 \leq n \leq N\}$ for $j = 1,2,\dots,J$,
    
    
    \item $\mathcal{K}_{u} \cap \mathcal{K}_{v} = \emptyset$ for all $1 \leq u,v \leq I$ and $u \neq v$,
    
    \item $\mathcal{B}_{q} \cap \mathcal{B}_{p} = \emptyset$ for all $1 \leq q,p \leq J$ and $q \neq p$. 
\end{itemize} 
We now define penalized $\beta$-NMF with disjoint linear equality constraints as follows 
\begin{equation}\label{eq:betaNMFmodel}
\begin{aligned}
& \underset{W\in \mathbb{R}^{F \times K}_+,H\in \mathbb{R}^{K \times N}_+}{\min}
& & D_{\beta}\left(V|WH\right) + \lambda_1 \Phi_1(W) + \lambda_2 \Phi_2(H) \\
& \text{such that}
%& & H \geq 0, W \geq 0, \\
%& \text{}
& & \alphab_i^{T} W \left( \mathcal{K}_{i} \right) = b_i \text{ for } 1\leq i \leq I, \\
& \text{}
& &  \gammab_j^{T} H \left( \mathcal{B}_{j} \right) = c_j \text{ for } 1\leq j \leq J,
\end{aligned}
\end{equation}
where %$D_{\beta}\left(V|WH\right)=\sum_{f,n} d_{\beta}(V_{fn}|[ \,WH] \,_{fn})$, 
\begin{itemize}
    \item the penalty functions $\Phi_1(W)$ and $\Phi_2(H)$ are separable functions\footnote{\ngi{This assumption is not strictly necessary, but is made because it greatly simplifies the presentation. It can be relaxed to the requirement that $\Phi_1(W)$ and $\Phi_2(H)$ possess an entry-wise quadratic separable majorizer of the form given in~\eqref{eq:Lipschtiz_case}. 
    This will be the case for our example in Section~\ref{sec_minvolKLNMF} where $\Phi_1(W) = \logdet(W^T W + \delta I)$ satisfies only the latter assumption.}} w.r.t.\ the rows of $W$ and columns of $H$,  respectively, that is, we have  
    $\Phi_2(H) = \sum_{n=1}^N \Phi_2(\hb_n)$ where $\hb_n \in \mathbb{R}_+^{F}$ denotes the $n$-th column of $H$, and similarly for $\Phi_1$. We will also need that $\Phi_1$ and $\Phi_2$ are concave, or admit an $L$-smooth gradient;  see Assumption~\ref{ass:phi} below. 
    
    \item $\lambda_1$ and $\lambda_2$ are the penalty weights (nonnegative scalars). 
    
    \item $\alphab_i \in \mathbb{R}^{|\mathcal{K}_i|}_{++}$ ($1\leq i \leq I$) and $\gammab_j \in \mathbb{R}^{|\mathcal{B}_j|}_{++}$ ($1\leq j \leq J$) are vectors with positive entries. 
    Note that if $\alphab_i$ or $\gammab_j$ contains zero entries,  the corresponding indices can be removed from $\mathcal{K}_{i}$ and $\mathcal{B}_{j}$.  
    
    \item $b_i$ ($1\leq i \leq I$) and $c_j$  ($1\leq j \leq J$) are positive scalars. 
\end{itemize}
% We denote by $\Psi$ the objective function 
% of~\eqref{eq:betaNMFmodel}, that is, 
% \[
% \Psi (W,H) = 
% D_{\beta}\left(V|WH\right) + \lambda_1 \Phi_1(W) + \lambda_2 \Phi_2(H). 
% \] 
%\ngc{(1) on a vraiment besoin qu'elles soient séparables? On montre justement plus bas comment s'en sortir si ce n'est pas le cas, non? Je pense qu'il faut juste qu'elles soient séparables par lignes de $W$ / colonnes de $H$, non? (2)  il faudrait de toute façon définir séparable.} \ngc{C'est la même pénalité sur $W$ et $H$? Ce n'est pas ce qu'on fait dans les exemples... Utiliser $\lambda_2 \Phi_2(H)$? Si c'était la même pénalité, il faudrait d'ailleurs plutôt utiliser  $\Phi_1(H^T)$ pour avoir la symmétrie.}  

As for most NMF algorithms, we propose to resort to a  block coordinate descent (BCD) framework 
to solve problem~\eqref{eq:betaNMFmodel}: at each iteration we tackle two sub-problems separately; one in $W$ and the other in $H$. 
% \algsetup{indent=2em}
% \begin{algorithm}[ht!]
% \caption{BCD framework to tackle NMF optimization problems \label{algo:metaalgo} }
% \begin{algorithmic}[1]
% \REQUIRE Input matrix $V \in \mathbb{R}^{F \times N}_+$, the factorization rank $K$ and
%  number of iterations maxiter. 
% \ENSURE $(W,H)$ is an approximate solution of~\eqref{eq:betaNMFmodel}. 
%     \medskip  
% \STATE Initialize $(W^{0}, H^{0}) \in \mathbb{R}^{F \times K}_+ \times \mathbb{R}^{K \times N}_+$. 
% \FOR {$k=1,2,\dots,$ maxiter}
%     \STATE \emph{\% Update $W$} 
%     \STATE $W^{k} \longleftarrow \text{update} (V,W^{k-1},H^{k-1}) \text{ typically such that }\Psi(W^{k},H^{k-1}) \leq \Psi(W^{k-1},H^{k-1})$ 
%     \STATE \emph{\% Update $H$} 
%     \STATE $H^{k} \longleftarrow \text{update} (V,W^{k},H^{k-1}) \text{ typically such that }\Psi(W^{k},H^{k}) \leq \Psi(W^{k},H^{k-1})$  
% \ENDFOR
% \end{algorithmic}
% \end{algorithm}  
The subproblems in $W$ and $H$ are essentially the same, by symmetry of the model. Hence, we may focus on solving the  subproblem in $H$ only, namely 
\begin{equation}
\label{eq:betaNMFmodelH}
 \underset{H\in \mathbb{R}^{K \times N}_+}{\min}
 D_{\beta}\left(V|WH\right) + \lambda_2 \Phi_2(H) 
\quad \text{ such that } \quad 
 \gammab_j^{T} H \left( \mathcal{B}_{j} \right)=c_j \text{ for } 1\leq j \leq J. 
\end{equation} 
In order to tackle~\eqref{eq:betaNMFmodelH}, we will design MU based on the majorization-minimization (MM) framework~\cite{sun2017majorization}, which is the standard in the NMF literature; see~\cite{Fevotte_betadiv} and the references therein. 
It consists in two steps: find a function that is an upper approximation of the objective and is tight at the current iterate, which is referred to as a majorizer, 
then minimize the majorizer to obtain the next iterate. This guarantees the objective function to decrease at each step of this iterative process. 


To do so, we first provide a majorizer for the objective of~\eqref{eq:betaNMFmodelH} in Section~\ref{sec:majorizer}. This majorizer has the property to be separable in each entry of $H$. In order to handle the equality constraints, 
we introduce Lagrange dual variables in Section~\ref{sec:lagrange}, and explain how they can be computed efficiently. 
This allows us to derive general MU in Section~\ref{betanmf_disjointconstraint} in the case of non-penalized $\beta$-NMF under disjoint linear equality constraints.
 This is showcased on simplex-structured $\beta$-NMF in Section~\ref{sec_ssbetaNMF}. In Section~\ref{sec_minvolKLNMF}, we will illustrate on minimum-volume NMF  how to derive MU in the presence of penalty terms. 



%and then derive the proposed MU for~\eqref{eq:betaNMFmodelH} in Section~\ref{}.   


\subsection{Separable majorizer for the objective function} 
\label{sec:majorizer} 

The objective function of~\eqref{eq:betaNMFmodelH} can be decoupled into $n$ independent terms, one for each column $\hb_n$ of $H$: 
\begin{equation}
\label{eq:psi(H)}
\psi(H) := D_{\beta}\left(V|WH\right) + \lambda \Phi(H) = \sum_{n=1}^N \psi(\hb_n), 
\end{equation}
\ji{where $\psi(\hb_n) = D_{\beta}\left(\vb_n|W\hb_n\right) + \lambda \Phi(\hb_n)$.}
Note that, to simplify the notation, we write $\Phi_2(H) = \Phi(H)$, and $\lambda = \lambda_2$.  
Let us focus on a specific column of $H$, denoted $\hb \in \mathbb{R}^K_+$, and 
let us majorize the function $\psi(\hb)$. % = D_{\beta}\left(v|Wh\right) + \lambda \Phi(h)$.
Given any $\widetilde{\hb}\geq 0$ of the same dimension as $\hb$, we need to find a majorizer $G\big(\hb|\tilde{\hb}\big)$ such that 
\begin{enumerate}
    \item $G\big(\hb|\widetilde{\hb}\big)  \geq \psi(\hb)$ for all $\hb$, and 

    \item $G\big(\widetilde{\hb}|\widetilde{\hb}\big)  = \psi\big(\widetilde{\hb}\big)$.
\end{enumerate}
%Now, let us provide a majorizer $G\big(\hb|\widetilde{\hb}\big)$ for $\psi(\hb)$ 
This can be done by majorizing $D_{\beta}(\vb|W\hb)$ and $\Phi(\hb)$ separately: 
\begin{itemize}
%\item The first term $D_{\beta}\big(v|Wh\right)$ is upper bounded using decomposition of $d_{\beta}$ presented in  Appendix~\ref{convconcacm}. It follows the methodology introduced in \cite{Fevotte_betadiv} to upper bound the convex and the concave terms. It is given by  
\item The first term $D_{\beta}(\vb|W\hb)=\sum_{f=1}^F d_{\beta}(v_f|(W\hb)_f)$ is upper bounded following the methodology introduced in \cite{Fevotte_betadiv}, \ji{which consists in applying a convex-concave procedure \cite{Yuille03} to $d_{\beta}$}, as presented in Appendix~\ref{convconcacm}. The resulting upper bound is given by
%
\begin{equation}
\label{eqn:auxbeta}
d_{\beta}(v_f|(W\hb)_f) \leq
\sum_{k=1}^K \frac{w_{fk}\widetilde{h}_k}{\widetilde{v}_f}\widecheck{d} \left( v_f |  \widetilde{v}_f \frac{h_k}{\widetilde{h}_k} \right)
+ \widehat{d}'\big(v_f|\widetilde{v}_f\big) \sum_{k=1}^K w_{fk} \big(h_k - \widetilde{h}_k\big)
+ \widehat{d}\big(v_f | \widetilde{v}_f\big), 
\end{equation}
where $\widetilde{v}_f = \big(W \widetilde{\hb}\big)_f$, and $\widehat{d}$ and $\widecheck{d}$ are the concave and convex parts of $d$, respectively. %\ngc{C'est correct?} 

\item For the second term $\Phi(\hb)$, we will rely on the following assumption for $\Phi$. 
\begin{assumption} \label{ass:phi}
The function 
$\Phi : \mathbb{R}^K_+ \mapsto \mathbb{R}$ %_\ngi{+}$
\jibis{is lower-bounded, and} it is either concave or has an $L$-Lipschitz continuous gradient. 
\end{assumption}
Let us consider the two cases separately:
\begin{enumerate}
    \item If $\Phi$ is concave, an upper approximation can be obtained using the first-order Taylor approximation of $\Phi$ at $\widetilde{\hb}$: 
%
\begin{equation}
\label{eq:concave_case}
\Phi(\hb)\leq\Phi\big(\widetilde{\hb}\big)+\left\langle\nabla\Phi\big(\widetilde{\hb}\big),\hb-\widetilde{\hb}\right\rangle . 
\end{equation}
%
Moreover,
\begin{equation}
\label{eq:geq0}
\nabla\Phi\big(\widetilde{\hb}\big) \geq 0,
\end{equation}
otherwise we would have $\lim_{y\rightarrow\infty}\Phi\big(\widetilde{\hb}+y\eb_j\big)=-\infty$ because of the concavity of $\Phi$, where $\eb_j$ is the $j$th unit vector. This would contradict the \jibis{fact that $\Phi$ is bounded from below.} %nonnegativity of $\Phi$. %\ngc{Où a-t-on supposé que $\Phi$ est nonnégatif? Mhmh... cela est-il le cas de fonctions concaves intéressantes? On a quoi en tête comme type de fonction à part du linéaire ($\ell_1$ penalty) en fait? J'avoue ne pas y avoir réfléchis avant.}   
%\ngc{Why is this important? Il faudrait expliquer.} 
\ngi{Examples of such penalty functions include \jibis{sparsity-promoting regularizers} $\Phi(\hb) = \| \hb \|_p^p =  \sum_k \hb_k^p$ for $0 < p \leq 1$ since $\hb \geq 0$.} %that promote the sparsity of $\hb$.}   

\item If $\Phi$ has an $L$-Lipschitz continuous gradient, we have: 
%
\begin{equation}
\label{eq:Lipschtiz_case}  
\Phi(\hb)\leq\Phi\big(\widetilde{\hb}\big)+\left\langle\nabla\Phi\big(\widetilde{\hb}\big),\hb-\widetilde{\hb}\right\rangle+\frac{L}2\big\|\hb-\widetilde{\hb}\big\|^2,
\end{equation}
%
for some constant $L > 0$, according to the descent lemma~\cite{Bertsekas99}. %\ngc{don't we need convexity here?}
\jibis{Examples of such penalty functions include any smooth convex functions;} \ngi{for example any quadratic penalty, such as   $||A \hb - b||_2^2$ for some matrix $A$ and vector $b$ in which case $L = \sigma_1(A)^2$.} 

%the \emph{minimum-volume} regularizer $\text{vol}(W)=\logdet(W^{T}W+\delta I)$ with $\delta>0$ (see \cite{9084229} and Section~\ref{sec_minvolKLNMF}).}
%\jibis{Section~\ref{sec_minvolKLNMF}, ça serait bien d'indiquer ce que vaut $L$. Logiquement, ce $L$ intervient dans l'algorithme, ce qu'on ne voit pas explicitement dans la Section~\ref{sec_minvolKLNMF}}
 

%\ngc{Je ne comprends pas le but de cette phrase ni ce que cela facilite... Pour $L=0$, la pénalité est linéaire et donc concave effectivement mais c'est un cas assez particulier...} 

\end{enumerate}

Interestingly \eqref{eq:concave_case} is a special case of  \eqref{eq:Lipschtiz_case} by taking $L=0$. This allows us to tackle these two classes of penalty functions in an unified way in what follows. Note that the result given by equation~\eqref{eq:geq0} is used further for the proof of Proposition~\ref{prop:mingmu} and is only valid for the special case $L=0$.

\end{itemize}


%\ngc{Par contre, on a pas $\nabla\Phi\big(\widetilde{\yb}\big) \geq 0$ pour le cas Lipschitz, non?-> en effet mais le résultat n'est utilisé plus tard que pour un cas particulier où L=0} 

\ji{For each column $\hb$ of $H$, a majorizer $G\big(\hb|\widetilde{\hb}\big)$ of $\psi(\hb)$ is obtained by combining \eqref{eqn:auxbeta} and \eqref{eq:Lipschtiz_case}. Finally, according to~\eqref{eq:psi(H)}, we obtain a majorizer $G\big(H|\widetilde{H}\big)$ for $\psi(H)$ as a sum of column-wise majorizers. The result is obviously separable into a sum of $K\times N$ component-wise majorizers, up to an additive constant:
%
\begin{equation}
%\label{eq:G}
G\big(H|\widetilde{H}\big) 
= \sum_{n=1}^N\sum_{k=1}^K g\big(h_{kn}|\widetilde{\hb}_n\big) + C\big(\widetilde{H}\big),
\end{equation}
where
\begin{align}
\label{eq:Gkn}
g\big(h_{kn}|\widetilde{\hb}_n\big) &= \sum_{f=1}^F \frac{w_{fk}\widetilde{h}_{kn}}{\widetilde{v}_{fn}}\widecheck{d} \left( v_{fn} |  \widetilde{v}_{fn} \frac{h_{kn}}{\widetilde{h}_{kn}} \right)
+ a h_{kn}^2 + p_{kn} h_{kn},
\\
C\big(\widetilde{H}\big) &= \sum_{n=1}^N\sum_{f=1}^F\left(\widehat{d}\big(v_{fn} | \widetilde{v}_{fn}\big)
- \sum_{k=1}^K\widehat{d}'\big(v_{fn}|\widetilde{v}_{fn}\big) w_{fk} \widetilde{h}_{kn}\right),
\notag
\end{align}
with $a=\lambda\frac{L}{2}$ and
\begin{equation*}
p_{kn}=\sum_{f=1}^F w_{fk}\widehat{d}'\big(v_{fn}|\widetilde{v}_{fn}\big) +\lambda\left(\frac{\partial \Phi}{\partial h_{kn}}\big(\widetilde{\hb}_n\big)- L\widetilde{h}_{kn}\right).
\end{equation*}
}
%Finally, it is important to note that the majorizer $G(h|\widetilde{h})$ of $\psi(h)$, obtained  by combining \eqref{eqn:auxbeta} and \eqref{eq:Lipschtiz_case}, is separable, that is, it can be written in the form 
%\[
%G(h|\widetilde{h}) 
%= \sum_{k=1}^K G_k(h_k|\widetilde{h}_k),
%\] 
%see~\eqref{eq:gj} in the next section for the expression of $G_k$.
This will allow us to minimize the majorizer under the equality constraints efficiently, as presented in the next section.  



\subsection{Dealing with equality constraints via Lagrange dual variables}  \label{sec:lagrange} 

In the previous section, we derived a majorizer for $\psi(H)$, $G\big(H|\widetilde{H}\big)$, which is separable in each entry of $H$. Without the equality constraints, we could then compute closed-form solutions to univariate problems to minimize $G\big(H|\tilde{H}\big)$ to obtain the standard MU for NMF as in~\cite{Fevotte_betadiv}. 

However, in problem~\eqref{eq:betaNMFmodelH}, the entries of $H$ in the subsets $\mathcal{B}_j$ are not independent as they are linked with the equality constraints $\gammab_j^{T} H ( \mathcal{B}_{j})=c_j$ for $j = 1,2,\dots,J$. 
In fact, to minimize the majorizer under the equality constraints, we need to solve 
%
\begin{equation}
\label{eq:betaNMFmodelHmajor}
\underset{H\in \mathbb{R}^{K \times N}_+}{\min}
 G\big(H|\widetilde{H}\big) 
\quad  \text{ such that } \quad 
\gammab_j^{T} H (\mathcal{B}_{j})=c_j \text{ for } 1\leq j \leq J. 
\end{equation} 
%
The variables in different sets $\mathcal{B}_j$ can be optimized independently, as they do not interact in the majorizer nor in the constraints. Note that, for the entries of $H$ that do not appear in any constraints, the standard MU~\cite{Fevotte_betadiv} can be used. 
For simplicity, let us fix $j$ and 
denote $\mathcal{B}=\mathcal{B}_j$, $L = |\mathcal{B}|$, 
$\yb = H(\mathcal{B}) \in \mathbb{R}^{L}_{+}$, $\gammab = \gammab_j \in \mathbb{R}^{L}_{++}$, 
and $c = c_j > 0$.  
The problems we need to solve have the form 
\begin{equation}
\label{eq:minG}
\min_{\yb \in \Yc} G\big(\yb | \widetilde{H} \big), 
\end{equation} 
where $\Yc=\left\{\yb \in \mathbb{R}^{L}_+ \ | \ \gammab^T\yb=c \right\}$
\ji{and
\begin{equation}
\label{eq:Gy}
G\big(\yb | \widetilde{H}\big)=\sum_{(k,n)\in \mathcal{B}}g\big(h_{kn}|\widetilde{\hb}_n\big),
\end{equation} 
where the component-wise majorizers $g\big(h_{kn}|\widetilde{\hb}_n\big)$ are defined by~\eqref{eq:Gkn}. Using a more convenient notation, let us rewrite~\eqref{eq:Gy} as $G\big(\yb | \widetilde{H}\big)=\sum_{\ell=1}^L g\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$, where $n(\ell)$ is the first element of any pair $\ell\in\mathcal{B}$, while $k(\ell)$ will denote the second element.}
%
%Recall that $G(\yb | \widetilde{\yb} )$ is separable, that is, 
%$$
%G(\yb|\widetilde{\yb}) 
%= \sum_{\ell = 1}^L g(y_\ell|\widetilde{\yb}) + C,
%$$
%where $C$ is a constant, and each component $g$ is given by: 
%\begin{align}
%g(y_\ell|\widetilde{\yb})&=\sum_{f=1}^F \frac{w_{fk(\ell)}\widetilde{\yb}_\ell}
%{\widetilde{v}_f}\widecheck{d} \big( v_f | \widetilde{v}_f \frac{y_\ell}{\widetilde{y}_\ell} \big) + a y_\ell^2 + p_\ell y_\ell,
%\label{eq:gj}
%\end{align}
%%
%\ngc{J'ai changé $b$ par $p$ car je l'utilisais pour les contraintes linéaires en $W$; cf. (2)}
%with $a=\lambda\frac{L}{2}$, 
%%
%\begin{equation}
%\label{eq:pell}
%p_\ell=\sum_{f=1}^F w_{fk(\ell)}\widehat{d}'(v_f|\widetilde{v}_f) +\lambda\big(\frac{\partial \Phi}{\partial y_\ell}(\widetilde{\yb})- L\widetilde{\hb}_{n(\ell)\big), 
%\end{equation}
%and the constants $w_{fk(\ell)}$ correspond to entries of $W$ and are assumed to be positive. \ngc{Il faudrait mieux les définir, je suppose que $z$ peut être construit à partir de $W$, mais ce serait intéressant d'écrire la formule explicitement.}    
%
%In order to solve \eqref{eq:minF} using an iterative majorization-minimization scheme, let us consider the constrained problem
%\begin{equation}
%\label{eq:minG}
%\min_{\yb\in \Yc} G(\yb|\widetilde{\yb}).
%\end{equation}
The corresponding Lagrangian function reads
\ji{
\begin{equation}
\label{eq:Gmuy}
    G^\mu\big(\yb|\widetilde{H}\big)  
    = G\big(\yb|\widetilde{H}\big)-\mu(\gammab^T\yb-c) 
    = \mu c + C\big(\widetilde{H}\big) + \sum_{\ell=1}^L g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big), 
\end{equation}
%\ngc{Faire attention avec les sommes indicées: cela peut prêter à confusion. Je préfère 
%$\mu c + C + \sum_{\ell=1}^L g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$.} 
where
%---------------------------
\begin{align}
g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)&=g\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)-\mu \gamma_\ell\,y_\ell\notag\\
&= \sum_{f=1}^F \frac{w_{fk(\ell)}\widetilde{y}_\ell}{\widetilde{v}_{fn(\ell)}}\widecheck{d} \left( v_{fn(\ell)} |  \widetilde{v}_{fn(\ell)} \frac{y_\ell}{\widetilde{y}_\ell} \right)
+ a y_\ell^2 + (p_\ell-\mu \gamma_\ell) y_\ell,
\label{eq:gmu}
\\
p_\ell&=\sum_{f=1}^F w_{fk(\ell)}\widehat{d}'\big(v_{fn(\ell)}|\widetilde{v}_{fn(\ell)}\big) +\lambda\left(\frac{\partial \Phi}{\partial y_\ell}\big(\widetilde{\hb}_{n(\ell)}\big)- L\widetilde{y}_\ell\right), 
\label{eq:pell}
\end{align}
}
and $\mu\in\mathbb{R}$.
Note that $G^\mu$ is separable, as is $G$, because the term $\gammab^T \yb$ is linear. 
%for any fixed value for $\mu$, $G^{\mu}$ \eqref{eq:Gmuy} is a separable approximation of the Lagrangian function $\Psi(\yb)-\mu(\gammab^T\yb-c)$.

Assume for now that the Lagrangian multiplier $\mu$ is known, and let us minimize $G^\mu\big(\yb|\widetilde{H}\big)$ on $(0,\infty)^L$. 
Such a problem is separable under the form of $L$ subproblems, consisting in minimizing univariate functions  $g^\mu\big(\cdot|\widetilde{\hb}_{n(\ell)}\big)$ separately over $(0,\infty)$. We now show in Proposition~\ref{prop:mingmu} that, under mild conditions, each subproblem admits a unique solution over $(0,\infty)$. %Let us emphasise the fact that in Proposition~\ref{prop:mingmu}, we assume that the optimal value for $\mu$ is known. 
%to be minimized on $y\in(0,\infty)$, where $\mu\in\mathbb{R}$.
%
%---------------------------
\begin{proposition}
\label{prop:mingmu}
%\ngc{Je pense que pour cette proposition, il faut considérer un seul $\ell$: j'ai modifié, please check :-)}
Let $\ell \in \{1,2,\dots,L\}$. 
Assume that $\beta<2$ and $\widetilde{y}_\ell,v_{fn(\ell)},w_{fk(\ell)}>0$ for all $f$.
%\ngc{Vérifier les indices... Faut-il vraiment que $V>0$? Cela parait restrictif...}
Moreover, if $\beta\leq1$ and $a=0$, assume that $\mu<\frac{p_\ell}{\gamma_\ell}$. 
Then there exists a unique minimizer $y_\ell^\star(\mu)$ of $g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ in $(0,\infty)$.  
\end{proposition}
%---------------------------

%
\begin{proof}
According to Proposition~\ref{prop:approxdbeta} (see Appendix~\ref{convconcacm}), each $g^\mu$ is $C^\infty$ and strictly convex on $(0,\infty)$, so its infimum is uniquely attained in the closure of $(0,\infty)$. We have to prove that it is neither reached at $0$ nor at $\infty$.

On the one hand, \ji{from \eqref{eq:gmu}, we have 
%
\begin{equation}
\label{eqgmu'}
(g^\mu)'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=\sum_{f=1}^F w_{fk(\ell)}\widecheck{d}' \left( v_{fn(\ell)} | \widetilde{v}_{fn(\ell)}\frac{y_\ell}{\widetilde{y}_\ell} \right) +2a y_\ell + p_\ell -\gamma_\ell\mu
\end{equation}
}%
and, for any $\beta<2$ and any $x>0$,
%
\begin{equation}
\label{eq:d'0}
\lim_{y\rightarrow0^+}\widecheck{d}'(x|y)=-\infty,\\
\end{equation}
%
so $\lim_{y_\ell\rightarrow0^+}(g^\mu)'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=-\infty$, which ensures that the infimum is not reached at $0$.
%\ji{This would not apply to the case $\beta\geq2$. Things are probably OK then if $\lambda=0$, but I have decided to discard the case $\beta\geq2$ for the sake of coherence, and because it is not of great interest from the application viewpoint. This could maybe deserve a comment somewhere (but we should first check the calculations when $\beta\geq2$).}

On the other hand,
%
\begin{equation}
\lim_{y\rightarrow\infty}\widecheck{d}'(x|y)=\begin{cases}0&\text{if } \beta\leq1,\\\infty&\text{otherwise.}\end{cases}
\label{eq:d'inty}
\end{equation}
%
According to \eqref{eqgmu'} and \eqref{eq:d'inty}, the distinction must be made between two cases:
%
\begin{itemize}
\item If $a>0$ or $\beta\in(1,2)$: $\lim_{y_\ell\rightarrow\infty}(g^\mu)'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=\infty$, so the infimum is reached at a finite value of $y_\ell$.
\item If $a=0$ and $\beta\leq1$: $\lim_{y_\ell\rightarrow\infty}(g^\mu)'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=p_\ell -\gamma_\ell\mu$, so the same conclusion holds if and only if $\mu<\frac{p_\ell}{\gamma_\ell}$. 
\end{itemize}
\end{proof}
We just proved that, under mild conditions, each $g^\mu$ has a unique minimizer over $(0,\infty)$.
%\ngc{Discuter la condition $\mu<\frac{p_\ell}{\gamma_\ell}$?} 
However we assumed that the value of $\mu$ is fixed.  
Now given $\yb^\star(\mu)=\big[y_1^\star(\mu),\ldots,y_L^\star(\mu)\big]^T$, let us show 
that the solution to $\gammab^T \yb^\star(\mu) =c$ is unique. The corresponding value of $\mu$, which we denote  $\mu^\star$, provides  the minimizer $\yb^\star(\mu^\star)$ of $G^\mu(\yb|\widetilde{H})$ that satisfies the linear constraint $\gammab^T\yb^\star(\mu^\star)=c$. \ji{Moreover, $\mu^\star$ naturally fulfills $\mu^\star<\frac{p_\ell}{\gamma_\ell}$ for all $\ell$ when $\beta\leq1$ and $a=0$, as required in Proposition~\ref{prop:mingmu}.}
%Finally, we prove that $\mu^\star$ is unique on some specific interval under mild conditions. 
%\sout{further}
%Let us remark that, at this stage, $\yb^\star$ is a vector function of $\mu$.
%
%---------------------------
\begin{proposition}
\label{prop:mu_unicity}
Assume that $\beta<2$ and $\widetilde{y}_\ell, v_{fn(\ell)},w_{fk(\ell)}>0$ for all $\ell,f$, %\ngc{Vérifier les indices}
%and let $y_\ell^\star(\mu)$ be the unique minimizer of  $g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ in $(0,\infty)$ as defined in Proposition~\ref{prop:mingmu}, for $\ell=1,2,\dots,L$. %\ngc{Ne doit-on pas indiquer les conditions sur $\mu$ comme dans la Proposition 1: $\mu < \min_{\ell} \frac{c_\ell}{\gammab_l}$ when $\beta \le 1$ et $a=0$?} 
%=(y_1^\star,\ldots,y_P^\star)^T$.  
Then the scalar equation $\gammab^T \yb^\star(\mu) =c$ in the variable $\mu$ admits a unique solution $\mu^\star$ in $(-\infty,t)$, where
$$
t=\begin{cases}\ji{\min_\ell \frac{p_\ell}{\gamma_\ell}}\geq0&\text{if $\beta\leq1$ and $a=0$},\\\infty&\text{otherwise,}\end{cases}
$$
such that $\yb^\star(\mu^\star)$ is the unique solution to problem~\eqref{eq:minG}.
\end{proposition}
%---------------------------
\begin{proof}
Under the conditions of Proposition~\ref{prop:mingmu}, $g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ has a unique minmizer $y^\star_\ell(\mu)$ for each $j$.  
%\ngc{A rephraser. Veux-tu dire que: 
%According to Proposition~\ref{prop:mingmu}, $g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ has a unique minmizer for each $j$, which we denote $y^\star_\ell$.} 
By the first-order optimality condition, $y^\star_\ell(\mu)$ is a solution of $(g^\mu)'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=0$ or equivalently, by \eqref{eqgmu'}, a solution of $\gamma_\ell^{-1}g'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=\mu$ over $(0,\infty)$ where 
%
\begin{equation}
\label{eq:g'}
\gamma_\ell^{-1}g'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=\gamma_\ell^{-1}\sum_{f=1}^F w_{fk(\ell)}\widecheck{d}' \left( v_{fn(\ell)} | \widetilde{v}_{fn(\ell)} \frac{y_\ell}{\widetilde{y}_\ell} \right) +2 \frac{a_\ell}{\gamma_\ell}y_\ell + \frac{p_\ell}{\gamma_\ell}
\end{equation}
%
is strictly increasing on $(0,\infty)$ (since $g$ is strictly convex) and one-to-one from $(0,\infty)$ to an open interval
$T_\ell=(t^-_\ell,t^+_\ell)$ where
%
\begin{align}
t^-_\ell&=\lim_{y_\ell\rightarrow0}g'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)=-\infty,\\
t^+_\ell&=\lim_{y_\ell\rightarrow\infty}g'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)
=\begin{cases}\frac{p_\ell}{\gamma_\ell}&\text{if $\beta\leq1$ and $a=0$,}\\\infty&\text{otherwise.}\end{cases}
\end{align}
%
Moreover, $p_\ell\geq0$ if $a=0$ (then $L=0$) and $\beta\leq1$ according to~\eqref{eq:geq0} and \eqref{eq:pell}.
As a consequence, $\gamma_\ell^{-1}g'(y_\ell^\star|\widetilde{y}_\ell)=\mu$ is equivalent to
\begin{equation}
\label{eq:yhat}
y_\ell^\star = \big(g'\big)^{-1}(\gamma_\ell\mu),
\end{equation}
where $\mu\in T_\ell$ and $\big(g'\big)^{-1}$ denotes the inverse function of $g'$.

Coming back to the multivariate problem~\eqref{eq:minG}, we must find a value $\mu^\star$ of the Lagrangian multiplier such that the constraint $\gammab^T\yb^\star(\mu)=c$ is satisfied. Given~\eqref{eq:yhat}, $\mu^\star$ is a solution of
%
\begin{equation}
\label{eq:muhat}
\sum_{\ell=1}^L \gamma_\ell\big(g'\big)^{-1}(\gamma_\ell\mu)=c.
\end{equation}
%
Each $g'\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ being strictly increasing on $(0,\infty)$, $(g')^{-1}(\gamma_\ell\mu)$ is also strictly increasing (from $T_\ell$ to $(0,\infty)$), this is a direct consequence of $(f^{-1})'=\frac1{f' \circ f^{-1}}$ where $f$ is any strictly increasing function on some interval. Finally $\sum_{\ell=1}^L \gamma_\ell(g')^{-1}(\gamma_\ell\mu)$ is strictly increasing from $\cap_{j=1}^J T_\ell=(-\infty,t)$ to $(0,\infty)$, with $t\geq0$. Therefore, the solution $\mu^\star$ is unique. 
\end{proof}

 Proposition~\ref{prop:mu_unicity} shows that the optimal Lagrangian multiplier is the unique solution of \eqref{eq:muhat}. It is clear that finding the solution of \eqref{eq:muhat} is equivalent to finding the root of a function $r(\mu)$. We propose here-under to use a Newton-Raphson method to compute $\mu^\star$, and show that this method generates a sequence of iterates $\mu_n$ that converges towards $\mu^\star$ at a quadratic speed.

%---------------------------
\begin{proposition}
\label{NR}
Assume that $\beta<2$ and $\widetilde{y}_\ell,v_{fn(\ell)},w_{fk(\ell)}>0$ for all $\ell,f$. %\ngc{Vérifier les indices}
Let
$$
r(\mu)=\sum_{\ell=1}^L \gamma_\ell(g')^{-1}\big(\gamma_\ell\mu\big)-c
$$
for $\mu\in(-\infty,t)$, and denote $\mu^*$ the unique solution of $r(\mu)=0$. From any initial point $\mu_0\in(\mu^*,t)$, Newton-Raphson's iterates
$$
\mu_{n+1}=\mu_n-\frac{r(\mu_n)}{r'(\mu_n)}
$$
decrease towards $\mu^*$ at a quadratic speed.
\end{proposition}
\begin{proof}
We already know that $r$ is strictly increasing from $(-\infty,t)$ to $(0,\infty)$. Let us show that $r$ is also strictly convex.
According to the third item of Proposition~\ref{prop:approxdbeta} in Appendix~\ref{convconcacm}, $\widecheck{d}''(x|y)$ is completely monotonic, so it is strictly decreasing in $y$. Equivalently, $\widecheck{d}'(x|y)$ is strictly concave in $y$, and each $g'$ is also strictly concave according to~\eqref{eq:g'}. Since the inverse of a strictly increasing, strictly concave function $f$ is strictly increasing and strictly convex, which is a direct consequence of $(f^{-1})''=-\frac{f''\circ f^{-1}}{(f' \circ f^{-1})^3}$, 
then each $(g')^{-1}$ is strictly convex, and finally, $r$ is strictly convex.

For any $\mu_0\in(\mu^*,t)$, we have $r(\mu_0)>0$, so $\mu_1=\mu_0-\frac{r(\mu_0)}{r'(\mu_0)}<\mu_0$. We have also $\mu_1>\mu^*$ as a consequence of the strict convexity of $r$. By immediate recurrence, we obtain that $\mu_n$ is a decreasing series that converges towards $\mu^*$. According to \cite{Ortega70}, it converges at a quadratic speed since $|r'|$ and $|r''|$ are bounded away from 0 in $[\mu^*,\mu_0]$.
\end{proof}

At this point, we have derived an optimization framework to tackle problem~\eqref{eq:minG}. 
The optimal Lagrangian multiplier value is determined before each majorization-minimization update using a Newton-Raphson algorithm. However, such a formal solution is implementable if and only if each $y_\ell^\star(\mu)$ can be actually computed as the minimizer of $g^\mu\big(y_\ell|\widetilde{\hb}_{n(\ell)}\big)$ in $(0,\infty)$. In some cases, computing $y_\ell^\star(\mu)$ is equivalent to extracting the roots of a polynomial of a degree smaller or equal to four, which is possible in closed form. In other cases, we have to solve a polynomial equation of degree larger than four, or even an equation that is not polynomial. Table~\ref{tab:poldeg} indicates the cases where a closed-form solution is available. 
\begin{table}[h]
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\hfill$\beta\in$     &$(-\infty,1)\setminus\{0\}$&$\{0\}$&$\{1\}$&\multicolumn{4}{|c|}{$(1,2)$}      \\
Penalization&    &   &   &$\frac54$&$\frac43$&$\frac32$&other           \\\hline
No penalization& 1 & 1  & 1  & 1        &  1       &  1       &  1           \\\hline
Concave&1&1&1&3&4&2&$\rip$\\\hline
Lipschitz continuous gradient&$\rip$&3&2&$\rip$&$\rip$&3&$\rip$\\\hline
\end{tabular}
\caption{%\ji{Est-ce que nous devrions ajouter une ligne "no penalization", qui correspondrait aus cas traite en Sous-section~\ref{betanmf_disjointconstraint} ? Dans ce cas, sauf erreur, le degre est 1 dans chaque cas. } \ngc{Oui, tout à fait d'accord, et cela permet de motiver pq on considère ce cas dans la section 2.3!} 
The cases where \eqref{eq:yhat} can be computed in closed form are indicated by the degree of the corresponding polynomial equation, otherwise the symbol $\rip$ is used.}
%\ji{(I have maintained $\beta\geq2$ here, we will need to decide what to do with this case.)}
\label{tab:poldeg}
\end{table}





% This section is organized as follows:
% \begin{itemize}
%     \item Subsection~\ref{convconcacm} presents the convexity, concavity and complete monotonicity properties of a convex-concave decomposition of the discrete $\beta$-divergence that is crucial for the efficiency of the general framework and the derived algorithms,
%     \item Subsection~\ref{prob_algo_generalframe} firstly introduces the general form of a multivariate minimization problem involving a finite sum of discrete $\beta$-divergence terms under a linear constraint with a possible penalty term in the objective function. This penalty term can be either concave or Lipschitz smooth. % with constant $L$.
%     Secondly we present the general framework to tackle such optimization problems relying on the construction at the current iterate of an auxiliary function for the Lagrangian that is minimized in closed-form. Thirdly, we present the rate of convergence for the Newton-Raphson method used to compute the optimal Lagrangian multipliers at each iteration of the optimization framework.
%     \item Subsection~\ref{betanmf_disjointconstraint} presents the algorithm obtained from the general framework in the case of nonpenalized $\beta$-NMF under disjoint linear equality constraints.
% \end{itemize}

% \subsection{Convexity, concavity and complete monotonicity for a convex-concave decomposition of the discrete $\beta$-divergence}\label{convconcacm}
% The discrete $\beta$-divergence can always be expressed as the sum of convex, concave, and constant terms. In Table~\ref{tab:decompbetadiv} we introduce a convex-concave decomposition of the $\beta$-divergence which slightly differ from the one given in \cite[Table\,1]{Fevotte_betadiv} (by the fact that ours contains no constant term $\widebar{d}$) as follows:
% % \[
% % \widecheck{d}(x|y)=  \begin{cases}
% % \frac{1}{1-\beta} x \,y^{\beta -1}
% %       &\text{for}\quad \beta<1, \beta\neq0,  \\
% % \frac{x}{y}
% %       &\text{for}\quad \beta=0,   \\
% % %y-x-x\log \frac{y}{x}           
% % -x\log y           
% %       &\text{for}\quad \beta=1,  \\
% % \frac1{\beta}y^{\beta}-\frac1{\beta-1} xy^{\beta-1} &\text{for} \quad \beta \in \left(1,2\right), \\
% % \frac{1}{\beta} y^{\beta}
% %       &\text{for}\quad \beta\geq2,
% %   \end{cases}
% % \]
% % and
% % \[
% % \widehat{d}(x|y)= \begin{cases}
% %  \frac{1}{\beta}y^{\beta}-\frac{1}{\beta\,(1-\beta)} x^{\beta}
% %       &\text{for}\quad \beta<1, \beta\neq0,  \\
% % \log\frac{y}{x} - 1
% %       &\text{for}\quad \beta=0,   \\
% % %y-x-x\log \frac{y}{x}           
% % y + x\, \log x - x          
% %       &\text{for}\quad \beta=1,  \\
% % \frac{1}{\beta\,(\beta-1)} x^{\beta} &\text{for} \quad \beta \in \left(1,2\right), \\
% % -\frac{1}{\beta-1} x \,y^{\beta -1}+\frac{1}{\beta\,(\beta-1)} x^{\beta}
% %       &\text{for}\quad \beta\geq2,
% %   \end{cases}
% % \]
% % \ji{a remplacer peut-etre par une table a 5 lignes, 2 colonnes}



% \begin{table}[h]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \hfill$\beta$     &$(-\infty,1)\setminus\{0\}$&$0$&$1$&$(1,2)$ &   $[2,+\infty)$    \\
% Decomposition $d_{\beta}(x|y)$&  &   &  &    &   \\\hline
% $\widecheck{d}(x|y)$& $\frac{1}{1-\beta} x \,y^{\beta -1}$    & $\frac{x}{y}$  & $-x\log y$  &  $\frac1{\beta}y^{\beta}-\frac1{\beta-1} xy^{\beta-1}$  & $\frac{1}{\beta} y^{\beta}$  \\\hline
% $\widehat{d}(x|y)$&$ \frac{1}{\beta}y^{\beta}-\frac{1}{\beta\,(1-\beta)} x^{\beta}$&$\log\frac{y}{x} - 1$&$y + x\, \log x - x  $&$\frac{1}{\beta\,(\beta-1)} x^{\beta}$&$-\frac{1}{\beta-1} x \,y^{\beta -1}+\frac{1}{\beta\,(\beta-1)} x^{\beta}$\\\hline
% \end{tabular}
% }
% \caption{
% Proposed concave-convex decomposition of the discrete $\beta$-divergence.}
% %\ji{(I have maintained $\beta\geq2$ here, we will need to decide what to do with this case.)}
% \label{tab:decompbetadiv}
% \end{table}



% where $y\in(0,\infty)$, $\beta$ is real valued and $x\in(0,\infty)$, so that $d_{\beta}(x|y)=\widehat{d}(x|y)+\widecheck{d}(x|y)$. Further, $\beta$ and $x$ are considered as parameters, $d_{\beta}$, $\widehat{d}$ and $\widecheck{d}$ being handled as univariate functions of $y$.\\

% Let us now recall the definition of a complete monotonic function $f$:
% \begin{definition}
% A function $r$ is said to be completely monotonic (c.m.) on an interval $I$ if $r$ has derivatives of all orders on $I$ and $(-1)^n f^{(n)}(x)\geq0$ for $x\in I$ and $n\geq0$.
% \end{definition}
% We can now introduce the properties of concavity, convexity and monotonicity for  our convex-concave formulation of the discrete $\beta$-divergence:

% \begin{proposition} Given $\widecheck{d}(\cdot|\cdot)$ and $\widehat{d}(\cdot|\cdot)$ as defined above, we have that
% \label{prop:approxdbeta}
% \hfill
% \begin{enumerate}
% \item $\widecheck{d}(x|y)$ is $C^\infty$ and strictly convex on $(0,\infty)$ for $x>0$ and $\beta\in\mathbb{R}$;
% \item $\widehat{d}(x|y)$ is concave for $x>0$ and $\beta\in\mathbb{R}$;
% \item for all $\beta<2$, $\widecheck{d}''_{\beta}(x|y)$ and $\widehat{d}'_{\beta}(x|y)$ are c.m. 
% \end{enumerate}
% %Functions $g_1,\ldots,g_5$ are stricly convex on $(0,\infty)$. Moreover, $g_1$, $g_2$, $1-g'_3$, and $g''_4$ are completely monotonic on $(0,\infty)$.
% \end{proposition}
% \begin{proof}
% The proof is straightforward, given that $\widecheck{d}(x|y)$ and $\widehat{d}(x|y)$ linearly combine $C^\infty$ functions on $(0,\infty)$, and that in the same interval, 
% \begin{itemize}
% \item $\log y$ is strictly concave;
% \item $y^\nu$ is strictly convex for all  $\nu\in(-\infty,0)\cup(1,\infty)$, and strictly concave for all $\nu\in(0,1)$;
% \item $y^\nu$ is c.m. for all $\nu<0$.
% \end{itemize}
% \end{proof}
% According to the first two items of Proposition~\ref{prop:approxdbeta}, $\widecheck{d}$ and $\widehat{d}$ indeed yield a convex-concave decomposition of the $\beta$-divergence, which is a variant of \cite[Table\,1]{Fevotte_betadiv}. Let us remark that the successive minimization of an upper approximation of this convex-concave decomposition following the methodology presented in \cite{Fevotte_betadiv} yields to the usual multiplicative update scheme. 
% In the following subsection, we take advantage of these properties to build up a framework that enables to efficiently tackle penalized minimization problems relying on discrete $\beta$-divergence under linear constraints.








\subsection{MU for $\beta$-NMF with disjoint linear equality constraints, without penalty terms}\label{betanmf_disjointconstraint}


In this section, we derive an algorithm based on the general framework presented in the previous section to tackle the $\beta$-NMF problem under disjoint linear equality constraints in the non-penalized case, that is,  problem~\eqref{eq:betaNMFmodel} with $\lambda_1=\lambda_2=0$.
We consider this simplified case here as it allows to provide explicit MU for any value of $\beta < 2$; see the first row 'No penalization' of Table~\ref{tab:poldeg}. These updates  satisfy the constraints after each update of $W$ or $H$, and monotonically decrease the objective function $D_{\beta}\left(V|WH\right)$. 
% \subsubsection{Algorithm for disjoint-constrained $\beta$-NMF}\label{sec_algodisjointConstrainedbetaNMF} 

Let us then consider the subproblem of \eqref{eq:betaNMFmodel} over $H$ when $W$ is fixed and with $\lambda_2=0$, that is,  
%
\begin{equation}\label{eq:subprobleminW}
 \underset{H\in \mathbb{R}^{K \times N}_+}{\min}
 D_{\beta}\left(V|WH\right) 
\quad \text{such that} \quad \gammab_j^{T} H (\mathcal{B}_{j})=c_j \text{ for } 1\leq j \leq J.
\end{equation}
%\ngc{Ce n'est pas très naturel de faire tout en $W$ ici, alors qu'on a fait $H$ avant... ce n'est pas grave, mais juste un peu 'confusing'. Surtout que dans la section suivante, on est de retour sur $H$ avec le showcase 1... Cela vaudrait la peine de changer, mais ce n'est pas une priorité.}  
%In the following we derive MU for $H$ that decrease the objective in \eqref{eq:subprobleminW}. 
Let us follow the framework presented above. First, an auxiliary function, which we denote $G(H| \widetilde{H})$, is constructed at the current iterate $\widetilde{H}$ so that it majorizes the objective for all $H$ and is defined as follows:
%
\begin{equation}
\label{eq:G}
\begin{aligned}
G\left(H|\widetilde{H}\right)&=\sum_{f,n}\left[\sum_{k} \frac{W_{fk}\widetilde{H}_{kn}}{\widetilde{V}_{fn}}\widecheck{d}\left(V_{fn}|\widetilde{V}_{fn}\frac{H_{kn}}{\widetilde{H}_{kn}}\right)\right] \\
&+\left[\widehat{d}'\big(V_{fn}|\widetilde{V}_{fn}\big)\sum_{k}W_{fk}\big(H_{kn}-\widetilde{H}_{kn}\big)+\widehat{d}\big(V_{fn}|\widetilde{V}_{fn}\big) \right], 
\end{aligned}
\end{equation} 
%\ngc{Give a bit more details: convex-concave-constant decomposition, etc.}
where $\widecheck{d}(.|.)$ and $\widehat{d}(.|.)$ are the ones defined in Appendix~\ref{convconcacm}.
Second, we need to minimize $G\left(H|\widetilde{H}\right)$ 
%$D_{\beta}\left(V|WH\right)$ over $\mathbb{R}_{+}^{K \times N}$ with the auxiliary function of $G$, 
while imposing the set of linear constraints $\gammab_j^{T} H (\mathcal{B}_{j})=c_j$. The Lagrangian function of $G$ is given by 
\begin{equation}\label{eq:Gmu}
\begin{aligned}
G^{\mu}(H|\widetilde{H})= G(H |\widetilde{H} )-\sum_{j}^{J} \left[\mu_{j} \left( \gammab_j^{T} H (\mathcal{B}_{j})-c_j\right) \right], 
\end{aligned}
\end{equation} 
 where $\mu_{j}$ are the Lagrange multipliers associated to each linear constraint $\gammab_j^{T} H (\mathcal{B}_{j})=c_j$. We observe that $G^{\mu}$ in~\eqref{eq:Gmu} is a separable majorizer in the variables $H$ of the Lagrangian function $D_{\beta}\left(V|WH\right) - \sum_{j}^{J} \left[ \mu_{j} \left( \gammab_j^{T} H (\mathcal{B}_{j})-c_j\right) \right]$. Due to the disjoitness of each subset of variables $\mathcal{B}_{j}$ \eqref{eq:Gmu}, we only consider the optimization over one specific subset $\mathcal{B}_{j}$. 
The minimizer \eqref{eq:yhat} of $G^{\mu}(H\left( \mathcal{B}_{j} \right)|\widetilde{H}\left( \mathcal{B}_{j} \right))$ has the following component-wise expression:
\begin{equation}\label{eq:updateW}
\begin{aligned}
H^\star\left(\mathcal{B}_{j}\right)=\widetilde{H}\left(\mathcal{B}_{j}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{j}\right) \right]}{\left[ D\left(\mathcal{B}_{j}\right) - \mu_{j}  \gammab_j \right]} \right)^{.\left( \gamma \left( \beta \right)\right)} , 
\end{aligned}
\end{equation}  
where $C=W^{T} \left( \left( WH \right)^{.\left( \beta-2 \right) } \odot V \right)$, $D=W^{T}\left( WH\right)^{.\left( \beta-1 \right) }$, $\gamma(\beta)=\frac{1}{2-\beta}$ for $\beta < 1$, $\gamma(\beta)=1$ for $\beta \in \left[1,2\right]$ and $\gamma(\beta)=\frac{1}{\beta-1}$ for $\beta >2$ \cite[Table 2]{Fevotte_betadiv}, $A \odot B$ 
(resp.\@ $\frac{\left[ A \right]}{\left[ B \right]}$) is the Hadamard product (resp.\@ division) between $A$ and $B$,  
$A^{.(\alpha)}$ is the element-wise $\alpha$ exponent of $A$. 
%\ngc{Tu ne définirais pas dès le début $f_i = a_i^T W\left(\mathcal{K}_{i}\right) + b_i$, cela simplifierai tout ceci et serait plus concret.} 
Finally, we need now to find the optimal value for $\mu_j$, denoted $\mu_j^\star$,  wihch is the solution of $\gamma_j^{T} H^\star \left( \mathcal{B}_{j} \right)=c_j$. It requires to finding the root of the function 
\begin{equation} \label{eq:fmulincstr}
r_j(\mu_j)=\sum_{\ell=1}^{L} \gamma_{j,\ell} \left[ \widetilde{H}\left(\mathcal{B}_{j}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{j}\right) \right]}{\left[ D\left(\mathcal{B}_{j}\right) - \mu_{j}  \gamma_j \right]} \right)^{.\left( \gamma \left( \beta \right)\right)} \right]_{\ell}  -c_j , 
\end{equation}
where $\left[A\right]_{\ell}$ denotes the $\ell$-th entry of expression $A$. Proposition~\ref{prop:mu_unicity} shows that $\mu_j^\star$ is unique on some interval $\left(-\infty, t \right)$. 
Indeed, $r_j(\mu_j)$ is a finite sum of elementary rationale functions of $\mu_j$ and each of them is an increasing, convex function in $\mu_{j}$ over $\left(-\infty, t_{\ell},\right)$ with  $t_{\ell}=\frac{D_{\ell}\left(\mathcal{B}_{j}\right)}{\gamma_{j,\ell}}$ for all $\beta$. It is even completely monotone for all $\beta$ in $\left(-\infty, t_{\ell}\right)$ because $\gamma\left( \beta \right)>0$~\cite{miller2001}. As a consequence $r_j(\mu_j)$ is also a completely monotone, convex increasing function of $\mu_{j}$ in $\left(-\infty, t \right)$, where $t=\text{min}\left( t_{\ell} \right)$. Finally, we can easily show that the function $r_j(\mu_j)$ changes of sign on the interval $\left(-\infty, t \right)$ by computing two limits at the closure of the interval. As $\mu^\star \in (-\infty,t)$, the update \eqref{eq:updateW} is nonnegative.
%\ji{Je pense qu'on peut encore raccourcir ce paragraphe en faisant reference aux propositions de la sous-section 2.2.} 
To evaluate $\mu^\star$, we use a Newton-Raphson method, with any initial point $\mu_0\in(\mu^*,t)$, with a quadratic rate of convergence as demonstrated in Proposition~\ref{NR}. 
Algorithm~\ref{consDisBetaNMF} summarizes our method to tackle~\eqref{eq:betaNMFmodel} for all the $\beta$-divergences which we refer to as disjoint-constrained $\beta$-NMF algorithm. The update for matrix $W$ can be derived in the same way, by symmetry of the problem. 


%where $\mathcal{K}$ designates the full set of variables in $W$.
%\ngc{On pourrait parler du computational cost ici, et ne plus en parler après, ou dire que c'est similaire à ce cas c-à-d que le coût est dominé par les matrix-matrix products, et par par le caclul de $\mu^*$.} 

It can be verified that the computational complexity of Algorithm~\ref{consDisBetaNMF} is asymptotically equivalent to the standard MU for $\beta$-NMF, that is, it requires $\mathcal{O}\left(FNK \right)$ operations per iteration. Indeed, the complexity is mainly driven by matrix products and, based on numerical experiments, we confirm that the Newton-Raphson shows quadratic rates of convergence as shown by Proposition~\ref{NR}. Provided that a good initial approximation is known and by imposing to compute $J+I$ roots, the average theoretical complexity is the cost of calculating $r_i(x)/r_i'(x)$ and $r_j(x)/r_j'(x)$ and the number of iterations to converge. In practice, we report that the number of iterations required for the convergence of the Newton-Raphson method is in the order of magnitude of 10 to 100 and since $\max(J,I) \ll \max(F,K,N)$ in practice, the resulting complexity is dominated by the matrix products that require $\mathcal{O}\left(FNK \right)$ operations. 
The same conclusions apply to the algorithms presented in 
Sections~\ref{sec_ssbetaNMF}, \ref{sec_minvolKLNMF} and~\ref{sec_nonlinear}. 

\algsetup{indent=2em}
\begin{algorithm}[ht!]
\caption{$\beta$-NMF with disjoint linear constraints \label{consDisBetaNMF}}
\begin{algorithmic}[1] 
\REQUIRE A matrix $V \in \mathbb{R}^{F \times N}$, 
an initialization $H \in \mathbb{R}^{K \times N}_+$ and $W  \in \mathbb{R}^{F \times K}$, 
a factorization rank $K$, 
a maximum number of iterations, maxiter, 
a value for $\beta$, and 
the linear constraints defined by 
$\mathcal{K}_{i}$, $\alphab_j$ and $b_i$ for $i=1,2,\dots,I$, and 
$\mathcal{B}_{j}$, $\gammab_j$ and $c_j$ for $j=1,2,\dots,J$.  
\ENSURE A rank-$K$ NMF $(W,H)$ of $V$ satisfying constraints in \eqref{eq:betaNMFmodel}. 
    \medskip  
\FOR{$it$ = 1 : maxiter}
    \STATE \emph{\% Update of matrix $H$} 
    \STATE $C \leftarrow W^{T}\left( \left( WH \right)^{.\left( \beta-2 \right) } \odot V \right)$
    \STATE $D \leftarrow W^{T}\left( WH\right)^{.\left( \beta-1 \right) }$
    \FOR{$j = 1 : J$}
            \STATE $\mu_{j} \leftarrow \text{root}\left( r_j(\mu_j) \right)$ \quad \emph{\% see Equation~\eqref{eq:fmulincstr} }
            \STATE $H\left(\mathcal{B}_{j}\right) \leftarrow H\left(\mathcal{B}_{j}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{j}\right) \right]}{\left[ D\left(\mathcal{B}_{j}\right) -  \mu_{j}  \gamma_j \right]} \right)^{.\left( \gamma \left( \beta \right)\right)}$
    \ENDFOR
    \STATE $\mathcal{B}_{c} = \{ (k,n) \ | 1 \leq k  \leq K, 1 \leq n \leq N \} \backslash  \left(\cup_{j}^{J} \mathcal{B}_{j} \right).$ \quad \emph{\% $\mathcal{B}_{c}$ is the complement of $\cup_{j}^{J} \mathcal{B}_{j}$  }
    
    \STATE $H\left(\mathcal{B}_{c}\right) \leftarrow H\left(\mathcal{B}_{c}\right) \odot \left( \frac{\left[C\left(\mathcal{B}_{c}\right) \right]}{\left[ D\left(\mathcal{B}_{c}\right) \right]} \right)^{.\left( \gamma \left( \beta \right)\right)}$
	\STATE \emph{\% Update of matrix $W$}
    \STATE $W$ is updated in the same way as $H$, by symmetry of the problem. 
\ENDFOR
\end{algorithmic}  
\end{algorithm} 



==> arXiv v2/Chapters/3_showcase1_Beta-SSNMF.tex <==

In this section, we showcase a particularly important example of $\beta$-NMF with linear disjoint constraints \ji{and no penalization}, namely, the simplex-structured matrix factorization (SSMF) problem. It is defined as follows:  
given a data matrix  $V \in \mathbb{R}^{F \times N}$  and a factorization rank $K$, SSMF  refers  to  the  problem of computing $W$ and $H$ such that $V \approx WH$ and  the  columns  of $H$ lie on the unit simplex, that is, the entries of each column of $H$ are nonnegative and sum to one. SSMF is a powerful tool in many applications such as hyperspectral unmixing in geoscience and remote sensing \cite{6200362,6678258,abdolali2020simplex}, 
document analysis~\cite{chi2012tensors},  
and 
self-modeling curve resolution~\cite{neymeyr2018set}. 
We refer the reader to the recent survey \cite{fu2019nonnegative} for more applications and details about SSMF. 

To understand the underlying significance of SSMF, it is necessary to give more insights on a research topic for which important SSMF techniques were initially developed which is the blind Hyperspectral Unmixing (HU), a main research topic in  remote sensing. The task of blind HU is to decompose a remotely sensed hyperspectral image into endmember spectral signatures and the corresponding abundance maps with limited prior information, usually the only known information being the number of endmembers. In this context, the columns of~$W$ correspond to the endmembers spectral signatures and the columns of~$H$ contain the proportion of the endmembers in each column of~$V$, so the column-stochastic assumption for $H$ naturally holds. The nonnegativity of $W$ follows from the nonnegativity of the spectral signatures.  
We refer to the corresponding problem as simplex-structured nonnegative matrix factorization with the $\beta$-divergence ($\beta$-SSNMF), and is formulated as follows: 
%The most popular SSNMF models rely on the Frobenius norm for the data fitting term. In this paper we consider a more general identification criterion based on the $\beta$-divergences family. 
%\subsection{Problem formulation and algorithm}
%\ji{remplacer $H\left( :,j \right)$ par $\hb_j$ en conformite avec la section 2 ?}
% \begin{equation}\label{eq:betaSSNMF}
% \begin{aligned}
% & \underset{W\in \mathbb{R}^{F \times K}_+,H\in \mathbb{R}^{K \times N}_+}{\text{min}}
% & D_{\beta}(V|WH) 
% \; \text{ such that } \;  
% H\left( :,j \right) \in \Delta ^{K} \text{ for all } j, 
% \end{aligned}
% \end{equation} 
% \ji{(On pourrait ecrire directement $H\in\left(\Delta ^{K}\right)^J$ sous le min, et enlever "such that ..." ?)}
% where 
% $\Delta ^{K}=\left\lbrace x \in \mathbb{R}^{K}_{+} | \sum_{k=1}^K x_{k}=1 \right\rbrace$ is the unit simplex. Let us rewrite \eqref{eq:betaSSNMF} as follows: 
\begin{equation}\label{eq:betaSSNMFmodel}
\underset{W\in \mathbb{R}^{F \times K}_+,H\in \mathbb{R}^{K \times N}_+}{\min}
 D_{\beta}\left(V|WH\right) 
\quad \text{ such that } \quad  
 \eb^{T} \hb_j = 1 \text{ for } 1\leq j \leq N, 
\end{equation}
where $\eb$ is the vector of all ones of appropriate dimension. 
This is particular case of \eqref{eq:betaNMFmodel} where 
\begin{itemize}
    \item the subsets $\mathcal{B}_j$ correspond to the columns of $H$, and there is no subset $\mathcal{K}_i$ (no constraint on $W$),  
    \item $\gammab_j^{T} = \eb$ and $c_j = 1$ for $j=1,2,\dots,N$. 
    %a H \left( \mathcal{B}_{j} \right)=c_j$ are given by $\eb^{T} hb_j = 1$  for $1\leq j \leq N$.
\end{itemize}
Hence Algorithm~\ref{consDisBetaNMF} can be directly applied to~\eqref{eq:betaSSNMFmodel}. 

%Based on Algorithm~\ref{consDisBetaNMF}, we easily derive Algorithm~\ref{consDisBetaNMF} to tackle problem \eqref{eq:betaSSNMFmodel}. 
%Note that variable $\mub$ at line 13 is the vector of Lagrangian multipliers of size $N$. 
%and $e_{K,1}$ is the $K$-by-$1$ all-one matrix. 
%In order to save space and since that Algorithm~\ref{consDisBetaNMF} is close to Algorithm~\ref{consDisBetaNMF}, Algorithm~\ref{consDisBetaNMF} is available in the Appendix \ref{appen_algo3}.

%\ngc{Comme indiqué dans mon email: ceci est une appliation directle de la Section 2.3: je ne mettrais pas de détails ici, juste les MU finales dans Algorithm 2, le reste éventuellement en Appendix.}

%As mentioned in section \ref{sec:lagrange}, each constraint $\gamma_j^{T} H \left( \mathcal{B}_{j} \right)=c_j$ is satisfied for a unique value of $\mu_{j}$ in $\left(-\infty,t \right)$. We can therefore use a Newton-Raphson method to find the $\mu_{j}$, see section \ref{sec:lagrange}. 
% On a practical point of view, the root $\mu_{j}$ will be searched over the interval $\left(\alpha b,+\infty \right)$ by starting in $\alpha b$ where $\alpha$ is a tuning parameter such that $\alpha \in \left[0,1 \right[$. The reason to use this parameter is twofold; on one hand, functions $f_{j}$ are not defined in $b$ and on the other hand, the root of $f_{j}$ can be arbitrarily close to $b$ from the right depending on the input matrix $V$ and the value chosen for $\beta$. By taking into account the monotone decreasing behaviour of the functions $f_{j}$, parameter $\alpha$ enables to tune the starting point for the Newton-Raphson method so that it remains on the left side of the root. 


%\ngc{Je pense que si on fait tout en $H$ dans la section précédente, on peut enlever cet algorithme; 
%à la limite le mettre en appendix car c'est la même chose que Algorithm 2.} 
%It can be verified that the computational complexity of the simplex-structured $\beta$-NMF algorithm is asymptotically equivalent to the standard MU for $\beta$-NMF, that is, it requires $\mathcal{O}\left(FNK \right)$ operations per iteration. Indeed, the complexity is mainly driven by matrix products and, based on numerical experiments, we confirm that the Newton-Raphson shows quadratic rates of convergence as shown by Proposition~\ref{NR}. Provided that a good initial approximation is known and by imposing to compute $N$ roots with $n$-digit precision, the average theoretical complexity is $\mathcal{O}\left(\text{log}\left( n \right) g(n) N \right)$ where $g(n)$ is the cost of calculating $f(x)/f^{'}(x)$ with $n$-digit precision. Provided that $g(n)$ tends to grow superlinearly, which is the case in practice, the cost of finding $N$ roots is therefore $\mathcal{O}\left(g(n) N \right)$.
%This complexity is dominated by $\mathcal{O}\left(FNK \right)$ since $g(n) \ll FK$ in practice. \ngc{Il a disparu où le $\log(n)$?} \ngc{Pourrais-tu expliquer pourquoi $g(n) \ll FK$ en pratique? Donner un exemple / valeur typique de $g$?} 
%\ngc{Tu aimes les $F$ ;-) On s'y perd vraiment ici.} 
%\subsection{Numerical experiments}\label{secnumexpssNMF}

\paragraph{Numerical experiments}  Let us perform numerical experiments to evaluate the effectiveness of Algorithm~\ref{consDisBetaNMF}  on the simplex-structure $\beta$-NMF problem against existing methods. To the best of our knowledge, the so-called group robust NMF (GR-NMF)  algorithm\footnote{\href{https://www.irit.fr/~Cedric.Fevotte/extras/tip2015/code.zip}{https://www.irit.fr/$\sim$Cedric.Fevotte/extras/tip2015/code.zip}} from \cite{7194802} is the most recent algorithm that is able to tackle problem \eqref{eq:betaSSNMFmodel} for the full range of $\beta$-divergences. 
%by integrating the $\ell_1$-normalization for each update of matrix $H$. 
The approach is not based on Lagrangian multipliers but introduces a change of variables for matrix $H$. This approach, initially used for NMF in \cite{1381036}, does not provide an auxiliary function for the subproblem in $H$ and resort to a heuristic commonly used in NMF, see for example  \cite{4100700,fevotte2009nonnegative}. 
Therefore there is no guarantee that the objective function is decreasing at each update of the abundance matrix, unlike Algorithm~\ref{consDisBetaNMF}.

%\footnotemark[\ref{fn1}]
%\footnotemark[\ref{fn1}]
We apply Algorithm~\ref{consDisBetaNMF} and GR-NMF on three widely used real hyperspectral data sets\footnote{\href{http://lesun.weebly.com/hyperspectral-data-set.html}{http://lesun.weebly.com/hyperspectral-data-set.html}}~\cite{zhu2017hyperspectral}:  
\begin{itemize}
    
    \item Samson:   156 spectral bands with 95$\times$95 pixels, containing mostly 3 materials $(K=3)$, 
    namely ``Soil", ``Tree" and ``Water". 

\item Jasper Ridge: 198 spectral bands with 100$\times$100 pixels, containing mostly 4 materials $(K=4)$, 
    namely ``Road", ``Soil", ``Water" and ``Tree". 
    

    \item Cuprite: 188 spectral bands with 250$\times$190 pixels, containing mostly 12 types of minerals $(K=12)$.

\end{itemize}

% \begin{itemize}
%     \item Samson: the original data set includes 952$\times$952 pixels and 156 spectral reflectance bands in the wavelength range 401\,nm to 889\,nm, resulting in a spectral resolution of 3.13\,nm. As the very large size of the original image has a strong impact on the computational cost, a region of  has been extracted starting at coordinates (252,332) in the original image.  In this paper we assume that the data set contains 3 endmembers: "Soil", "Tree" and "Water" respectively and then set the factorization rank $K$ to 3.
%     \item Jasper Ridge: the original data set consists of 512 $\times$ 614 pixels and 224 spectral reflectance bands in the wavelength range 380 nm to 2500 nm, resulting in a spectral resolution of 9.46 nm. As the original image is too large, we consider a subimage of 100$\times$100  pixels. starting  at coordinates (105,269) in the original image. After removing channels 1--3, 108--112, 154--166 and 220--224 (due to dense water vapor and atmospheric effects), the number of remaining channels was 198. We assume that the data set contains 4 endmembers: "Road", "Soil", "Water" and "Tree" and then set the factorization rank $K$ to 4.
%     %\item HYDICE Urban: this data set\footnote{\url{http://lesun.weebly.com/hyperspectral-data-set.html} } has been acquired with HS Digital Imagery Collection Experiment (HYDICE) HS sensor \cite{Basedow1995} over an urban area at Copperas Cove, TX, U.S. in October 1995. The Urban data set consists of 307$\times$307 pixels and 210 spectral reflectance bands in the wavelength range 400 nm to 2500 nm, resulting in a spectral resolution of 10 nm. After the channels 1--4, 76, 87, 101--111, 136--153 and 198--210 are removed (due to dense water vapor and atmospheric effects), we remain 162  channels. There are three versions of ground truth, which contain 4, 5 and 6 endmembers respectively. In this paper, we assume that the data set contains 6 endmembers and then set the factorization rank $K$ to 6.
%     \item Cuprite: this data set has been acquired over Cuprite in Las Vegas, NV, U.S. The Cuprite data set consists of 250$\times$190 pixels and 224 spectral reflectance bands in the wavelength range 370\,nm to 2480\,nm, resulting in a spectral resolution of 10\,nm. Channels 1--2, 221--224 (noisy channels), 104--113 and 148--167 (water absorption channels) were removed, and the number of remaining channels was 188. The data set contains 14 types of minerals. Since there are minor differences between variants of similar minerals, we reduce the number of endmembers to 12 then set the factorization rank $K$ to 12 as well.
% \end{itemize}

$\beta$-SSNMF has shown itself as a powerful one to tackle blind HU, hence this comparative study between Algorithm~\ref{consDisBetaNMF} and GR-NMF~\cite{7194802} focuses on the convergence aspects including the  evolution of the objective function and the runtime. The algorithms are compared\revise{\footnote{\revise{
For $\beta = 3/2$, we had an error in our derivations, and use~\eqref{eq:updateW} with $\eta(\beta) = 1$ for $\beta \in (0,1)$; see the discussion after~\eqref{eq:updateW}. 
However, the corresponding MU always decreases the objective function values (which we were monitoring), although we do not have a theoretical justification for this. A possible approach to obtain such as result would be to come up with a majorizer of the majorizer that has a closed-form minimizer given by~\eqref{eq:updateW} with $\eta(\beta) = 1$ for $\beta \in (0,1)$. 
}
}} 
for $\beta \in  \left\{0,\frac12,1,\frac32,2\right\}$. 
To report the results, we use the relative objective function, denoted $\Bar{F}(W,H)$ and defined as\footnote{For the Frobenius norm, that is, $\beta = 2$, the relative error is typically defined as $\frac{D_\beta(V|WH)}{D_\beta(V|0)}$ meaning that the trivial solution used is the all-zero matrix. However, for other $\beta$-divergences, the value of $D_\beta(V|0)$ might not be defined; in particular, for $\beta \leq 1$ and $v_{fn} > 0$ for some $f,n$. } 
\begin{equation*}
    \Bar{F}(W,H) = \frac{D_\beta(V|WH)}{D_\beta(V|v \eb\eb^T)} , 
\end{equation*} 
where $v = \frac{\eb^T V \eb}{FN}$ is the average of the entries of $V$. 
The relative error  $\Bar{F}$ should be between 0 and 1: it is equal to 0 for an exact decomposition with $V = WH$, and is equal to 1 for a trivial rank-one approximation where all entries are equal to the average of the entries of $V$. 
This allows to meaningfully interpret the results, especially since we consider in this comparative study multiple values for $\beta$. In fact, the degree of homogeneity of the $\beta$-divergence is a  function of $\beta$.
For example, if all the entries of the input matrix are multiplied by 10 and keeping the same  NMF solution properly scaled,   the squared Frobenius error ($\beta$ = 2) is multiplied by 100 while the IS-divergence ($\beta$ = 0) is not affected. 
\color{black}


As for all tests performed in this paper, the algorithms are tested on a desktop computer with Intel Core i7-8700@3.2GHz CPU and 32GB memory. The codes are written in MATLAB R2018a, and available from \href{https://sites.google.com/site/nicolasgillis/}{https://sites.google.com/site/nicolasgillis/}.  
For all simulations, the algorithms are run for 20 random initializations of $W$ and $H$ (each entry sampled from the uniform distribution in $[0,1]$). 
Table~\ref{table:ssbetaNMFperf} reports the average and standard deviation of the runtime (in seconds) as the final value for the {relative} objective function over these 20 runs for a maximum of 300 iterations. 
%\begin{center}
\begin{table}[ht!]
\centering
%\begin{center}
\caption{Runtime performance in seconds and final value of {relative} objective function ${\Bar{F}}_\text{end}(W,H)$ for Algorithm~\ref{consDisBetaNMF} and the GR-NMFreported for $\beta \in  \left\{0,\frac12,1,\frac32,2\right\}$. The table reports the average and standard deviation over 20 random initializations with a maximum of 300 iterations for three hyperspectral data sets. A bold entry indicates the best value for each experiment. %\ngc{Cb itérations? Mettre en gras le meilleur.}
}
\label{table:ssbetaNMFperf}
\setlength{\tabcolsep}{2pt}
%\footnotesize
%\small
\resizebox{\columnwidth}{!}
{
\begin{tabular}{|c|c|c|c|c|c|c|}
  \hline
  Algorithms       & \multicolumn{2}{|c|}{Samson} & \multicolumn{2}{|c|}{Jasper Ridge} & \multicolumn{2}{|c|}{Cuprite}\\
                   & runtime (s.) & ${\Bar{F}}_\text{end}(W,H)$ & runtime (s.) & ${\Bar{F}}_\text{end}(W,H)$ & runtime (s.) & ${\Bar{F}}_\text{end}(W,H)$ \\
  \hline
                   &\multicolumn{6}{|c|}{$\beta=2$}\\
  \hline 
   Algorithm~\ref{consDisBetaNMF}   &\textbf{16.62$\pm$0.15}  &{\textbf{(1.89$\pm$0.04)}$10^{-3}$}  &\textbf{22.86$\pm$0.08}  &{\textbf{(4.68 $\pm$ 0.39)$10^{-3}$}} &121.04 $\pm$ 0.62 &{ \textbf{(0.98 $\pm$ 0.06)$10^{-3}$}} \\
 
  
  GR-NMF &18.23$\pm$0.29  &{(1.91$\pm$0.05)$10^{-3}$}  &25.32$\pm$0.16  &{(5.87 $\pm$ 1.22)$10^{-3}$} &\textbf{114.27 $\pm$ 0.20} &{ (1.29 $\pm$ 0.07)$10^{-3}$}\\

  \hline
                  &\multicolumn{6}{|c|}{$\beta=3/2$}\\
  \hline 
   Algorithm~\ref{consDisBetaNMF}   &\textbf{63.69$\pm$0.40}  &{\textbf{(2.52 $\pm$0.78)$10^{-3}$}}  & \textbf{89.23 $\pm$0.30} &{ \textbf{(4.92 $\pm$ 0.29)$10^{-3}$}} &\textbf{421.49 $\pm$ 2.79} &{\textbf{(1.54 $\pm$ 0.07)$10^{-3}$}}\\
 
 
  GR-NMF &80.09$\pm$0.60    &{(2.60 $\pm$0.63)$10^{-3}$}    &112.72 $\pm$0.67  &{(6.32 $\pm$ 1.37)$10^{-3}$}  &508.57 $\pm$ 3.50 &{(2.01 $\pm$ 0.09)$10^{-3}$}\\

  \hline
                  &\multicolumn{6}{|c|}{$\beta=1$}\\
  \hline 
   Algorithm~\ref{consDisBetaNMF}   &\textbf{18.33 $\pm$ 0.08} &{\textbf{(3.54 $\pm$ 0.27)}$10^{-3}$ } &\textbf{24.82 $\pm$ 0.35}  &{ \textbf{(6.07 $\pm$ 0.21)$10^{-3}$}} &\textbf{182.98 $\pm$ 14.14} &{\textbf{(2.07 $\pm$ 0.09)$10^{-3}$}}\\
 
  
  
  GR-NMF &44.78 $\pm$ 0.18 &{(3.77 $\pm$ 0.38 ) $10^{-3}$} &62.83 $\pm$ 0.76  &{ (7.26 $\pm$ 1.50)$10^{-3}$ }&370.25 $\pm$ 21.33 &{(2.67 $\pm$ 0.10)$10^{-3}$}\\

  \hline
  
                  &\multicolumn{6}{|c|}{$\beta=1/2$}\\
  \hline 
   Algorithm~\ref{consDisBetaNMF}   &\textbf{89.80 $\pm$ 0.65}  &{(7.21 $\pm$ 0.75)$10^{-3}$}  &\textbf{126.43 $\pm$ 0.61}  &{ \textbf{(1.08 $\pm$ 0.10)$10^{-2}$}}&682.80 $\pm$ 3.32 &{\textbf{(3.13 $\pm$ 0.15)$10^{-3}$}}\\
 
  
  GR-NMF &102.21 $\pm$ 0.72  &{\textbf{(6.93 $\pm$ 0.88)$10^{-3}$}}  &141.75 $\pm$ 0.69  &{ (1.12 $\pm$ 0.13)$10^{-2}$} &\textbf{642.49 $\pm$ 1.22} &{(3.14 $\pm$ 0.14)$10^{-3}$}\\
  \hline
                  &\multicolumn{6}{|c|}{$\beta=0$}\\
  \hline 
   Algorithm~\ref{consDisBetaNMF}   &\textbf{52.89$\pm$0.54}  &{(4.60 $\pm$ 0.66)$10^{-2}$}  &\textbf{69.59$\pm$0.44}  &{\textbf{(3.76 $\pm$ 0.11)$10^{-2}$}} &479.84 $\pm$ 16.02 &{(4.39 $\pm$ 0.31)$10^{-3}$}\\
 
  
  GR-NMF &55.61$\pm$0.47  &{\textbf{(4.22 $\pm$ 0.79)$10^{-2}$  }}&77.87$\pm$0.63  &{(3.76 $\pm$ 0.44)$10^{-2}$} &\textbf{354.65 $\pm$6.01} &{\textbf{(3.35 $\pm$ 0.10)$10^{-3}$}}\\

  \hline
\end{tabular} 
}
%\end{center}
\end{table}
%\end{center}


We observe that  Algorithm~\ref{consDisBetaNMF} outperforms the GR-NMF in terms of runtime and final values for the {relative} objective function for all test cases except when $\beta=0$ for the Samson and Cuprite data sets. In particular, for $\beta=1$,  Algorithm~\ref{consDisBetaNMF} is up to 2.5 times faster than the GR-NMF.
For the Cuprite data set with $\beta=1/2$, Algorithm~\ref{consDisBetaNMF} and GR-NMF perform similarly. We also observe that the standard deviations obtained with Algorithm~\ref{consDisBetaNMF} are in general significantly smaller for all $\beta$, except for $\beta=0$ for the Samson and Cuprite data sets. 

In the supplementary {material} S1, we provide figures that show the  evolution of the {relative} objective function values with respect to iterations, and that confirm the observations above. 
%Figures \ref{fig:ssbetaNMF_lossfun_compa_part1} and \ref{fig:ssbetaNMF_lossfun_compa_part2}  display the average  objective function values along the 300 iterations for the three data sets and the five values considered for $\beta$. 
%Additionally, based on Figures \ref{fig:ssbetaNMF_lossfun_compa_part1} and \ref{fig:ssbetaNMF_lossfun_compa_part2}, we observe that in the cases $\beta\geq1$, Algorithm~\ref{consDisBetaNMF} converges faster than the GR-NMF. 

==> arXiv v2/Chapters/4_showcase2_quadSepReg.tex <==

%\ngc{Restructurer cette partie (Pour le moment, on s'y perd): 
%(1) donner le modèle, 
%(2) parler brièvement de l'identifiabilité et de son importance, 
%(3) parler de l'application en audio, mais aussi applicable à l'hyperspecral et autres. 
%(4) Dire que cela ne rentre pas dans le framework précédant car il y a une méchante régularisation, mais qu'on va quand même montrer comment dériver des updates --> et expliquer que cela pourrait s'appliquer à d'autres modèles régularisés. 
% } 



In this section, we showcase another important example of $\beta$-NMF with linear disjoint constraints, namely, the minimum volume NMF with the $\beta$-divergences (min-vol $\beta$-NMF) model. This model is based on the minimization of $\beta$-divergences including a
penalty term promoting solutions with minimum volume spanned by the columns of the matrix $W$. It is defined as follows:
%
\begin{equation}\label{eq:4}
 \underset{W\in \mathbb{R}^{F \times K}_+,H\in \mathbb{R}^{K \times N}_+}{\min}  
 D_{\beta}(V|WH) + \lambda \text{vol}(W) \quad \text{ such that } \quad 
 W^T e = e. 
\end{equation} 
where
$\lambda$ is a penalty parameter,
and 
$\text{vol}(W)$ is a function measuring the volume spanned by the columns of $W$.  In \cite{9084229}, the authors use 
$\text{vol}(W)=\logdet(W^{T}W+\delta I)$, 
 where $\delta$ is a small positive constant that prevents $\logdet(W^{T}W)$ to go to $-\infty$ when $W$ tends to a rank-deficient matrix (that is, when $\text{rank}(W)< K$). 
This model is particularly powerful as it leads to identifiability which is crucial in many applications such as in hyperspectral imaging or audio source separation~\cite{fu2019nonnegative}. 
Indeed, under some mild assumptions and in the exact case, authors prove in \cite{9084229} that \eqref{eq:4} is able to identify the groundtruth factors $(W^\#,H^\#)$ that generated the input data $V$, in the absence of noise. 
%Moreover, it is able to recover the factors even when the factorization rank is overestimated. In fact, this model automatically sets extra factors to zero in this situation, hence performs model order selection automatically. 
In \cite{9084229}, \eqref{eq:4} is used for blind audio source separation. In a nutshell, blind audio source separation consists in isolating and extracting unknown sources based on an observation of their mix recorded with a single microphone\footnote{We invite the interested reader to watch the video \href{https://www.youtube.com/watch?v=1BrpxvpghKQ}{https://www.youtube.com/watch?v=1BrpxvpghKQ} to see the application of min-vol KL-NMF on the decomposition of a famous song from the city of Mons.}. 
We have to mention that model \eqref{eq:4} is also well suited for hyperspectral imaging as discussed in \cite{gillis2020bk}. 



In the next subsections, we show that we can tackle the min-vol $\beta$-NMF optimization problem defined in \eqref{eq:4} with the general framework presented in Section~\ref{sec_generalframework} in the case $\beta = 1$.  

%The logdet function  in \eqref{eq:4} is majorized by its first-order Taylor approximation at the current iterate, which itself is majorized by  %\footnote{This is a two-step majorizization approach applied on a composition of function: the first-order Taylor approximation is a majorizer for any concave function, which is then majorized.}, 
% a quadratic form in $W$ with a $L$-Lipschitz continuous gradient. We then derive multiplicative updates for $W$ that satisfy the full set of constraints (nonnegativity and  sum-to-one constraint). 

\subsection{Problem formulation and algorithm}

As the minimum-volume penalty of model \eqref{eq:4} concerns matrix $W$ only, the main challenge concerns the update of $W$. Indeed, the update of $H$ is simply the one from~\cite{algoNMFlee}. Let us therefore consider the subproblem in $W$ for $H$ fixed: 
\begin{equation}\label{eq:betaminvolNMFinW} 
\underset{W\in \mathbb{R}^{F \times K}_+}{\min}
D_{\beta}\left(V|WH\right)+ \lambda \logdet(W^{T}W+\delta I) 
\quad 
\text{such that} \quad  \eb^{T} \wb_i = 1 \text{ for } 1\leq i \leq K. 
\end{equation}
 Compared to the general model \eqref{eq:betaNMFmodel}, we have that 
\begin{itemize}
    \item the subsets $\mathcal{K}_{i}$ correspond to the columns of $W$, and there is no subset $\mathcal{B}_j$, 
    \item $\alphab_i^{T} = \eb$ and $b_i = 1$ for $1\leq i \leq K$. 
   % W \left( \mathcal{K}_{i} \right)=$ are given by $\eb^{T}W(:,i)=1$ 
\end{itemize}
To upper bound $\logdet(W^{T}W+\delta I)$ as required by~\eqref{eq:Lipschtiz_case} in Assumption~\ref{ass:phi}, 
we majorize it using a convex quadratic separable auxiliary function  provided in \cite[Eq.~(3.6)]{9084229} and which is derived as follows. First, the concave function $\logdet(Q)$ for $Q \succ 0$ can be upper bounded using the first-order Taylor approximation: for any $\widetilde{Q} \succ 0$, 
\[
\logdet( Q ) 
\; \leq \;  \logdet( \widetilde{Q} ) + \langle 
\widetilde{Q}^{-1} , Q - \widetilde{Q} \rangle 
\; =  \;
\langle \widetilde{Q}^{-1} , Q \rangle + \text{cst}, 
\]
where cst is some constant independent of $Q$.  
For any $W, \widetilde{W}$, and denoting  
$\widetilde{Q} = \widetilde{W}^T \widetilde{W} + \delta I \succ 0$, we obtain  
\[
\logdet( W^T W + \delta I ) 
\,  \leq \, 
\left\langle \widetilde{Q}^{-1} ,  
W^T W  \right\rangle + \text{cst} 
\, = \, \tr ( W \widetilde{Q}^{-1} W^T ) + \text{cst} , 
%\, =  \,   \sum_{f=1}^F W(:,f)^T ( \widetilde{W}^T \widetilde{W} + \delta I )^{-1} W(:,f) + \text{cst}, 
%= 
%\tr ( W \widetilde{W}^T \widetilde{W} + \delta I )^{-1} W^T ) +
\]
which is a convex quadratic and Lipschitz-smooth function in $W$. 
In fact, letting $\widetilde{Q}^{-1} = DD^T$ be a decomposition (such as Cholesky) of  $\widetilde{Q}^{-1} \succ 0$, we have 
$\tr ( W \widetilde{Q}^{-1} W ) = \| WD \|_F^2$, 
from which~\eqref{eq:Lipschtiz_case} can be derived easily; see  \cite{9084229} for the details. 
With this and following our framework from Section~\ref{sec_generalframework}, we obtain the Lagrangian function 
% defined at current iterate $\widetilde{W}$ as follows: 
% \begin{equation*}\label{eq:betaminvolNMFauxiliaryfun}
% \begin{aligned}
% & \bar{F}\big(W|\widetilde{W}\big) 
% = \sum_{f} G\left( \wb_f |\widetilde{\wb}_f \right) + \lambda \left( \sum_{f} \bar{l}\left( \wb_f |\widetilde{\wb}_f\right) + c\right), 
% \end{aligned}
% \end{equation*}
\begin{equation}\label{eq:Gmuminvol} 
G^{\mu}\big(W|\widetilde{W}\big) = \sum_{f} G\left( \wb_f |\widetilde{\wb}_f \right) + \lambda \left( \sum_{f} \bar{l}\left( \wb_f |\widetilde{\wb}_f\right) + c\right) 
 +\mub^{T} \sum_{f}\left(\wb_{f} - \frac1F \eb \right), 
\end{equation} 
where \ji{$\wb_f\in$ denotes the $f$-th row of $W$}, 
$G$ is given by \eqref{eq:G}, $\bar{l}$ by~\cite[Eq.~(3.6)]{9084229} and derived as explained above, and $c$ is a constant. Let $\mub$ is the vector Lagrange multipliers of dimension $K$ %\ngc{Ne pas redéfinir les notations 2 fois. Cela vaudrait peut-être la peine d'avoir une seciton 'Notation' à la fin de l'intro?}
associated to each linear constraint $\eb^{T} \wb_i = 1$. 
Exactly as before (hence we omit the details here), $G^{\mu}$ is separable and,  given $\mub$, one can compute the closed-form solution: 
% let us consider one specific row $\wb \in \mathbb{R}^{K \times 1}$ of $W$ and rewrite \eqref{eq:Gmuminvol} for $\wb$ as follows:
% \begin{equation}\label{eq:Gmuminvolw}
% \begin{aligned}
% G^{\mu}(\wb|\widetilde{\wb})&= G\left(\wb |\widetilde{\wb} \right) + \lambda \bar{l}\left(\wb |\widetilde{\wb}\right) + c + \mub^{T} \left(\wb - \frac1F \eb \right) .
% \end{aligned}
% \end{equation} 
% For $\beta=1$, the derivative of $G^{\mu}(\wb|\widetilde{\wb})$ \eqref{eq:Gmuminvolw} w.r.t.\  a specific entry $\wb_{k}$ is given by:
% \begin{equation*}\label{eq:gradGmu}
% \begin{aligned}
% \nabla_{\wb_{k}} G^{\mu}(\wb|\widetilde{\wb})&=\sum_{n}h_{kn}-\sum_{n}h_{kn}\frac{\widetilde{\wb}_{k} v_{n}}{\wb_{k}\widetilde{v}_{n}}+2\lambda \left[ Y \widetilde{\wb} \right]_{k} + 2 \lambda \left[ \diag \left( \frac{Y^{+}\widetilde{\wb}+Y^{-}\widetilde{\wb}}{\widetilde{\wb}} \right) \right]_{k} \wb_{k}\\
% & \qquad- 2 \lambda \left[ \diag \left( \frac{Y^{+}\widetilde{\wb}+Y^{-}\widetilde{\wb}}{\widetilde{\wb}} \right) \right]_{k} \widetilde{\wb}_{k} + \mu_{k}. 
% \end{aligned}
% \end{equation*} 
% Due to the separability, canceling the derivative provides the following closed-form solution:
% \begin{equation}\label{eq:updatewk}
% \begin{aligned}
% & \wb^\star_{k}=\widetilde{\wb}_{k} \frac{\sqrt{\left(\sum_{n}h_{kn} - 4\lambda \left[ Y^{-} \widetilde{\wb} \right]_{k} + \mu_{k} \right)^{2}+8 \lambda \left[ \diag \left( Y^{+}\widetilde{\wb}+Y^{-}\widetilde{\wb} \right) \right]_{k} \sum_{n}h_{kn}\frac{v_{n}}{\widetilde{v}_{n}}}-\sum_{n}h_{kn} + 4\lambda \left[ Y^{-} \widetilde{\wb} \right]_{k} - \mu_{k}}{4\lambda \left[ \diag \left( Y^{+}\widetilde{\wb}+Y^{-}\widetilde{\wb} \right) \right]_{k}}
% \end{aligned}
% \end{equation} 
% which is non-negative. 
%For clarity purpose, let us introduce
% so that \eqref{eq:updatewk} can be written in the following matrix form 
\begin{equation}\label{eq:updateWminvolNMF}
\begin{aligned}
& W^\star(\mu) = \widetilde{W} \odot  
\frac{\left[\left[ \left[ C + \eb \mub^{T} \right]^{.2}+S \right]^{.\frac{1}{2}} - \left(C + \eb  \mub^{T}\right)\right]}{\left[ D  \right] }, 
\end{aligned}
\end{equation} 
where 
$C=e_{F,N}  H^{T} - 4\lambda \big( \widetilde{W} Y^{-}\big)$, $D =4\lambda \widetilde{W} \left( Y^{+}+Y^{-}\right)$, 
and 
$S=8 \lambda \widetilde{W} \left( Y^{+}+Y^{-}\right)\odot \left( \frac{\left[ V \right]}{\left[\widetilde{W}H\right]} H^{T} \right)$ 
with 
$Y=Y^{+}-Y^{-}=\big(\widetilde{W}^{T}\widetilde{W}+\delta I\big)^{-1}$, 
$Y^{+} = \text{max}(Y,0) \geq 0$ 
and 
$Y^{-} = \text{max}(-Y,0) \geq 0$, and 
$e_{F,N}$ is the $F$-by-$N$ matrix of all ones. 
As proved in Proposition~\ref{prop:mu_unicity}, the constraint  
$W^\star(\mu)^T \eb = \eb$ is satisfied for a unique $\mub$ in $\left(-\infty,t \right)$ where $t=\infty$ in this case. We can therefore use a Newton-Raphson method to find the $\mu_{i}$ with quadratic rate of convergence, see Proposition~\ref{NR}.
Algorithm~\ref{dcminvolKLNMF} summarizes our method to tackle~\eqref{eq:4}. 
\algsetup{indent=2em}
\begin{algorithm}[ht!]
\caption{Min-vol KL-NMF \label{dcminvolKLNMF}}
\begin{algorithmic}[1] 
\REQUIRE A matrix $V \in \mathbb{R}^{F \times N}$, an initialization $H \in \mathbb{R}^{K \times N}_+$, an initialization $W  \in \mathbb{R}^{F \times K}$ , a factorization rank $K$, and a maximum number of iterations, maxiter, the parameters $\delta > 0$ and $\lambda > 0$. 
\ENSURE A min-vol rank-$K$ NMF $(W,H)$ of $V$ satisfying constraints in \eqref{eq:4}. 
    \medskip  
\FOR{$it$ = 1 : maxiter}
    \STATE \emph{\% Update of matrix $H$}
	\STATE  $H \leftarrow H \odot \frac{\left[  W^{T} \left( \frac{\left[ V\right]}{\left[ WH\right]} \right) \right]}{\left[  W^{T} e_{F,N} \right]}$ \quad 
	\STATE \emph{\% Update of matrix $W$}
	\STATE $Y \leftarrow \left(W^{T}W+\delta I \right)^{-1}$
	\STATE $Y^{+} \leftarrow \text{max}\left(Y,0\right)$
	\STATE $Y^{-} \leftarrow \text{max}\left(-Y,0\right)$
    \STATE $C \leftarrow e_{F,N}  H^{T} - 4\lambda \left( W Y^{-}\right)$
    \STATE $S \leftarrow 8 \lambda W \left( Y^{+}+Y^{-}\right)\odot \left( \frac{\left[ V \right]}{\left[WH\right]} H^{T} \right)$
    \STATE $D  \leftarrow 4\lambda W \left( Y^{+}+Y^{-}\right)$
    %\FOR{$i$ = 1 : $K$}
            \STATE $\mub \leftarrow 
            \text{root}\left( W^\star(\mu)^T \eb = \eb  \right)$ over $\mathbb{R}^K$  \quad \emph{\% see \eqref{eq:updateWminvolNMF} for the expression of $W^\star(\mu)$}   
    %\ENDFOR
    \STATE $W \leftarrow W \odot  \frac{\left[\left[ \left[ C + e  \mub^{T} \right]^{.2}+S \right]^{.\frac{1}{2}} - \left(C + \eb  \mub^{T}\right)\right]}{\left[ D  \right] }$
\ENDFOR
\end{algorithmic}  
\end{algorithm} 

%It can be verified that the computational cost of the disjoint-constraint min-vol KL-NMF is asymptotically equivalent to the standard MU for $\beta$-NMF, that is, it requires $\mathcal{O}\left(FNK \right)$ operations per iteration. Indeed, the cost of finding $K$ roots with $n$-digit precision with a Newton-Raphson method is $\mathcal{O}\left(g(n) K \right)$. \ngc{Même comment qu'avant: et le log(n)?} 
%This complexity is dominated by $\mathcal{O}\left(FNK \right)$ since $g(n) \ll FN$ in practice.

\subsection{Numerical experiments}

In this section we compare baseline KL-NMF (that is, the standard MU), the min-vol KL-NMF from \cite[Algorithm 1]{9084229} that 
solves~\eqref{eq:4} using MU combined with line search (min-vol KL-NMF LS), 
and Algorithm~\ref{dcminvolKLNMF} applied to the spectrogram of two monophonic piano sequences considered in \cite{9084229}. The first audio sample is the first measure of ``Mary had a little lamb", a popular English song. The second audio sample corresponds to the first 30 seconds of ``Prelude and Fugue No.1 in C major" from de Jean-Sebastien Bach played by Glenn Gould\footnote{\href{https://www.youtube.com/watch?v=ZlbK5r5mBH4}{https://www.youtube.com/watch?v=ZlbK5r5mBH4}}. 
%We observed that the results obtained for $W$ and $H$ with Algorithm~\ref{dcminvolKLNMF} and min-vol KL-NMF were very similar, therefore the comparative study focuses on the runtime. 
We use the following three setups: 
\begin{itemize}
    \item Setup $\sharp$1: sample ``Mary  had  a  little  lamb" with \mbox{$K=3$}, 200 iterations. 
    \item Setup $\sharp$2: sample ``Mary  had  a  little  lamb" with \mbox{$K=7$}, 200 iterations. 
    \item Setup $\sharp$3: ``Prelude and Fugue No.1 in C major" with $K=16$, 300 iterations.
\end{itemize}
For each setup, the algorithms are run for the same 20 random initializations of $W$ and $H$. 
Table~\ref{table:runtimeperf} reports the average and standard deviation of the runtime (in seconds) over these 20 runs. Table~\ref{table:lossfunperf} reports the average and standard deviation of the final values for $\beta$-divergences (data fitting term) and the objective function of \eqref{eq:4} over these 20 runs for min-vol KL-NMF LS and Algorithm~\ref{dcminvolKLNMF}. For this last comparison, the value for the penalty weight $\lambda$ has been chosen so that KL-NMF leads to reasonable solutions for $W$ and $H$. More precisely, the values for $\lambda$ are chosen so that the initial value of  $\frac{\lambda \left| \logdet( {W^{(0)}}^T W^{(0)} + \delta I)\right|}{D_{\beta}\left(V|WH \right)}$  is  equal to 0.1, 0.1 and 0.022 for setup $\sharp$1, setup $\sharp$2 and setup $\sharp$, respectively. 
\begin{center}
\begin{table}[ht!]
\begin{center}
\caption{ Runtime  performance in seconds of baseline KL-NMF, min-vol KL-NMF LS and Algorithm~\ref{dcminvolKLNMF}. The table reports the average and standard deviation over 20 random initializations. 
%\ngc{Il faudrait aussi une table qui compare les function values, comme pour SSNMF. Evidemment, ile ne faut dans ce cas que comparer ce qui est comparable càd les objectifs de nos also avec le même paramètre de pénalité. A ce propos, il faudrait expliquer comment tu le choisis. } 
} 
\label{table:runtimeperf}
\begin{tabular}{|c|c|c|c|}
  \hline
  Algorithms       & \multicolumn{3}{|c|}{runtime in seconds} \\
                   & setup $\sharp$1 & setup $\sharp$2 & setup $\sharp$3  \\
  \hline
  baseline KL-NMF   & 0.53$\pm$0.03 & 0.45$\pm$0.02 & 4.32$\pm$0.30  \\
 
  \hline
  min-vol KL-NMF LS \cite{9084229} & 3.79$\pm$0.13 & 2.39$\pm$0.30 & 10.19$\pm$1.28     
      \\  \hline
  Algorithm~\ref{dcminvolKLNMF}    & 0.58$\pm$0.03 & 0.66$\pm$0.03 & 4.80$\pm$ 0.38                  \\  \hline
\end{tabular} 
\end{center}
\end{table}
\end{center}

% \begin{center}
% \begin{table}[ht!]

% \begin{center}
% \caption{
% Final values for $D_{\beta}$ and $F$ from \eqref{eq:4} obtained with min-vol KL-NMF (Algorithm 1 from \cite{9084229}) and Algorithm~\ref{dcminvolKLNMF}. The table reports the average and standard deviation over 20 random initializations for three experimental setups described in the text. 
% \ngc{table trop petite... je la mettrais dans l'autre sense (setups sur lignes, algo sur colonnes)} 
% } 
% \label{table:lossfunperf}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|}
%   \hline
%   Algorithms       & \multicolumn{2}{|c|}{ setup $\sharp$1} & \multicolumn{2}{|c|}{ setup $\sharp$2} & \multicolumn{2}{|c|}{ setup $\sharp$3}\\
%                   & $D_{\beta,\text{end}}$ & $\Psi_\text{end}$ & $D_{\beta,\text{end}}$ & $\Psi_\text{end}$ & $D_{\beta,\text{end}}$ & $\Psi_\text{end}$  \\
%   \hline
%   min-vol KL-NMF \cite{9084229} & (3.52 $\pm$ 0.03)$10^{3}$ & (4.17 $\pm$ 0.03)$10^{3}$ & (3.54 $\pm$ 0.03)$10^{3}$ & (4.42 $\pm$ 0.04)$10^{3}$ & (7.77 $\pm$ 0.23)$10^{3}$ & (9.14 $\pm$ 0.20)$10^{3}$     
%       \\  \hline
%   Algorithm~\ref{dcminvolKLNMF}    & \textbf{(2.31 $\pm$ 0.01)$10^{3}$} & \textbf{(3.08 $\pm$ 0.01)$10^{3}$} & \textbf{(1.77 $\pm$ 0.02)$10^{3}$} & \textbf{(2.87 $\pm$ 0.02)$10^{3}$} & \textbf{(4.67 $\pm$ 0.08)$10^{3}$} & \textbf{(6.50 $\pm$ 0.06)$10^{3}$}     
%       \\  \hline
% \end{tabular} 
% }
% \end{center}
% \end{table}
% \end{center}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{center}
\begin{table}[ht!]

\begin{center}
\caption{
Final values for $D_{\beta}$ and the penalized objective $\Psi$ from \eqref{eq:4} obtained with min-vol KL-NMF LS and Algorithm~\ref{dcminvolKLNMF}. The table reports the average and standard deviation over 20 random initializations for three experimental setups. A bold entry indicates the best value for each experiment. 
} 
\label{table:lossfunperf}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\hfill }   & min-vol KL-NMF LS \cite{9084229}& Algorithm~\ref{dcminvolKLNMF}  \\   \hline 
 \multirow{2}{4em}{setup $\sharp$1} & $D_{\beta,\text{end}}$ & (3.52 $\pm$ 0.03)$10^{3}$ & \textbf{(2.31 $\pm$ 0.01)$10^{3}$} \\
                 & $\Psi_\text{end}$              & (4.17 $\pm$ 0.03)$10^{3}$ & \textbf{(3.08 $\pm$ 0.01)$10^{3}$} \\ \hline
 \multirow{2}{4em}{setup $\sharp$2} & $D_{\beta,\text{end}}$ & (3.54 $\pm$ 0.03)$10^{3}$ & \textbf{(1.77 $\pm$ 0.02)$10^{3}$} \\
                 & $\Psi_\text{end}$              & (4.42 $\pm$ 0.04)$10^{3}$ & \textbf{(2.87 $\pm$ 0.02)$10^{3}$} \\ \hline
 \multirow{2}{4em}{setup $\sharp$3} & $D_{\beta,\text{end}}$ & (7.77 $\pm$ 0.23)$10^{3}$ & \textbf{(4.67 $\pm$ 0.08)$10^{3}$} \\
                 & $\Psi_\text{end}$              & (9.14 $\pm$ 0.20)$10^{3}$ & \textbf{(6.50 $\pm$ 0.06)$10^{3}$} \\ \hline


\end{tabular}
%}
\end{center}
\end{table}
\end{center}

We observe that the runtime of Algorithm~\ref{dcminvolKLNMF} is close to the baseline KL-NMF algorithm which confirms the negligible cost of the Newton-Raphson steps to compute $\mub^\star$ as discussed in Section~\ref{betanmf_disjointconstraint}.
On the other hand, since no line search is needed, we have a drastic acceleration from 2x to 7x compared to the backtracking line-search procedure integrated in min-vol KL-NMF LS \cite{9084229}. 
Moreover, we observe in Table~\ref{table:lossfunperf} that Algorithm~\ref{dcminvolKLNMF} outperforms min-vol KL-NMF LS in terms of final values for the data fitting term and objective function values, with lower standard deviations. 

==> arXiv v2/Chapters/5_Quadratic_constraints.tex <==
%\ngc{Essayer d'être un peu plus générale et mieux motiver: 
Our general framework presented in Section~\ref{sec_generalframework} applies to $\beta$-NMF under disjoint linear equality constraints with penalty terms satisfying Assumption~\ref{ass:phi}; 
see problem~\eqref{eq:betaNMFmodel}. 
We have showcased our approach on $\beta$-SSNMF in Section~\ref{sec_ssbetaNMF} and on min-vol KL-NMF under sum-to-one constraints on the columns of $W$ in Section~\ref{sec_minvolKLNMF}. 
In this section, we show that the same framework can be extended to other simple constraints, namely disjoint quadratic constraints. 
% \ngc{Il faudrait aussi mieux motiver ce modèle peut-être en terme de conservation d'énergie? Y'a-t-il quelque chose de ce type dans la litérature? }
% \ngc{Il faudrait aussi pouvoir dire au lecteur quelles sont les conditions pour que le framework de la Section 2 est généralisable; 
% pas juste donner deux exemples intéressants... } 

% \ngc{Un bon flow serait: 
% (1) On présente un genral framework for $\beta$-NMF for disjoint linear constraints, 
% (2) On showcase sur SSNMF. 
% (3) On se pose la question: est-ce que cela peut être généralisé? Deux cas: 
% (3a) Si on modifie l'objectif. Je pense que si l'objectif reste simple, cela s'applique directelement, par exemple la sparse NMF avec penalité $\ell_1$. Il faudrait le mentionner. Si l'objectif est plus compliqué, comme min-vol, alors c'est plus au cas par cas --> on peut faire min-vol KL-NMF mais pas les autres $\beta$ facilment. 
% (3b) Si on passe à des contraintes non-linéaires: elle ne doivent pas être tro méchante: showcase example - quadratic. 
% (3c) Si on a des contraintes non-disjointe: cela est envisagleable mais on devra résoudre des equations poly. à plus de 1 varibles --> further research.} 
We consider sparse $\beta$-NMF for $\beta=1$ where 
the rows of $H$ are penalized with the $\ell_1$ norm and 
each column of $W$ have a fixed $\ell_2$ norm. 
We show that MU satisfying the set of constraints can be derived which we apply on blind HU. 

%\subsection{Algorithm}
%for $\beta=1,2$
%\subsection{Showcase example: hyperspheric-structured sparse $\beta$-NMF}
\subsection{Problem formulation and algorithm}

In this section we consider the following model involving quadratic disjoints constraints, that we refer to as hyperspheric-structured sparse $\beta$-NMF:
\begin{equation}\label{eq:betahsminvolNMFmodel}
 \underset{W\in \mathbb{R}^{F \times K}_+,H\in \mathbb{R}^{K \times N}_+}{\min} 
 D_{\beta}(V|WH) + \sum_{k=1}^{K}\lambda_{k} \left\| H(k,:) \right\|_{1} \\
\quad \text{such that} \quad  
 \eb^{T} \wb_j^{.(2)} = \rho \text{ for } 1\leq i \leq K, 
\end{equation}
where %$\left\| . \right\|_{1}$ stands for the $\ell_{1}$-norm that induces sparsity, 
$\lambda_{k}$ is a penalty weight to control the sparsity of the $k$-th row of $H$, and the quadratic constraints require the columns of $W$ to lie on the surface of a hyper-sphere centered at the origin with radius $\sqrt{\rho} > 0$. 
Without this normalization, the $\ell_{1}$-norm regularization would make $H$ tends to zero and $W$ grows to infinity. 

As done before, we update $W$ and $H$ alternatively. We tackle the subproblem in $H$ with $W$ fixed based on the MU developed in \cite{fevotte2009nonnegative} and guaranteed to decrease the objective function: 
\begin{equation}\label{eq:updateHhssparseNMF}
\begin{aligned}
& H = \widetilde{H} \odot \frac{\left[  W^{T}\left(  V \odot \big[ W\widetilde{H}\big]^{.(\beta-2)} \right) \right]}{\left[  W^{T} \big[ W\widetilde{H}\big]^{.(\beta-1)} + \lambdab e^T \right]} , 
\end{aligned}
\end{equation} 
where $\lambdab\in\mathbb{R}_+^K$ is the vector of penalty weights.
It remains to compute an update for $W$. To do so, we use the convex separable auxiliary function $G$ from \cite{Fevotte_betadiv} constructed at the current iterate $\widetilde{W}$, from which we obtain, as before, the Lagrangian function 
\begin{equation}\label{eq:Gmuhsminvol}
\begin{aligned}
G^{\mu}\big(W|\widetilde{W}\big)&= \sum_{f} G\left( w_f |\widetilde{w}_f \right) + \sum_{k}\lambda_{k} \left\| H(k,:) \right\|_{1}+ {\mub}^{T} \sum_{f}\left(w_{f}^{.(2)} - \frac1F\rho \eb \right), 
\end{aligned}
\end{equation} 
where $\mub\in\mathbb{R}^K$ is the vector of Lagrange multipliers associated to the constraint $\eb^{T} \Wb^{.(2)} = \rho \eb^{T}$. 
% As $G^{\mu}$ is separable, let us consider one specific row $\wb \in \mathbb{R}^{K \times 1}$ of $W$ and rewrite \eqref{eq:Gmuhsminvol} for $w$ as follows:
% \begin{equation}\label{eq:Gmuhsminvolh}
% \begin{aligned}
% G^{\mu}(\wb|\widetilde{\wb})&= G\left( \wb |\widetilde{\wb} \right) + \sum_{k}\lambda_{k} \left\| H(k,:) \right\|_{1}+ {\mub}^{T} \left(\wb^{.(2)} - \frac1F\rho e \right). 
% \end{aligned}
% \end{equation} 
% For $\beta=1$, the derivative of $G^{\mu}(\wb|\widetilde{\wb})$ \eqref{eq:Gmuhsminvolh} w.r.t. a specific entry $w_{k}$ is given by:
% \begin{equation*}\label{eq:gradGmuhs}
% \begin{aligned}
% \nabla_{w_{k}} G^{\mu}(\wb|\widetilde{\wb})&=\sum_{n}h_{kn}-\sum_{n}h_{kn}\frac{\widetilde{w}_{k} v_{n}}{w_{k}\widetilde{v}_{n}} + 2 \mu_{k} w_{k}. 
% \end{aligned}
% \end{equation*} 
% Due to the separability, canceling the derivative provides the following closed-form solution:
% \begin{equation}\label{eq:updatehk}
% \begin{aligned}
% & w^\star_{k}(\mu) = \frac{\sqrt{\left(\sum_{n}h_{kn}\right)^{2}+8 \mu_{k} \sum_{n}h_{kn}\frac{\widetilde{w}_{k}v_{n}}{\widetilde{v}_{n}}}-\sum_{n}h_{kn} }{4\mu_{k}}
% \end{aligned}
% \end{equation} 
% which is non-negative as soon as $\mu_{k} > 0$.
Exactly as before (hence we omit the details here),  given $\mub$, 
one can obtain a closed-form solution: 
%Let, so (\ref{eq:updatehk}) can be written in the following matrix form 
\begin{equation}\label{eq:updateHhsminvolNMF}
\begin{aligned}
& W^\star(\mub) = \frac{\left[\left[ \left[ C \right]^{.2}+8 \left( 
\eb \mub^{T}\right) \odot S \right]^{.\frac{1}{2}} - C\right]}{\left[ 4  \eb \mub^{T} \right] } , 
\end{aligned}
\end{equation}   
where  $C=e_{F,N}  H^{T}$ and $S=\widetilde{W}\odot \left(  \frac{\left[ V \right]}{\left[ \widetilde{W} {H}\right]} H^{T} \right)$. 
Let us now write the expression of the quadratic constraint $\sum_{f}(W^{\star}(\mub)_{f,i})^{2}-\rho=0$ for one specific column of $W$, say the $i$-th: 
\begin{equation} \label{eq:rootsparseNMF}
r_{i}\left( \mu_i \right) := \sum_{f}(W^{\star}_{f,i}(\mu_i))^{2}-\rho 
= \sum_{f} \left(\frac{\sqrt{ \left( C_{f,i}  \right)^{2}+8 \mu_{i} S_{f,i} } - C_{f,i} }{ 4 \mu_{i} }\right)^{2} -\rho =0. 
\end{equation} 
Computing the Lagrangian multiplier $\mu_{i}$ to satisfy the constraint requires computing the roots of the functions $r_{i}\left( \mu_i \right)$. We can show that each $W^{\star}_{f,i}(\mu_i)$ \eqref{eq:updateHhsminvolNMF} is a monotone decreasing, nonnegative convex function over $(0,+\infty)$. Therefore $\sum_{f}(W^{\star}_{f,i}(\mu_i))^{2}$ is also monotone decreasing and convex in $\mu_{i}$ over $(0,+\infty)$. Indeed, let $g$ : $\mathbb{R}_{+} \rightarrow \mathbb{R}_{+}$ be a monotone decreasing, nonnegative convex function. If $g$ is twice-differentiable, then $\left( g^{2}\right)'' = 2\left( g'\right)^{2}+2gg'' \geq 0$ since $g,g''\geq 0$ and $\left( g^{2} \right)'=2g'g \leq 0$ since  $g\geq 0$, $g'\leq 0$ by hypothesis. Now we can conclude that $r_{i}\left( \mu_i \right)$ is a monotone decreasing convex function over $(0,+\infty)$. Moreover, using Hospital's rule, we have: 
\begin{equation*}
\underset{\mu_{i}\rightarrow 0^{+}}{\text{lim}} \sum_{f}(W^{\star}_{f,i}(\mu_i))^{2}-\rho= +\infty 
\quad  \text { and } \quad 
\underset{\mu_{i}\rightarrow +\infty}{\text{lim}} \sum_{f}(W^{\star}_{f,i}(\mu_i))^{2}-\rho = -\rho <0,
\end{equation*} 
since $\rho > 0$. Therefore, the root of $r_{i}\left( \mu_i \right)$ is unique over  $(0,+\infty)$. We use a Newton-Raphson method to solve the problem.
Algorithm~\ref{dchsminvolKLNMF} summarizes our method. 
%For clarity purpose, we pose $f_{i}\left( \mu_i \right)=\sum_{f}(W^{\star}_{f,i}(\mu_i))^{2}-\rho$.
 

\algsetup{indent=2em}
\begin{algorithm}[ht!]
\caption{Hyperspheric-structured sparse KL-NMF \label{dchsminvolKLNMF}}
\begin{algorithmic}[1] 
\REQUIRE A matrix $V \in \mathbb{R}^{F \times N}$, an initialization $H \in \mathbb{R}^{K \times N}_+$, an initialization $W  \in \mathbb{R}^{F \times K}$ , a factorization rank $K$, 
a maximum number of iterations, maxiter, a weight vector $\lambda >0$.
\ENSURE A sparse rank-$K$ NMF $(W,H)$ of $V$ satisfying constraints in \eqref{eq:betahsminvolNMFmodel}. 
    \medskip  
\FOR{$it$ = 1 : maxiter}
	\STATE \emph{\% Update of matrix $H$}
    \STATE $H \leftarrow H \odot \frac{\left[  W^{T}\left(  V \odot \big[ WH\big]^{.(\beta-2)} \right) \right]}{\left[  W^{T} \big[ WH\big]^{.(\beta-1)} + \lambdab e^T \right]}$
    \STATE \emph{\% Update of matrix $W$}
    \STATE $C \leftarrow  e_{F,N} H^T$
    \STATE $S \leftarrow W \odot \left( \frac{\left[ V \right]}{\left[WH\right]} H^T \right)$
    \FOR{$j$ = 1 : K}
            \STATE $\mu_{i} \leftarrow \text{root}\left( r_{i}\left( \mu_i \right) \right)$ over $(0,+\infty)$ \emph{\% See Equation~\eqref{eq:rootsparseNMF}}
    \ENDFOR
	\STATE  $W \leftarrow \frac{\left[\left[ \left[ C \right]^{.2}+8 \left(  \eb \mub^T \right) \odot S \right]^{.\frac{1}{2}} - C\right]}{\left[ 4 \mub \eb^{T} \right] }$  
% 	\STATE \emph{\% Update the weight vector $\lambda$}
% 	\FOR{$k$ = 1 : K}
%             \IF {$it \in \left[it_{\min}, it_{\max}\right] \text{ and } \text{sp}\left( H(k,:) \right) \leq sp$}
%                 \STATE $\lambda(k) \leftarrow \lambda(k) \times \alpha$
%             \ENDIF
%     \ENDFOR
\ENDFOR
\end{algorithmic}  
\end{algorithm} 

%It can be verified that the computational complexity of the hyperspheric-structured min-vol KL-NMF algorithm is asymptotically equivalent to the standard MU for $\beta$-NMF, that is, it requires $\mathcal{O}\left(FNK \right)$ operations per iteration. Indeed, the cost of finding $K$ roots with $n$-digit precision with a Newton-Raphson method is $\mathcal{O}\left(g(n) K \right)$.
%This complexity is dominated by $\mathcal{O}\left(FNK \right)$ since $g(n) \ll FN$ in practice.

\subsection{Numerical experiments}





% In this section we report the results obtained with Algorithm~\ref{dchsminvolKLNMF} applied to the spectrogram of two monophonic piano sequences. The first audio sample, referred as data set 1, is the first measure of ``Mary had a little lamb" that is composed of three notes; $E_{4}$, $D_{4}$ and $C_{4}$. The second audio sample, initially proposed in \cite{fevotte2009nonnegative}, is a piano sequence played from the score given in Figure \ref{fig:audio2_representations}. The piano sequence is composed of four notes; $D_{4}$, $F_{4}$, $A_{4}$ and $C_{5}$, played all at once in the first measure and then played by pairs in all possible combinations in the remaining measures. Note that both sequences are made of pure piano notes, the factorization rank $K$ should therefore correspond to the number of notes present into the signals. The numerical experiments are conducted with a focus on the case where the factorization rank $K$ is overestimated compared to the number of sources. For data set 1, Algorithm~\ref{dchsminvolKLNMF} was run for 1000 iterations which allowed it to converge with $\delta=0.1$, $\rho=1/10$ and $\lambda=5$.
% For the second data set, Algorithm~\ref{dchsminvolKLNMF} was run for 500 iterations with $\delta=1$, $\rho=1/10$ and $\lambda=107$. For all simulations, random initializations are used for $W$ and $H$, the best results among 5 runs are kept.

% \begin{figure}[h!]
% \centering 
%         \includegraphics[width=0.50\textwidth]{Images/Section5/audiosample2.png}
% \caption{
% Musical score of the second audio sample (referred as data set 2).
% }
% \label{fig:audio2_representations}
% \end{figure} 


% Figure~\ref{fig:compa_datasets_hsminvolKLNMF} presents from top to bottom the columns of $W$, the rows of $H$, the evolution of the objective function of \eqref{eq:betahsminvolNMFmodel} and the evolution of $\left\| \mu^{T} \sum_{n}\left(h_{n}^{.(2)} - \rho e_{K}/N \right)\right\|$ for hyperspheric-structured min-vol KL-NMF with $K=7$ for data set 1 (left) and data set 2 (right).

% \begin{figure}
%     \centering  %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%       %(or a blank line to force the subfigure onto a new line)
%     \begin{subfigure}[b]{0.4\textwidth}
%         \includegraphics[width=\textwidth]{Images/Section5/basis_dataset1_K7-eps-converted-to.pdf}
%         \includegraphics[width=\textwidth]{Images/Section5/activations_dataset1_K7-eps-converted-to.pdf}
%         \includegraphics[width=\textwidth]{Images/Section5/lossfun_dataset1-eps-converted-to.pdf}
%         \caption{Data set 1}
%     \end{subfigure}
%     ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%     %(or a blank line to force the subfigure onto a new line)
%     \begin{subfigure}[b]{0.4\textwidth}
%         \includegraphics[width=\textwidth]{Images/Section5/basis_dataset2_K7-eps-converted-to.pdf}
%         \includegraphics[width=\textwidth]{Images/Section5/activations_dataset2_K7-eps-converted-to.pdf}
%         \includegraphics[width=\textwidth]{Images/Section5/lossfun_dataset2-eps-converted-to.pdf}
%         \caption{Data set 2}
%     \end{subfigure}
%     \caption{Results obtained with Algorithm~\ref{dchsminvolKLNMF} for data sets 1 (left) and 2 (right) with the parameters detailed in the text. From top to bottom: columns of W, rows of H, objective function along iterations (logarithmic scale for y axis) and evolution of $\left\| \mu^{T} \sum_{n}\left(h_{n}^{.(2)} - \rho e_{K}/N \right)\right\|$  .}\label{fig:compa_datasets_hsminvolKLNMF}
% \end{figure} 

% For data set 1, we observe that min-vol KL-NMF is able to extract the three pitches correctly. We obtain four extra components that correspond to hammer hits and pedal releases, for which the associated rows of $H$ are strictly equivalent and the associated columns of $W$ present small values that seem to be constant along the frequency range. For data set 2, min-vol KL-NMF extracts the four pitches correctly. We obtain one component that corresponds to the residual noise and two components for the transient events (the hammer hits and pedal releases) for which the associated rows of $H$ are strictly equivalent and the associated column of $W$ present small values along the frequency range. Therefore, even if the factorization rank is overestimated, min-vol KL-NMF preserves and correctly extracts the sources.

% We finally report that for both data sets;
% \begin{itemize}
%     \item the objective function is not-increasing along iterations, 
%     \item the constraints on the rows of $H$ to lie on the hyper-sphere of radius $\sqrt{\rho}$ are satisfied at each iteration, 
%     \item Algorithm~\ref{dchsminvolKLNMF} shows computational performances as anticipated; the runtimes are close to the baseline KL-NMF (that is, the standard MU).
% \end{itemize}

In this section, we perform numerical experiments to evaluate the effectiveness of Algorithm~\ref{dchsminvolKLNMF} on the HU problem. 
To the best of our knowledge, sparse $\beta$-NMF\footnote{\href{http://www.jonathanleroux.org/software/sparseNMF.zip}{http://www.jonathanleroux.org/software/sparseNMF.zip}}  from \cite{Leroux} is the most recent algorithm that is able to tackle problem \eqref{eq:betahsminvolNMFmodel} for the KL-divergence by integrating the $\ell_2$-normalization for each update of matrix $W$. 
This approach is similar to that of~\cite{7194802} for $\beta$-SSNMF, that is, it uses  parametrization, and resort to a heuristic with no guarantee on the decrease of the objective function. 
We refer to this algorithm as $\beta$-SNMF. 
%The approach is not based on Lagrangian multipliers but introduces a change of variables for matrix $W$. More precisely, this approach consists in directly reformulating the objective function including a column-wise normalized version of $W$ and the derivation of the updates of $W$ relies on computing the gradient of the objective function and splitting it into the difference of two non-negative terms. This approach does not provide an auxiliary function for the subproblem in $W$ and resort to a heuristic commonly used in NMF, see, \emph{e.g.}, \cite{4100700,fevotte2009nonnegative}, to cite a few. Therefore there is no guarantee that the objective function is decreasing at each update of the abundance matrix, unlike Algorithm~\ref{dchsminvolKLNMF}.

We apply Algorithm~\ref{dchsminvolKLNMF} and $\beta$-SNMF~\cite{Leroux} to the three real hyperspectral datasets detailed in Section~\ref{sec_ssbetaNMF}. This comparative study focuses on the convergence aspects including the evolution of the objective function and the runtime; we refer the interested reader to the Supplementary Material S2 for qualitative result on the ability of sparse $\beta$-NMF to decompose such images. %All the algorithms are implemented and tested on a desktop computer with Intel Core i7-8700@3.2GHz CPU and 32GB memory. The codes are written in MATLAB R2018a. 
For all simulations, the algorithms are ran for 20 random initializations of $W$ and $H$, the entries of the penalty weight $\lambdab$ has been set to 0.1, 0.05 and 0.05 for Samson, Jasper Ridge and Cuprite data sets, respectively. In order to fairly compare both algorithms, $\rho$ has been set to 1 as $\beta$-SNMF considers a $\ell_2$-normalization for the columns of $W$, and the entries of the weight vector $\lambdab$ in Algorithm~\ref{dchsminvolKLNMF} have the same values as $\beta$-SNMF requires to use the same values for all rows of $H$. Table~\ref{table:hsbetaNMFperf} reports the average and standard deviation of the runtime (in seconds) as the final value for the objective function over these 20 runs for a maximum of 300 iterations. 
Figure~\ref{fig:hsbetaNMF_lossfun_compa} displays the objective function values. 
%\begin{center}
\begin{table}[ht!]
%\footnotesize
\centering
%\begin{center}
\caption{Runtime performance in seconds and final value of objective function $\Phi_\text{end}(W,H)$ for Algorithm~\ref{dchsminvolKLNMF} and $\beta$-SNMF. The table reports the average and standard deviation over 20 random initializations with a maximum of 300 iterations for three hyperspectral data sets. A bold entry indicates the best value for each experiment.  %\ngc{idem Table 4} %\ngc{Cb itérations? Mettre en gras le meilleur.}
} 
\label{table:hsbetaNMFperf}
\setlength{\tabcolsep}{2pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
  \hline
  Algorithms       & \multicolumn{2}{|c|}{Samson data set} & \multicolumn{2}{|c|}{Jasper Ridge data set} & \multicolumn{2}{|c|}{Cuprite data set}\\
                   & runtime (sec) & $\Phi_\text{end}(W,H)$ & runtime (sec) & $\Phi_\text{end}(W,H)$ & runtime (sec) & $\Phi_\text{end}(W,H)$ \\
  \hline 
   Algorithm~\ref{dchsminvolKLNMF}   &11.07$\pm$0.19  &(2.68$\pm$0.00)$10^{3}$  &15.67$\pm$0.17  &\textbf{(4.65 $\pm$ 0.00)$10^{3}$} &70.16 $\pm$ 0.85 & \textbf{(2.12 $\pm$ 0.00)$10^{3}$} \\ 
  $\beta$-SNMF~\cite{Leroux}  &\textbf{7.63$\pm$0.13}  &(2.68$\pm$0.00)$10^{3}$ &\textbf{10.98$\pm$0.18}  &(4.71 $\pm$ 0.00)$10^{3}$ &\textbf{51.86 $\pm$ 0.74} & (2.18 $\pm$ 0.00)$10^{3}$\\
  \hline
\end{tabular} 
}
%\end{center}
\end{table}
%\end{center} 
\begin{figure}[ht!]  %add desired spacing between images, e. g.~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
      \begin{tabular}{ccc} 
    %\begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=0.3\textwidth]{Images/Section5/lossfun_sec5_Samson_averagev2-eps-converted-to.pdf}
      %  \caption{Samson Data set}
    %\end{subfigure} 
    & 
 %add desired spacing between images, e. g.~, \quad, \qquad, \hfill etc.
    %(or a blank line to force the subfigure onto a new line)
    %\begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=0.3\textwidth]{Images/Section5/lossfun_sec5_Jasper_averagev2-eps-converted-to.pdf}
       % \caption{Jasper Ridge Data set}
    %\end{subfigure} 
    & 
    %\begin{subfigure}[b]{0.333\textwidth}
        \includegraphics[width=0.312\textwidth]{Images/Section5/lossfun_sec5_Cuprite_averagev2-eps-converted-to.pdf}
      % \caption{Cuprite Data set}
    %\end{subfigure} 
    \\ 
     %\begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=0.3\textwidth]{Images/Section5/lossfun_sec5_Samson_averagev2_part2-eps-converted-to.pdf}
       % \caption{Samson Data set}
    %\end{subfigure} 
    & 
 %add desired spacing between images, e. g.~, \quad, \qquad, \hfill etc.
    %(or a blank line to force the subfigure onto a new line)
    %\begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=0.3\textwidth]{Images/Section5/lossfun_sec5_Jasper_averagev2_part2-eps-converted-to.pdf}
        %\caption{Jasper Ridge Data set}
   % \end{subfigure}
   & 
   % \begin{subfigure}[b]{0.312\textwidth}
        \includegraphics[width=0.312\textwidth]{Images/Section5/lossfun_sec5_Cuprite_averagev2_part2-eps-converted-to.pdf}
       % \caption{Cuprite Data set}
   % \end{subfigure} 
    \end{tabular} 
    \caption{Averaged objective functions over 20 random initializations obtained for Algorithm~\ref{dchsminvolKLNMF} with 300 iterations (red line with circle markers), and the heuristic $\beta$-SNMF from \cite{Leroux} (black dashed line).  
    }\label{fig:hsbetaNMF_lossfun_compa}
\end{figure} 

According to Table~\ref{table:hsbetaNMFperf} (top row), we observe that  Algorithm~\ref{dchsminvolKLNMF} outperforms the heuristic from \cite{Leroux} in terms of final value for the objective functions while $\beta$-SNMF shows lower runtimes. 
Additionally, based on Figure~\ref{fig:hsbetaNMF_lossfun_compa}, we observe that Algorithm~\ref{dchsminvolKLNMF} converges on average faster than $\beta$-SNMF for all the data sets, in terms of iterations.  
However, $\beta$-SNMF has a lower computational cost per iteration.
Thus, we complete the comparison between both algorithms by imposing the same computational time: we run Algorithm~\ref{dchsminvolKLNMF} for 300 iterations, record the computational time and run $\beta$-SNMF for the same amount of time. 
\begin{table}[ht!]
%\footnotesize
\centering
%\begin{center}
\caption{Final value of objective function values $\Phi_\text{end}(W,H)$ for Algorithm~\ref{dchsminvolKLNMF} and the heuristic from \cite{Leroux}. The table reports the average and standard deviation over 20 random initializations for an equal computational time that corresponds to 300 iterations of Algorithm~\ref{dchsminvolKLNMF}.  A bold entry indicates the best value for each experiment. %\ngc{idem Table 4} %\ngc{Cb itérations? Mettre en gras le meilleur.}
} 
\label{table:hsbetaNMFperf2}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{|c|c|c|c|}
  \hline
  Algorithms       & Samson data set & Jasper Ridge data set & Cuprite data set\\
                   & $\Phi_\text{end}(W,H)$ & $\Phi_\text{end}(W,H)$ & $\Phi_\text{end}(W,H)$ \\
  \hline 
   Algorithm~\ref{dchsminvolKLNMF}   &(2.68$\pm$0.00)$10^{3}$  &\textbf{(4.65 $\pm$ 0.00)$10^{3}$} & \textbf{(2.12 $\pm$ 0.00)$10^{3}$} \\
  $\beta$-SNMF~\cite{Leroux}  &(2.68$\pm$0.00)$10^{3}$  &(4.66 $\pm$ 0.00)$10^{3}$  & (2.15 $\pm$ 0.00)$10^{3}$\\
  \hline
\end{tabular} 
%\end{center}
\end{table}
Table~\ref{table:hsbetaNMFperf2} reports the average and standard deviation of the final value for the objective function over 20 runs in this setting.  Figure~\ref{fig:hsbetaNMF_lossfun_compa} (bottom row) displays the objective function w.r.t.\ time for the three data sets. 
%We observe that the conclusions are similar except that heuristic from \cite{Leroux} shows a higher rate of convergence for the first data set. For Jasper and Cuprite data sets, Algorithm~\ref{dchsminvolKLNMF} converges faster in average. 
On this comparison, Algorithm~\ref{dchsminvolKLNMF} and the heuristic from \cite{Leroux} perform similarly although Algorithm~\ref{dchsminvolKLNMF} has slightly better final objective function values. However, keep in mind that only Algorithm~\ref{dchsminvolKLNMF} is theoretically guaranteed to decrease the objective function. 
%\begin{center}
%\end{center}
% \begin{figure}
%     \centering  %add desired spacing between images, e. g.~, \quad, \qquad, \hfill etc. 
%       %(or a blank line to force the subfigure onto a new line)
%     \begin{subfigure}[b]{0.32\textwidth}
%         \includegraphics[width=\textwidth]{Images/Section5/lossfun_sec5_Samson_averagev2_part2-eps-converted-to.pdf}
%         \caption{Samson Data set}
%     \end{subfigure}
% ~ %add desired spacing between images, e. g.~, \quad, \qquad, \hfill etc. 
%     %(or a blank line to force the subfigure onto a new line)
%     \begin{subfigure}[b]{0.32\textwidth}
%         \includegraphics[width=\textwidth]{Images/Section5/lossfun_sec5_Jasper_averagev2_part2-eps-converted-to.pdf}
%         \caption{Jasper Ridge Data set}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.333\textwidth}
%         \includegraphics[width=\textwidth]{Images/Section5/lossfun_sec5_Cuprite_averagev2_part2-eps-converted-to.pdf}
%         \caption{Cuprite Data set}
%     \end{subfigure}
%     \caption{Averaged objective functions over 20 random initializations obtained for Algorithm~\ref{dchsminvolKLNMF} (red line with circle markers) and the heuristic from \cite{Leroux} (black dashed line) applied to the three data sets detailed in Section \ref{secnumexpssNMF} for an equal computational time.  Logarithmic scale for y axis. 
%     }\label{fig:hsbetaNMF_lossfun_compa2}
% \end{figure} 


%In Appendix \ref{appen_quali_res_algoKLsparse}, we report qualitative results obtained with Algorithm~\ref{dchsminvolKLNMF} applied to three HS real data sets, that are Samson, Jasper and Urban data sets.


==> arXiv v2/Chapters/6_Conclusions.tex <==


In this paper we have presented a general framework to solve penalized $\beta$-NMF problems that integrates a set of disjoint constraints on the variables; see the general formulation~\eqref{eq:betaNMFmodel}.  
%penalized multivariate minimization problems based on $\beta$-divergences under linear constraints. The framework treats in a unified manner the penalty term that can be upper bounded as required in Assumption~\ref{ass:phi}. 
Using this framework, we showed that we can derive algorithms that compete favorably with the state of the art for a wide variety of $\beta$-NMF problems, such as  the simplex-structured NMF and the minimum-volume $\beta$-NMF with sum-to-one constraints on the columns of $W$. 
%We have compared the effectiveness and the performance of our algorithms on real data sets against existing and recent methods. In particular we highlighted the gain obtained with our algorithms in terms of convergence rate, runtime and objective function values for many data sets.
We have also shown how to extend the framework to non-linear disjoints constraints, with application to a sparse $\beta$-NMF model for $\beta=1$ where each column of $W$ lie on a hyper-sphere. 

Further works will focus on the possible extension of the methods to non-disjoints constraints. %such as weighted sparsity measured using the ratio of a weighted $\ell_1$ and the $\ell_2$ norms recently introduced in \cite{gillis2019grouped}. 
The non-disjoint constraints will lead to roots finding problems of  polynomial equations in the Lagrangian multipliers for which we hope to find conditions that ensure the uniqueness of the solution. 

Another interesting direction of research would be to apply our framework to other NMF models. For example, in probabilistic latent semantic analysis/indexing (PLSA/PLSI), the model is the following: given a nonnegative matrix $V$ such that $\eb^T V \eb = 1$ (this can be assumed w.l.o.g.\ by dividing the input matrix by $\eb^T V \eb$), solve 
    \[
    \max_{W \geq 0, H \geq 0, s \geq 0} 
    \sum_{f,n} v_{fn} \log(W\diag(s)H)_{fn} 
    \text{ such that } W^T \eb = \eb, H\eb = \eb, s^T \eb = 1 . 
    \] 
    This model is equivalent to KL-NMF~\cite{ding2008equivalence}, with the additional constraint that $\eb^T WH \eb = \eb^T X \eb$, and hence our framework is applicable to PLSA/PLSI. 
    Such constraints have also applications in soft clustering contexts; see~\cite{yang2016low}. 
    


==> arXiv v2/alphabet.tex <==
% Document LaTeX        GLB (25/05/94)
% Modification :        Gio (15/09/95)
%                       JI  (format Latex 2e, taille adaptative 22/03/99)
%                           (fonte blackboard 27/08/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{(necessite les packages xspace, amsmath, bbm)}
\typeout{}

\RequirePackage{amsmath}
\RequirePackage{xspace}
%\RequirePackage{bbm}
\RequirePackage{amssymb}
%\RequirePackage{bbold}
%\RequirePackage{mathbbol}
%\RequirePackage{doublestroke}

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
%\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)
\def\sbl#1{\ensuremath{\mathbb{#1}}}              % Style blackboard (necessite amssymb)

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}

% Complément intéressant...

\def\ellb{\sbmm{\ell}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}


% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}    \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}


